ARMAND: Anti-Repackaging through Multi-pattern Anti-tampering based on Native Detection

App repackaging refers to the practice of customizing an existing mobile app and redistributing it in the wild to fool the final user into installing the repackaged app instead of the original one. In this way, an attacker can embed malicious payload into a legitimate app for different aims, such as access to premium features, redirect revenue, or access to user's private data. In the Android ecosystem, apps are available on public stores, and the only requirement for an app to execute properly is to be digitally signed. Due to this, the repackaging threat is widely spread. Anti-repackaging techniques aim to make harder the repackaging process for an attack adding logical controls - called detection node - in the app at compile-time. Such controls check the app integrity at runtime to detect tampering. If tampering is recognized, the detection nodes lead the repackaged app to fail (e.g., throwing an exception). From an attacker's standpoint, she must detect and bypass all controls to repackage safely. In this work, we propose a novel anti-repackaging scheme - called ARMAND - which aims to overcome the limitations of the current protection schemes. We have implemented this scheme into a prototype - named ARMANDroid - which leverages multiple protection patterns and relies on native code. The evaluation phase of ARMANDroid on 30.000 real-world Android apps showed that the scheme is robust against the common attack vectors and efficient in terms of time and space overhead.

==> [PMC] ARMAND Anti-Repackaging/sections/abstract.tex <==
\begin{abstract}
\emph{App repackaging} refers to the practice of customizing an existing mobile app and redistributing it in the wild to fool the final user into installing the repackaged app instead of the original one. In this way, an attacker can embed malicious payload into a legitimate app for different aims, such as access to premium features, redirect revenue, or access to user's private data. In the Android ecosystem, apps are available on public stores, and the only requirement for an app to execute properly is to be digitally signed. Due to this, the repackaging threat is widely spread.

Anti-repackaging techniques aim to make harder the repackaging process for an attack adding logical controls - called detection node - in the app at compile-time. Such controls check the app integrity at runtime to detect tampering. If a tampering is recognized, the detection nodes lead the repackaged app to fail (e.g., throwing an exception). From an attacker's standpoint, she must detect and bypass all controls to repackage safely. 
% The high-availability of working repackaged apps in the Android ecosystem suggests that the attacker's side is winning. 

In this work, we propose a novel anti-repackaging scheme - called \textbf{\schema{}} - which aims to overcome the limitations of the current protection schemes. We have implemented this scheme into a prototype - named \textbf{\toolname{}} - which leverages multiple protection patterns and relies on native code. The evaluation phase of \toolname{} on 30.000 real-world Android apps showed that the scheme is robust against the common attack vectors and efficient in terms of time and space overhead.

\end{abstract}


==> [PMC] ARMAND Anti-Repackaging/sections/background.tex <==
\section{Background \& Threat Model} \label{sec:background}

This section summarizes the basics of app development and distribution in mobile world with a specific focus on Android, a threat model for app repackaging, and the main techniques at the basis of anti-repackaging schemes.

\subsection{Android App  Life-cycle}
An Android app is usually developed in Java or Kotlin, and leverages XML files to represent the graphical user interface of the app. In addition, some developers can implement parts of their app in Native code (i.e., C/C++ code) leveraging the Android NDK toolset \cite{android-ndk}. 
Each app is distributed and installed as an Android Package ($apk$) file, which is a zip archive containing the executable code in a set of \texttt{classes.dex} files, some binary resources (e.g., picture and movies) as well as a \textsl{manifest} file containing, among others, the description of the app components and the permissions required by the app to execute properly. Finally, the $apk$ also includes some meta-files containing the signature of the app, the public-key certificate of the developers and some file for redundant integrity check. 

Android apps are mainly delivered through software repositories, called \textsl{app stores}, which allow the developers to publish their $apks$, and the users to search, download and install them on their devices.
In addition, it is also possible to distribute an $apk$ directly (e.g., through email or URLs) without the need to upload the app to an app store.

Android requires all $apks$ to be digitally signed in order to be installed on a device.
This mechanism grants the integrity of the $apk$: during the installation phase, Android checks the signature of the $apk$ according to the public-key certificate therein, and denies the installation in case either the signature or the integrity check fail.
However, no identification of the signer is required, thus allowing the installation of apps with self-signed or unknown certificates \cite{android-publish-app}.
%cannot provide any authentication mechanism. 

\subsection{Threat Model}\label{sub:threat-model}
\begin{figure}[!ht]
  \includegraphics[width=\textwidth]{figs/threat-model.pdf}
  \caption{App repackaging: threat model.}
  \label{fig:threat-model-design}
\end{figure}

The threat model for app repackaging involves three actors: the developer, the attacker, and the user.
In an ideal (i.e., attacker-free) scenario, the developer implements the app (Step 1), signs it, and delivers the app to the users via one or more app stores (Step 3). 
The user fetches the app (Step 4) and downloads it (Step 5). Android verifies the signature and the integrity of the $apk$ and installs it on the user's device. Then, the app can execute (Step 6). 

Nonetheless, in a real scenario the developer applies some anti-repackaging protection schemes during the app development (Step 2), to deter the attacker to repackage the app. From her side, the attacker accesses the app directly from the app store, behaving like any regular user: she downloads the app (Step 7), decompiles and reverses the $apk$ (Step 8), and tries to detect and disable potentials anti-repackaging (Step 9). Then, the attacker add some malicious payload to the app (Step 10) and builds-and-signs a repackaged version (i.e., $Rep_{apk}$) of the original app (Step 11). Finally, the attacker tests whether $Rep_{apk}$ works properly (Step 12): if this is the case, the attacker redistributes $Rep_{apk}$ both on app stores and through side-channels (e.g., by email, web servers, or leveraging phishing attacks), aiming to force the user to install $Rep_{apk}$ instead of the original $apk$.  
Otherwise, the attacker tries further to detect and disable other anti-repackaging protections on the original $apk$ (back to Step 8). Steps 8 to 12 are also known as the \textsl{try and error cycle} that the attacker must keep executing until she gets a working repackaged app. To this aim, an ideal anti-repackaging scheme never allows the attacker to obtain a working repackaged app (i.e., moving out from the \textsl{try and error cycle}). Actually, a reliable anti-repackaging solution makes the repackaging non cost-effective, i.e., it requires so much time to be disabled that the attacker gives up from repackaging the app. 

As a final observation, \textsl{repackaging detection techniques} are instead applied on the app store and, sometimes, on the mobile device to detect already repackaged apps. However, in this paper we will focus on anti-repackaging only. 

\subsection{Anti-repackaging Techniques}\label{sub:anti-repackaging}

Anti-repackaging - also known as \textsl{repackaging avoidance} or \textsl{self-protection} - aims to protect an app from being successfully repackaged by adding some protection code - called \textsl{detection nodes} - in the app code before building the $apk$ and delivering it to the app store (Step 2 in Fig. \ref{fig:threat-model-design}). 
%If the effort to overcome the protection would overcome the one needed to develop a new app from scratch, the attacker would likely desist from the repackaging attempt.
The idea of detection nodes has been put forward in \cite{7579771} and it refers to a self-protecting mechanism made by a piece of code inserted into the original $apk$, which carries out integrity checks - called \textsl{anti-tampering} controls (e.g., signature check, package name check) - when executed at runtime \cite{merlo2020you}.
More specifically, anti-tampering checks compare the signature of a specific part of the $apk$ with a value pre-computed during the building of the original app; if such values differs, then a repackaging is detected and the detection node usually leads the app to fail, thereby frustrating the repackaging effort.
 
From the attacker side, most of the activities related to detect and disable anti-tampering refers to the identification and removal of detection nodes. 
To protect detection nodes, most of the anti-repackaging schemes hide them into the so-called \textsl{logic bombs} \cite{10.1145/3168820, 8186215, 10.1007/978-3-030-45371-8_12}, that has been originally conceived in the malware world to hide malicious payloads \cite{sharif2008impeding}. A logic bomb protects (i.e., hides) a detection node by ciphering the node using reliable ciphers at the state of the art. An actual value of a program variable is often used as the key. Logic bombs rely on the information asymmetry between the developer and the attacker, i.e., since the attacker has partial knowledge of the app behaviors, it is unlikely that she can correctly guess the key value used to encrypt the code. % (i.e., constant value \texttt{const}).
\begin{figure}[!ht]
    \centering
    \includegraphics[width=\textwidth]{figs/QC_to_LB.pdf} 
    \caption{Transformation process of a qualified condition into a logic bomb.}
    \label{fig:qc_to_lb}
\end{figure}

Figure \ref{fig:qc_to_lb} shows a common scheme for building a logic bomb by re-writing a \textsl{qualified condition} - i.e., a condition containing an equality check, where one of the operands is a constant value (e.g., \longstring{v==const}) - in a branch. 
The original condition is transformed in a new one where the pre-computed hash value of the constant \texttt{const} (i.e., \texttt{HASH}) is compared with the result of the hash function applied to variable \texttt{v} plus some \texttt{salt}. 
The detection nodes are embedded into the body of the qualified condition, which is encrypted using the original \texttt{const} as the encryption key. The protection of the logic bomb is granted by the one-way property of cryptographic hash functions, that makes hard for the attacker to retrieve the original \texttt{const} value (i.e., the decryption key) from its hash. In addition, the anti-tampering checks can be embedded either in Java or in native code (i.e., C/C++) to improve reliability.

From an attacker standpoint, all logic bombs must be detected and removed to create a fully working repackaged $apk$. To this aim, an attacker can leverage both static and dynamic analysis to locate and deactivate the anti-tampering controls (e.g., code analysis and pattern matching, code instrumentation). As a complete analysis of such attacking techniques is out of scope in this paper, the interested reader may refer to \cite{merlo2020you, 10.1145/2996358, LI201767, GAJRANI202073}.


==> [PMC] ARMAND Anti-Repackaging/sections/bios.tex <==
\bio{figs/alessio.jpg}
\textbf{Alessio Merlo} is an Associate Professor in Computer Engineering in the Departiment of Informatics, Bioengineering, Robotics and System Engineering Department (DIBRIS) at the University of Genoa, and a member of the Computer Security Laboratory (CSEC Lab). His main research field is Mobile Security, with a specific interest on Android security, automated static and dynamic analysis of Android apps, mobile authentication and mobile malware. More information can be found at: \url{http://csec.it/people/alessio\_merlo/} 
\endbio

\vspace{0.2in}

\bio{figs/antonio.jpg}
\textbf{Antonio Ruggia} is a PhD student in Computer Engineering at the University of Genoa. He is interested in several security topics that include Mobile Security, with a specific interest in Android and data protection. He graduated in October 2020 at University of Genoa and participated in the 2019 CyberChallenge.it, an Italian practical competition for students in Cybersecurity. He regularly participates in international Capture-The-Flag (CTF) competitions. Since 2018, he has been working as a full-stack developer in a multinational corporation.
\endbio

\vspace{0.1in}

\bio{figs/luigi.jpg}
\textbf{Luigi Sciolla} holds a Master degree in Computer Engineering at University of Genoa. During his studies he worked as a system administrator and full stack mobile developer. His area of interests are computer networks and Android security. He participated in the 2018 CyberChallenge.IT finals. Since 2018, he is also member of ZenHack, the capture-the-flag team at the University of Genoa. With ZenHack he competed in dozens of online and onsite competitions. 
\endbio

\vspace{0.25in}

\bio{figs/lucav.jpeg}
\textbf{Luca Verderame} obtained a Ph.D. in Electronic, Information, Robotics, and Telecommunication Engineering at the University of Genoa (Italy) in 2016, where he worked on mobile security. He is currently working as a post-doc research fellow at the Computer Security Laboratory (CSEC Lab), and he is also the CEO and Co-founder of Talos, a cybersecurity startup and university spin-off. His research interests mainly cover information security applied, in particular, to mobile and IoT environments.
\endbio


==> [PMC] ARMAND Anti-Repackaging/sections/conclusion.tex <==
\section{Conclusion and Future Works} \label{sec:conclusion}

In this work, we proposed \schema{}, an anti-repackaging protection scheme that overcomes the main limitations of current state-of-the-art protection schemes by introducing multiple protection patterns (i.e., Java anti-tampering checks and six different types of logic bombs) that relies on native technologies.

Furthermore, we implemented \schema{} in a tool for protecting Android apps, called \toolname{}, that is publicly available on GitHub\footnote{\url{https://github.com/Mobile-IoT-Security-Lab/ARMANDroid}} and on Docker Hub\footnote{\url{https://hub.docker.com/repository/docker/totor13/armand}}.
The evaluation of 30.000 Android apps demonstrated the applicability and the efficacy of the tool and the proposed protection scheme.
\toolname{} enables developers to protect their apps against repackaging attacks and can be easily included in existing application development processes. Furthermore, \toolname{} support the application, after the protection phase, of different obfuscation techniques (e.g., Obfuscapk \cite{aonzo2020obfuscapk}, ProGuard \cite{proguard}) to make static analysis harder for an attacker.

As a future extension of this work, we plan to \emph{i)} define a heuristic to evaluate and select the best QCs to be transformed into detection nodes, \emph{ii)} extend the multi-pattern protections (e.g., by adding mixed client-side and server-side controls), and \emph{iii)} evaluate the applicability to the iOS environment.

%In the first part of this work, we identified and examined the guidelines to improve the reliability of anti-repackaging techniques at the state of the art. Then, we proposed \schema{}, an anti-repackaging protection scheme which aims to overcome current limitations. We implemented this scheme in a tool, \toolname{}, for protecting Android apps.
%The evaluation phase shows that the protected apps are equipped with several detection nodes and the performance impact is negligible. 

%We investigate the possibility to defend an app with multiple protection schemes (e.g., NRP - detailed in Section \ref{sec:related_works} - and after \toolname{}). Each scheme modifies the source code (i.e., Java bytecode) to adds detection nodes and anti-tampering controls whose goal is to detect tampering. Due to this, if we protect the same app with two protection schemes, the first one will detect the tampering caused by the second protection scheme. However, an app developer can apply different obfuscation techniques (e.g., Obfuscapk \cite{aonzo2020obfuscapk}, ProGuard \cite{proguard}) after \toolname{} protection to make static analysis harder for an attacker.

\begin{comment}
We focused on Android OS, but, the \schema{} protection scheme can be ported to iOS too. Furthermore, \toolname{} can be improved by adding other anti-tampering functions or finding more qualified conditions.
In particular, client-server paradigm (e.g., server side anti-tampering controls or code splitting techniques) could generate new types of bomb (i.e., new logic bomb patterns). %The server-side ones are based on a secure communication channel and a trusted data source (i.e., the server relies on clients’ data). Due to this, anti-repackaging server-side controls can be bypassed by tampering with the communication channel. Contrary, the server-side controls allows an app developer to change often the serve-side controls (i.e., transparently to the app) and to make unusable oldest app versions. In this way, a repackaged version of an app stop working after some time (due to it is an oldest and deprecate version of the app) and an attacker have to continuously repackaged new version of the same app.

%With this work, we hope to be able to help Android App developers against the repackaging threat. 
\end{comment}


==> [PMC] ARMAND Anti-Repackaging/sections/implementation.tex <==
\section{\toolname{}: an implementation for Android of \schema{}} \label{sec:implementation}

We implemented the \schema{} anti-repacking scheme in a prototype tool called \toolname{}, that can be executed as a Docker image available at \url{https://hub.docker.com/repository/docker/totor13/armand}.
The tool is transparent to the development pipeline as it can work directly on pre-delivery $apk$ files. Indeed, the developer can build the app bundle, apply the \toolname{} protection, and finally sign the resulting app for the distribution.

%Due to \toolname{} works directly on an $apk$ file, the protection process is transparent to a developer: she builds its app bundle (i.e., $apk$ file), apply the \toolname{} protection, sign the app with her private key and distribute the protected app, for instance, through one or more app stores.

\toolname{} is written in Java and relies on the Soot framework \cite{soot} to analyze and modify the Java bytecode, %using the Jimple intermediate language,
 and the Axml\footnote{\url{https://github.com/Sable/axml}} library to parse and modify the Android manifest file.
The tool exposes four input parameters, i.e., three percentage values ($P_{Java\_{AT}}$, $P_{native\_key}$, and $P_{native\_AT}$) and a package name (\texttt{PN}).
Briefly, the three percentage values allow \toolname{} to determine the probability to include the Java AT checks and the six types of logic bombs. 
The package name specifies the part of the app in which the tool will inject the protection controls. If \texttt{PN} is set to $none$, the tool will apply the protection to all the Java classes in the app. 

\begin{figure}[!ht]
    \includegraphics[width=\textwidth]{figs/antirepackaging-flow.pdf}
    \caption{The \toolname{} protection workflow.}
    \label{fig:antirepackaging-protection-flow}
\end{figure}
The protection process can be divided into three macro-steps (see Figure \ref{fig:antirepackaging-protection-flow}):
\begin{enumerate}
    \item \emph{App Pre-processing.} \toolname{} unpacks the $apk$ file to extract the \texttt{classes.dex} file(s). The bytecode is then translated into an intermediate language, called Jimple \cite{vallee1998jimple}, used by Soot for analysis and modification tasks.  During this phase, \toolname{} scans the app code in \texttt{PN} to find all the qualified conditions (QC).
    Furthermore, the tool injects a set of Java AT checks into the bytecode. 
    \item \emph{Bomb Injection.} For each QC, the tool includes - according to the input probabilities $P_{Java\_AT}$, $P_{native\_key}$, and $P_{native\_AT}$ - one or more logic bombs belonging to the six different types defined in Section \ref{subsec:spatternization}. If the bomb requires native code, \toolname{} builds the corresponding native method and all the auxiliary code needed for its execution.
    %native methods and add their invocation. The logic bombs created match one of the six types introduced in \ref{subsec:spatternization}
    \item \emph{App Packing.} Finally, \toolname{} transforms back the Jimple representation into bytecode, adds the native libraries, updates the \longstring{AndroidManifest.xml} file, and creates the protected $apk$ file, ready for the signing process.
\end{enumerate}


The rest of this section details the implementation of each of the steps.

\subsection{App Pre-Processing}\label{subsec:app-analysis}

During this phase, the tool processes the app's code to i) identify all the QCs that can host logic bombs and ii) inject the Java AT controls.

\paragraph{\textbf{Unpacking and translation.}} At first, \toolname{} unpacks and extracts from the $apk$ file the \texttt{classes.dex} file(s) containing the compiled Java code. The compiled code is then transformed in the Jimple intermediate language using Soot.

\paragraph{\textbf{QC Identification.}} \toolname{} scans the Jimple code belonging to the package $PN$ to detect sets of consecutive instructions (hereafter, blocks) that can host one or more logic bombs. These blocks must match the \emph{qualified condition} pattern as described in Section \ref{sub:anti-repackaging}.

In the current implementation, \toolname{} considers two types of QCs, i.e., if statements and switch-case statements. For the latter case, each case of the switch instruction is translated into a separate qualified condition. 
For each discovered QC, \toolname{} builds an Abstract Syntax Tree (called \emph{transformation tree}) with the qualified condition as the root node.
In the case of nested QCs, the transformation tree will add the inner QCs as leaf nodes to keep track of their hierarchy.

Moreover, the tool also stores the link to the beginning and the end of the block of instructions that can be encrypted in the bomb, namely the \emph{encryption range}, for each discovered QC. The encryption range encloses the set of consecutive instructions (up to the maximum size of \texttt{or\_code}) that do not contain further branches. 

\paragraph{\textbf{Java AT Injection.}} During the parsing phase, \toolname{} injects Java AT controls into the app code. In detail, the tool injects a Java AT before each parsed instruction with the input probability $P_{Java\_AT}$, using the algorithm sketched in Figure \ref{fig:add-java-at}.
At the end of the process, the probability to embed at least a Java AT into a set of \texttt{n} instructions is $P_{Java\_AT\_embedded} = 1 - (1-P_{Java\_AT})\;^{n}$.

\begin{figure}[!htbp]
    \begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
    ]
    Iterator<Unit> iter = units.snapshotIterator();
    Unit currentUnit = iter.hasNext() ? iter.next() : null;
    Unit nextUnit = null;
    while (iter.hasNext()) {
        nextUnit = iter.next();
        Stmt stmt = (Stmt) currentUnit;
        
        [...]
        
        if (!(stmt instanceof IdentityStmt) && 
                random.nextInt(100) >= (100-P_JAVA_AT)) {
            // add Java AT before stmt
            [...]
        }
        currentUnit = nextUnit;
    }
    \end{lstlisting}
\caption{Code snippet adding Java anti-tampering checks.}
\label{fig:add-java-at}
\end{figure}

\subsection{Bomb Injection} \label{sub:code_transformation}

In the Bomb Injection phase, \toolname{} traverses each transformation tree using a post-order procedure to process all the QCs detected in the previous phase. The goal of this phase is to transform each QC into a logic bomb belonging to one of the six types defined in Section \ref{sec:methodology}, using the process depicted in Figure \ref{fig:creation-of-logic-bomb}.  
\begin{figure}[!ht]
    \includegraphics[width=\textwidth]{figs/creation-of-logic-bomb.pdf}
    \caption{Transformation of a candidate node into a logic bomb.}
    \label{fig:creation-of-logic-bomb}
\end{figure}

At first, the qualified condition is transformed into 
%the encrypted form. In details, the condition $v == const$ is transformed into 
$hash(v, salt) == H$, where the \texttt{salt} is a pseudo-random value and $H$ is the pre-computed hash value of the constant \texttt{const} (Step 2.1). Step 2.2  evaluates the \texttt{or\_code} to ensure that the original method will be correctly executed after the transformation process. To do so, \toolname{} inspects the execution flow to detect how the execution will behave after the execution of \texttt{or\_code}.
In particular, we identify four possible situations, as the original code may i) proceed to the next block of instructions, ii) throw an exception, iii) jump to a different block, or iv) terminate the execution returning an object.
Thus, the tool - similarly to the solution proposed in  \cite{10.1007/978-3-030-45371-8_12} - adds an auxiliary Java class called \longstring{ResultWrapper} in charge of enforcing the original execution flow after \texttt{or\_code}.

After the first two steps, \toolname{} evaluates the content of \texttt{or\_code} and injects a native call implementing either a Native-key or a Native AT function (Step 2.3).
The probability to create a specific type of a logic bomb depends on the input percentages $P_{native\_key}$ and $P_{native\_AT}$, and the content of the \texttt{or\_code}.

In detail, if the \texttt{or\_code} contains at least one (or more) \texttt{Java AT} (with probability $P_{Java\_AT\_embedded}$), the resulting bomb will be a \texttt{Java AT \& Native-key} bomb with a probability of $P_{native\_key}$, while the probability to have a \texttt{Java \& Native AT bomb} is $P_{native\_AT\; |\; \neg\; native\_key}$. 
If no native functions are injected, then the QC will contain a plain \texttt{Java Bomb} with the probability $P_{Java\_bomb} = 1 - P_{native}$ where $P_{native}$ corresponds to the join probabilities of having a logic bomb with a \emph{native key} or a native AT control (i.e., $P_{native} = P_{native\_key}\; \cup \;P_{native\_AT\; |\; \neg\; native\_key}$).

Otherwise, if \texttt{or\_code} does not contain any Java AT (with probability $1 - P_{Java\_AT\_embedded}$), the bomb could be a \texttt{Native-key bomb} (with probability $P_{native\_key}$), a \texttt{Native AT} bomb (with probability $P_{native\_AT\; |\; \neg\; native\_key}$), or - if no injection occurred - a \texttt{Honeypot}.

In Step 2.4, \toolname{} encrypts \texttt{inner\_code} in the \emph{encryption range} using AES-128 and the result is included in an encoded string using $base64$ (\texttt{inner\_code\_encr}). The encryption/decryption key is derived from the value of \texttt{const}. 
Then, \toolname{} adds the  instructions required to decrypt and invoke the encrypted inner code. To this aim, the tool embeds two auxiliary classes in the Android app, i.e., \longstring{EncryptHelper} and \longstring{InvokeHelper}. The first one is responsible to decrypt \texttt{inner\_code\_encr} using the decryption key. The latter class is responsible for loading a byte array (corresponding to the bytecode resulting from the decryption of the \texttt{inner\_code\_encr}) into the memory and invoking the $execute$ method. In particular, \longstring{InvokeHelper} leverages the \longstring{InMemoryDexClassLoader} class\footnote{\url{https://developer.android.com/reference/dalvik/system/InMemoryDexClassLoader}} to load and execute the code from a byte array (i.e., the byte of the dex file). 
Finally, in Step 2.5, the tool recovers the original execution flow by invoking the \longstring{ResultWrapper} object. 

\subsection{App Packing}

The last step enables the generation of a working protected $apk$ file. 
At the beginning, the Jimple representation of the code is transformed back into the Java bytecode. 
After that, \toolname{} generates a set of shared libraries, one for each supported ABI, containing the native functions included by the tool in the previous phase. The current implementation of the tool supports \texttt{armeabi-v7a}, \texttt{arm64-v8a}, \texttt{x86}, and \texttt{x86-64}.

Then, \toolname{} updates the \longstring{AndroidManifest.xml} file to include the auxiliary classes and the new shared libraries and builds the new $apk$ file.
Finally, \toolname{} sends the protected app to the Obfuscapk \cite{aonzo2020obfuscapk} tool to mask the anti-tampering protections included in the app. 
At the end of this phase, the output \texttt{apk} is ready for the signing process. 

==> [PMC] ARMAND Anti-Repackaging/sections/intro.tex <==
\section{Introduction}

In the mobile world \textsl{repackaging} refers to the practice of retrieving an app from a public store, decompile it, add some extra code, and then build a new version of the app to deliver in the wild. In the Android ecosystem, repackaging is the main carrier for malware to spread, as an attacker may retrieve a target official app (i.e., Facebook), reverse engineer it \citep{2011-android-reversing}, and enclose a malicious payload. Finally, the attacker packs and signs the modified version of the app (i.e., the repackaged app), and re-distributes it in official app stores (e.g., Google Play Store \cite{google-play-store} and Samsung App Store \cite{samsung-store}) or over the Internet, trying to fool the user to install the repackaged version of the app instead of the original one. This last step can be achieved by well-established attack vectors, like phishing \cite{phishing-ccs18}.  

Albeit in recent years several proposal have been put forward to counteract this threat \cite{7299906, 7579771, 8368344, 8186215, 10.1145/3168820, 10.1007/978-3-030-45371-8_12}, this issue is far from being solved \cite{merlo2020you}, mostly due to the fact that Android carries out just some soft checks on the signature of an app. More precisely, the only requirement for an app bundle (i.e., the $apk$ file) to be installed on a mobile device is that it contains a valid signature, independently from the actual identity of the developer. 
Furthermore, the user has the possibility to install third-party apps from unknown sources, thus limiting the efficacy of security controls carried out on the official app stores (e.g., Google Bouncer \cite{google-bouncer} and Google Play Protect \cite{google-play-protect} for Google Play Store).
Previous choices foster the spread of repackaged apps and demand for proper solutions to counteract this threat.

In this respect, the current SotA is divided into two orthogonal categories, namely i) \textsl{repackaging detection}, that focuses on recognizing and identifying already repackaged apps in the wild, and ii) \textsl{anti-repackaging} (also known as \textsl{repackaging  avoidance}) that aims at protecting original apps against repackaging. 
Briefly, \textsl{anti-repackaging} methodologies focus on inserting logic controls (called \textsl{detection nodes}) that embed integrity checks on the content of the $apk$, called \textsl{anti-tampering} (AT) controls. 
The detection nodes are triggered during the execution of the app, and if some tampering is detected, the app is usually forced to crash. The rationale is to discourage the attacker from repackaging if the likelihood of building a working repackaged app is low.

Concerning anti-repackaging, the scientific community proposed several protection schemes that leverage some fruitful combination of AT controls and detection nodes to protect apps.
Unfortunately, as we demonstrated in a recent work \cite{merlo2020you}, all the proposals so far rely on rigid patterns for inserting detection nodes or adopt only some trivial AT controls that could be easily detected and circumvented by attackers.

To tackle this problem, in this paper we propose a novel anti-repackaging scheme - called \textbf{\schema{}} (\textsl{\underline{A}nti-\underline{R}epackaging through \underline{M}ulti-pattern \underline{A}nti-tampering based on \underline{N}ative \underline{D}etection}) -  that is able to overcome the limitations of the current proposals. \schema{} fulfills the anti-repackaging challenges identified in \cite{merlo2020you} as it relies on multiple protection patterns, heterogeneous AT controls, multi-level detection nodes, and self-hiding techniques. 
\schema{} allows developers to include novel, hard-to-identify and hard-to-reverse security controls in their apps to prevent repackaging.

Furthermore, we developed a prototype implementation for Android apps - \textbf{\toolname{}} - that can be included in the standard development life-cycle of an $apk$. The tool has been evaluated on 30000 Android apps downloaded from different app stores, such as F-Droid \cite{f-droid} and Google Play Store \cite{google-play-store}. The evaluation phase proved the reliability of \schema{} that allows distributing a high number of detection nodes in the apps at the cost of a negligible runtime overheads in terms of memory and cpu usage. To prove the latter result, we tested 220 apps to compare the runtime overhead between original and protected apps. The \toolname{} tool is publicly available on GitHub at \url{https://github.com/Mobile-IoT-Security-Lab/ARMANDroid}, while a Docker image can be found at \url{https://hub.docker.com/repository/docker/totor13/armand}.

\paragraph{\textbf{Structure of the paper.}} First, we introduce the threat model related to the app repackaging in the Android ecosystem and the main app-repackaging techniques (Section \ref{sec:background}). 
In Section \ref{sec:related_works}, we report state-of-the-art anti-repackaging protection schemes, thereby underlying their current limitations. 
Then, we present the \schema{} protection scheme, its distinguish features (Section \ref{sec:methodology}), and its resiliency against the main repackaging attacks (Section \ref{sec:security}). 
In Section \ref{sec:implementation}, we present the \toolname{} implementation and, in Section \ref{sec:experimental_result}, we detail the experimental campaign on 30.0000 real-world Android apps and the run-time evaluation of 220 protected apps.
Finally, in Section \ref{sec:conclusion} we conclude the paper by summing-up the main takeaways and putting forward some consideration for future works.


==> [PMC] ARMAND Anti-Repackaging/sections/limitations.tex <==
\subsection{Prototype Limitations} \label{sec:limitation}

The experimental campaign led to the identification of some limitations of the \toolname{} tool that will be discussed below.
During the protection of 30.000 apps, 963 of them (i.e., 3.2\% of total apps) resulted in a crash due to the transformation in Jimple code. This is mainly related to the transformation of the switch-case statements. 
In particular, \toolname{} has to replace each switch-case statement with a list of if statements, and, thus, it has to update all links and dependencies to preserve the original execution flow. In some cases, \toolname{} fails to reconstruct the original dependencies causing a crash of the protection process.

Besides, \toolname{} inherits all the limitations of third-party libraries (e.g., the Soot framework) for both the protection phase and the runtime execution. In particular, during the transformation of the Java bytecode, Soot automatically applies some optimization techniques. Thus, the resulting bytecode, even the one outside $PN$, always differs from the original one. Unfortunately, such modifications in the case of third-party libraries (e.g., AdMob\footnote{\url{https://developers.google.com/admob/android/quick-start}}) may cause runtime errors that result in a user-experience glitch (e.g., a not-working advertisement banner).

Furthermore, \toolname{} leverages the \texttt{InMemoryDexClassLoader} class (which is introduced in API 26) to load and invoke the decrypted code at runtime. Due to this, the protected app needs to support API 26 as minimum API level or exceptions can occur\footnote{For instance, \url{https://stackoverflow.com/questions/38200282/android-os-fileuriexposedexception-file-storage-emulated-0-test-txt-exposed}} during its execution.

Finally, it is worth noticing that the protection depends on the portion of code that could be processed (i.e., the code contained in \texttt{PN}). Indeed, the selection of a package name with few classes and methods could result in an insufficient protection. For instance, some protected apps (6.115 out of the 27.656 apps) have not been equipped with any anti-tampering protection mechanism because the package name $ApplicationID$ contains few lines of Java bytecode (e.g., the case of hybrid apps). For this reason, the tool does not find any candidate qualified condition suitable to embed logic bombs.
However, it is worth noticing that such a problem can be mitigated by using a more permissive package name to cover, for instance, the entire app (i.e., setting \texttt{PN} to \emph{none}) and not only the $ApplicationID$ package.


==> [PMC] ARMAND Anti-Repackaging/sections/methodology.tex <==
\section{The \schema{} Scheme} \label{sec:methodology}

In this work, we present \schema{} (\underline{A}nti-\underline{R}epackaging through \underline{M}ulti-pattern \underline{A}nti-tampering based on \underline{N}ative \underline{D}etection), a novel anti-tampering protection scheme that embeds logic bombs and AT detection nodes directly in the $apk$ file.
\schema{} aims at overcoming the main limitations of the current state-of-the-art schemes briefly introduced in Section \ref{sec:related_works}, by addressing the following challenges:

\begin{enumerate}
    \item \textbf{Use of multiple patterns} to disseminate and hide logic bombs in the app. Current techniques adhere to a single common pattern (i.e., qualified conditions and adoption of hash functions as shown in Figure \ref{fig:qc_to_lb}), that can be detected and de-activated by an attacker through static code analysis and pattern matching techniques. To this aim, \schema{} includes several - distinct - patterns for logic bombs and AT tampering checks to harden the detection and removal phase.
    \item \textbf{Rely on native technologies (C/C++)} to hide the anti-tampering protection. As reversing and instrumenting native code significantly increase the detection and removal of security controls, \schema{} introduces a set of logic bombs and AT checks specifically designed to exploit native code.
    \item \textbf{Optimize the effectiveness of the detection nodes}. Some approaches implement few controls in the name of performance, while others embed many bombs that are not actually triggered at runtime. In this respect, \schema{} adopts an effective deployment of logic bombs, ensuring that logic bombs and AT checks are not included in unused code.
    \item \textbf{Use Honeypot bombs}. The idea is to include fake logic bombs that - disguised as legitimate ones - increase the complexity of the detection and removal phases. Although such a concept has already been proposed in the literature, \schema{} is the first methodology that relies on their usage.
    \item \textbf{Hide the anti-repackaging protection}. It is fundamental to improve the stealthiness of anti-repackaging controls and detection nodes to make  hard for the attacker to understand that the reverse-engineered app includes a protection scheme. Therefore, \schema{} relies on hiding techniques, e.g., obfuscation \cite{aonzo2020obfuscapk}, to mask the detection nodes.
\end{enumerate}

In the remaining of this section, we detail the main features of \schema{} and presents the deployment of the protection scheme and the hiding strategies. Finally, we describe the runtime behavior of our anti-repackaging scheme.

\subsection{Multi-patterning Logic Bombs \& AT checks}
\label{subsec:spatternization} 

As logic bombs are currently built according to the canonical pattern depicted in Fig. \ref{fig:qc_to_lb}, the attacker can systematically detect any potential location of the anti-tampering detection nodes by identifying all branches containing hash values in their condition, and then automate their removal. 
To mitigate such an issue, \schema{} adopts six different types of logic bombs:
\begin{enumerate}
    \item \textbf{Java bomb}. It represents the canonical logic bomb implemented in Java code. The inner code is enriched with one or more Java AT checks and then encrypted with the value of the qualifying condition (\texttt{const}). 
    \item \textbf{Native-key bomb.} It is built by encrypting the inner code of the qualified condition where the decryption key is the return value of an anti-tampering check that is implemented in the native code. 
    Figure \ref{fig:native_encryption_procedure} shows the creation process of this type of bomb. 
    
     \begin{figure}[!ht]
      \includegraphics[width=1.05\textwidth]{figs/native_encryption_procedure.pdf}
      \caption{Creation process of a Native-key bomb.}
      \label{fig:native_encryption_procedure}
    \end{figure}
   
    
    First, the qualifying condition is transformed into a hash comparison using the $const$ value and a salt (Step 1) generated by a pseudo-random function at compile time. The inner code of the qualifying condition is substituted with a native call (Step 2) whose return value is used to encrypt the original inner code (i.e., \texttt{or\_code}) (Step 3). Then, the bomb includes an instruction to decrypt and run \texttt{or\_code\_encr} (Step 4).
    Finally, the entire \texttt{inner\_code} is encrypted with the \texttt{const} value of the qualified condition to generate the \texttt{encr\_code} (Step 5).
    \item \textbf{Native AT bomb.} It implements one or more anti-tampering checks inside the native code. In detail, \schema{} adds an invocation to a native function in the \texttt{or\_code} that implements one or more native AT checks. Finally, the entire \texttt{inner\_code} is encrypted with the \texttt{const} value of the qualified condition to generate the \texttt{encr\_code}. 
    \item \textbf{Java AT \& Native-key bomb.} This bomb extends the Native-key bomb with AT checks in Java code. To do that, \schema{} includes additional instructions in the \texttt{or\_code} to execute one or more AT checks. The code is then encrypted using the workflow of the native-key bomb.
    \item \textbf{Java \& Native AT bomb.} This category of bombs combines AT checks executed in Java and in native code. The bomb enriches the \texttt{or\_code} with instructions to execute one or more Java AT checks and with a native function invocation that executes one or more native AT checks. Then, the entire \texttt{inner\_code} is encrypted with the \texttt{const} value of the qualified condition to generate the \texttt{encr\_code}.
    \item \textbf{Honeypot bomb.} This is a fake logic bomb, which does not contain any anti-tampering check (i.e., the \texttt{or\_code} is not changed). Honeypots aim at tricking the attacker into spending time and effort to decrypt them uselessly.
\end{enumerate}

In our work, each anti-tampering node executes a different AT technique to detect a \emph{specific type} of repackaging. 
\schema{} supports several controls in either Java and native code, such as environment controls (e.g., emulator detection), signature check, package name check, and file integrity check (e.g., resource and image files). We refer the interested reader to \cite{merlo2020you} for a detailed description of the different AT techniques that can be used in an anti-repackaging scheme.

In addition to logic bombs, \schema{} also allows the inclusion of additional detection nodes, called \textbf{Java AT}. Such anti-tampering checks are spread in the entire Java code of the app to detect potential repackaging attempts and are not included in logic bombs. To this aim, the attacker needs to scan and inspect the entire code (and not only the qualifying conditions) to detect and bypass each of them.

\subsection{Protection Deployment and Hiding Strategies}

State of the art anti-tampering schemes tend to add multiple detection nodes that share a single implementation of an AT check (e.g., a signing verification) located either in the Java or native part of the app. Consequently, disabling a single AT check (e.g., using dynamic code instrumentation) could imply the removal of several (or all, in the worst case) detection nodes, thus invalidating the protection.

To mitigate the problem, \schema{} replicates - for each logic bomb or AT check - the corresponding code, and encrypts each piece of code with a different key of the bomb. Such a deployment strategy allows the mitigation of single-point-of-failure exploits since the attacker needs to detect and disable every single control included in the $apk$ file.

Furthermore, \schema{} extends the concept of a logic bomb to \textbf{nested logic bomb}, i.e., where the content of a logic bomb can hide one or more encrypted bombs. In this way, an attacker has to decrypt all the nested logic bombs to recover and remove the included anti-tampering checks.
Besides, \schema{} inserts a different type of bomb for each qualified condition and a different AT controls each time, based on semi-stochastic criteria. Briefly, the \schema{} anti-tampering scheme allows the definition of a set of probability values (one for each type of bomb), which are used to determine the type of logic bombs that will be embedded. Also, \schema{} includes a percentage indicating the frequency with which the Java AT node is spread through the bytecode to increase the complexity of the protection profile. This process is detailed in Section \ref{sec:implementation}.

Finally, \schema{} empowers a set of obfuscation engines, based on the Obfuscapk methodology \cite{aonzo2020obfuscapk}, to further prevent the detection of logic bombs and AT checks. 

\subsection{Runtime  Behavior}

At runtime, the Java AT checks and the logic bombs included in the app are executed. The code in the logic bombs is executed if and only if the hash value of the variable (\texttt{v}) in the qualifying condition (combined with the pseudo-random salt) is equal to the hard-coded hash (i.e., the pre-computed hash value of \texttt{const}). 
If this is the case, the inner code is decrypted using \texttt{v} as the decryption key.
Such a code could contain: i) the original instructions and no anti-tampering checks (Honeypot bombs), ii) one or more Java AT checks - that are immediately executed, iii) a call to a native function (e.g., Native anti-tampering controls), or iv) an inner logic bomb. In the latter case, the execution will proceed iteratively to decrypt the inner bomb and act accordingly. When an AT check is triggered, the code immediately runs the anti-tampering control (e.g., a signature verification). In case of failure, the AT check raises an exception that blocks the execution of the app.

Figure \ref{fig:LB-runtime-behavior} depicts an example of two nested logic bombs: a \emph{Native-key bomb} that contains a \emph{Java bomb}.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=1.02\textwidth]{figs/LB_runtime_example.pdf}
    \caption{Runtime behavior of a nested logic bomb.}
    \label{fig:LB-runtime-behavior}
\end{figure}
Initially, the app evaluates a first logic (canonical) condition ($hash(v, salt) == HASH$). If the equality is satisfied, 
the inner code (i.e., \texttt{encr\_code}) of the logic bomb is decrypted and executed (Step 1). 
The \texttt{inner\_code} contains i) a call to a native function that returns the correct decryption key if a tampering control succeeds and ii) a ciphered code (i.e., \texttt{or\_code\_encr}). 
In this way, if a repackaging is detected, the decryption function fails (i.e., the decryption key is not correct), and the app crashes, throwing an exception; otherwise, the decrypted code is executed (Step 2). 
Part of the decrypted code (i.e., \texttt{or\_code\_1}) can be executed directly, while the remaining part corresponds to a Java bomb.
Thus, the app evaluates the second logic condition ($hash(v1, salt1) == HASH1$) (Step 3). In case of success, the code is decrypted to obtain \texttt{or\_code\_2}. Finally, the app executes the Java AT checks included in the Java bomb (in the example, it checks the debugger flag). If such a control detects a repackaging, it will throw an exception (causing an app crash); otherwise, the app continues the execution of \texttt{or\_code\_2} (Step 4).


==> [PMC] ARMAND Anti-Repackaging/sections/old paper files/attacking.tex <==
\section{Disabling Anti-Repackaging} \label{sec:attack} 

In this section we discuss how the attacking techniques previously discussed can be leveraged to disable the anti-repackaging techniques presented in Section \ref{sec:attacking_model}, and to build a fully working repackaged app. 
%We will shortly describe the novelty introduced in each work, and eventually try to attack them. 

Unfortunately, the vast majority of the older anti-repackaging techniques (i.e., described in Sections \ref{subsec:dyn-self-prot-encrypt-2015}, \ref{subsec:ssn-2016}, \ref{subsec:appis-2017}, \ref{subsec:sdc-2018} and \ref{subsec:bombdroid-2018}) have no available implementation to date. We tried to contact their authors via institutional emails, but we did not receive any positive answer (i.e., neither the source code nor a sample of a protected app). %\luigi{forse nelle parentesi precedenti ci manca il predicato? Oppure in inglese va bene così?} 
For this reason, we will just provide some motivated guidelines on how such techniques can be circumvented. 

However, the source code of the  native extension of BombDroid \cite{10.1007/978-3-030-45371-8_12}, described in Section \ref{subsec:bombdroid-native-2019}, is available as source code on GitHub \cite{repackaging-protection}. For this latter and more recent proposal, we describe a full-fledged attack able to circumvent all the anti-repackaging checks.

It is also worth noticing that none of the anti-repackaging techniques carries out any anti-debugging or emulation check. This basically simplifies the execution of cumulative attacks because the attacker is able to perform tests without worrying about emulator or debugging detection.


\subsection{Self-Protection through $dex$ Encryption}
The encryption method used to cipher the \texttt{classes.dex} file is a XOR encryption. This method could be easily extended to adopt more secure ciphers, like, e.g., AES; nonetheless, this would increase the runtime overhead.

Independently from the cipher, the main drawback of the proposal is that the  decryption key of the ciphered bytecode (i.e., the \texttt{classes.dex} file) is hardcoded in an obfuscated (via LLVM/OLLVM) native activity.  However, there is no need to statically de-obfuscate the native code to retrieve the key, as three dynamic analysis attacking techniques can be leveraged:
\begin{itemize}
    \item symbolic execution could reveal the decryption key and how it is obtained. This technique allows tracking several execution flows showing the value of the variables, including the decryption key;
    \item the debugger allows to detect the actual value of the key at runtime. To debug the app, the only modification is to change the value of the debuggable flag into the \emph{AndroidManifest.xml} file. This tampering is not detected by the XOR-based checksum at runtime;
    \item code instrumentation could allow retrieving the decryption key which is passed as parameter to the decryption function. Function calls could be intercepted with different tools (e.g., see the Frida script in Figure \ref{fig:native-dump-argument-frida}) in order to report back the the values of its arguments. 
    \begin{figure}[!htbp]
    \begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
    ]
    function inspectModule(module) {
      var m = Process.getModuleByName(module);

      Interceptor.attach(m.getExportByName("decrypt"), {}
        onEnter: function(args) {
          // Dump arguments
          send("Argument 1 of decrypt function" , args[0]);
          send("Argument 2 of decrypt function" , args[1]);
          [...]
        }
      });
    }
    \end{lstlisting}
    \caption{Frida script to dump arguments provided as input to the native method $decrypt$.}
    \label{fig:native-dump-argument-frida}
    \end{figure}
\end{itemize}
The access to the decryption key allows the attacker to decrypt any slice of ciphered code.
Furthermore, cumulative attacks can be performed to retrieve all the decrypted code using runtime memory dumping and process exploration. In this scenario, the attacker can dump each decrypted bytecode at runtime, thereby recovering the original code and she can leverage code manipulation (e.g., code deletion or binary patching) to add malicious code or remove anti-tampering controls. 

Once the code is recovered and tampered, one of the following approaches can be leveraged to create a working tampered $apk$ based on code deletion and binary patching:
\begin{itemize}
    \item override the body with the encrypted tampered code. This approach can be used only if a symmetric-key algorithm is used to encrypt and decrypt the code. In this way, once the attacker recovered the encryption key, she can perform both encryption and decryption.
    \item replace directly the body with the tampered code. In this scenario, the final app does not contains encrypted code.
\end{itemize}

\subsection{Stochastic Stealthy Networks} 
% Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/Repackage-proofing%20Android%20Apps%20~%20Stochastic%20Stealthy%20Network.pdf
% https://cse.sc.edu/~lluo/papers/ssn-robustness-2017.pdf, riassunto nel capitolo 2.1 di bombdroid

Several works \cite{Norboev2018OnTR, 10.1145/3168820, 10.1007/978-3-030-45371-8_12} have already pointed out some weaknesses of SSN, as well as some attacks that can be used to circumvent this protection. %\alessio{What I do not understand is whether we are reporting such already discussed attack in the following sentences, or we are reporting our attacks. } \antonio{both, we imagine (we cannot test them) some attacks that is confirmed by other papers}
 There are two ways to circumvent SSN, namely i) deactivating the integrity check or ii) detect and remove all the detection nodes from the code.

Concerning the first strategy, recall that each detection node implements the same integrity check on any candidate method, based on the developer's public key. Therefore, it is sufficient to analyze a single detection node to define a de-activation strategy. To this aim, code injection or vtable hijacking allow replacing the target method (\textit{getPublicKey} and \textit{generateCertificate}) with a custom implementation, which returns the original developer's public key, instead of the attacker's one. % which repackaged the app. %In this way we overcame all integrity checks.

Regarding the latter strategy, blackbox fuzzing can be used to generate a massive number of pseudo-random input in order to trigger all repackaging detection nodes (which are invoked stochastically) to detect them. In addition, whitebox fuzzing (or symbolic execution) can reveal the destination of the reflection calls.
Once all detection nodes are detected, either code deletion (i.e., to remove the repackaging detection nodes) or binary patching (i.e., to make the repackaging detection node unreachable) can be leveraged.

\subsection{AppIS: Protect Android Apps Against Runtime Repackaging Attacks}
%Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/AppIS-%20Protect%20Android%20Apps%20Against%20Runtime%20Repackaging%20Attacks%20-%20ICPADS_2017.pdf
The simplest way to repack an AppIS-protected app is to modify only parts (methods, resources or data), which are not protected by guards. It is possible to recognize whether an app snippet is protected through static analysis, as no code obfuscation is applied by AppIS.
Static analysis also allows obtaining the set of guarding nets, and delete them from the code. This is made possible by the fact that each guard has a specific design pattern %\alessio{which one? Can we say something about it? As we do not say anything on this in Section 3.} \antonio{authors do not specify how to implements the guard, but only a guarding net from a general point of view} 
 which the attacker can detect through bytecode analysis. In future works, the authors put forward the possibility to encrypt the set of guarding nets and decrypt it at runtime. Nonetheless, the encrypted guarding nets would be likewise vulnerable to deletion attack, as it is sufficient for the attacker to remove the parts of code where the decryption is carried out.
%Once we have been careful to remove the deleted guards from the guard-net generation at runtime, repackaging can be performed. 

Beyond removing guarding nets, it is also possible to bypass the integrity detection on the goals, by exploiting cumulative attacks to collect a large number of the original hash values. Then, such values can be hardcoded in the corresponding integrity detection methods. In this way, the attacker is able to bypass the anti-tampering controls without deleting the guarding nodes. 

\subsection{Self-Defending Code through Information Asymmetry}
% Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Other%20Anti-Repack%20techniques/Leveraging%20Information%20Asymmetry%20to%0ATransform%20Android%20Apps%20into%20Self-Defending%0ACode%20Against%20Repackaging%20Attacks.pdf
Recall that this approach is an improvement of the previous one: it moves the integrity checks to the native code and uses cryptographic obfuscation to resist static analysis.
Nonetheless, it remains vulnerable to several dynamic analysis techniques: first, blackbox fuzzing allows triggering a large number of SDC segments. For each triggered segment, a code instrumentation tool like Frida can be leveraged to hook the \texttt{encrypt} function in the \texttt{if} statement in order to recover the correct value of the variable \texttt{v}. 
%\antonio{1) blackbox fuzzing allow to trigger a lot of SDC segment 2) While the app is blackbox fuzzed, a code instrumentation tool can hook the decrypt function -> attack = blackbox (or other techniques to run the app with a lot of input, such as monkey) + code instrumentation (e.g. frida)} 
 Once this data is obtained, it is possible to retrieve the decryption key of the encrypted code, in both modes supported by this anti-repackaging technique. Then, code deletion can be leveraged to substitute an SDC segment with the original code, thereby deactivating the protection.
Previous attacks succeed only if all SDC sufficient for repackaging succesfully are discovered. %\luigi{In realtà ha successo solo se sono trovate tutte le sdc che ci permettono di raggiungere il nostro scopo (se la app si rompe dopo chissene frega)} 
Therefore, the robustness of this anti-repackaging technique is directly dependent on the number and the distribution of SDC statements in the app.

Finally, if the attacker is able to locate the checksum method in the native code (the anti-tampering control), she would override the body of such method through binary patching, in order to force it returning the excepted value. In this way, we would be able to tamper an application and bypass all checks with low effort. 

\subsection{BombDroid: Decentralized Repackaging Detection through Logic Bombs} \label{subsec:attack-bombdroid}
% Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/Resilient%20Decentralized%20Android%20Application%20Repackaging%20Detection%20Using%20Logic%20Bombs%20-%20CGO%202018.pdf
In BombDroid, any logic bomb follows the same, well-defined, specific pattern (i.e., \longstring{hash(v)==const}). Text search and pattern matching can be used to statically analyze the app source according to this pattern, in order to locate potential pieces of codes hiding logic bombs. However, code obfuscation could complicate this pattern-based search.
%\alessio{Could we have some problem with obfuscated apps?} \antonio{yes, obfuscation can limit static binary analysis}

Once a potential logic bomb is detected, the attacker can try to retrieve the decryption key (which is the constant value of the qualified condition) through dynamic analysis by leveraging:
\begin{itemize}
    \item \textbf{Brute force}: The attacker can try all possible values for the integer value \texttt{v}. Potentially, this key space is huge (i.e., \texttt{$2^{32}$}, as Java stores integer values in 4 bytes). Nonetheless, the actual distribution of valid constant values is smaller \cite{repackaging-protection}. Furthermore, there is a small number of unique constant values (i.e., in the range [-1024, 1024], according to the authors). %\alessio{I don't get the point clearly, what does it mean in practice? How much small?}. \antonio{From NRP paper, most of constant value are in range [-1024, 1024] and an attacker can easily use brute force to guess the value of the trigger condition. Moreover, exists significant value for constants (e.g. 0x0 is a null variable)}
    \item \textbf{Extraction of information from open source code}: If an app includes external open source libraries, and the static analysis recognize some potential logic bombs on such libraries, then an analysis of the original source code can allow guessing the right constant value of  \texttt{v}. 
    \item \textbf{Code instrumentation}: Proper code instrumentation applied on the potential logic bombs can allow intercepting the call to the decryption function (e.g., AES), thereby recovering the decryption key or the plain code (once the logic bomb has been triggered). 
\end{itemize}

Another way to retrieve the value of \texttt{v} is by means of cumulative attacks. In fact, as authors showed that at most 9.3\% of bombs are triggered using both state of the art Android fuzzing tools and human analysis, the detection and de-activation of such few logic bombs can suffice to obtain a repackaged app that works properly in the most of the cases. Put another way, this fact indicates that albeit BombDroid can add a lot of logic bombs, only few of them actually trigger.  Therefore, it is unnecessary for an attacker to delete each logic bomb, but she needs to remove just the mostly triggered ones on average.

Once a constant value is retrieved from a single-trigger bomb, the logic bomb could be deleted (i.e., deletion attack) and replaced directly with the (original) decrypted code. The attacker can also add some extra code to the original one.
It is worth noticing that the previous attacking procedure applies on nested bombs if all constant values (i.e., contained in all nested qualified conditions) are discovered. 

Another possibility is to bypass the anti-tampering checks contained in the encrypted code of the bomb (i.e., the \longstring{tampering\_detection} function in Figure \ref{fig:bombdroid-scheme}):
\begin{itemize}
    \item leverage code injection to replace the tampering detection function with an attacker-defined one;
    \item try a replay attack to modify the MANIFEST.MF file used in the code digest comparison checks. In this scenario, the anti-tampering controls compare the hardcoded values with the one in the original MANIFEST.MF file.
\end{itemize}

Recall that the BombDroid prototype relies on a tampering detection function based on a public-key comparison. Such function can be dynamically rewritten by instrumenting the Dalvik bytecode in order to return the expected value (i.e., the public-key of the original developer). %\alessio{I lost myself here: after rewriting (through which technique?) we force the function to provide what exactly as output? the public key of the original developer?} \antonio {yes, the hooked function return the original key that correspond to the expected value}
%Authors left the inclusion of other detection methods in future work.

\subsection{Native Repackaging Protection}
%Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/Repackaging_Protection__FPS_Paper%20-%202019.pdf
The Native Repackaging Protection is the most recent and advanced repackaging avoidance technique to date, as it inherits and extends methodologies and techniques from the other proposals. 
For previous anti-repackaging techniques, we have pinpointed some high-level attack patterns by leveraging the attacking techniques described in Section \ref{sec:attacking_model}, since no source code, nor any protected app have been made available. 
However, as the source code of NRP is publicly available, we were able to analyze it in detail and carry out an actual and full-fledged attack to this technique.
We will describe the attack in details by relying on a real app, i.e., Antimine~\cite{antimine-android}, an open source, minesweeper-like game app available on F-Droid (see Figure \ref{fig:antimine-fig}).

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\textwidth]{images/antimine.pdf}
    \caption{A snapshot of the Antimine game.}
    \label{fig:antimine-fig}
\end{figure}


More specifically, we will i) apply NRP to Antimine, showing how a candidate method is protected, ii) prove how such protection can be circumvented and iii) build a full-working repackaged version of the protected Antimine app. 

%e have the tool source code. An attacker could not have access to it, anyway it’s just a more time consuming process to exploit this approach.
%We ... For our test examples we will use .

As a preliminary remark, we found an implementation bug by analyzing the NRP source code: the tool statically pre-computes the signature of the \longstring{classes.dex} file through a Java function, while at runtime the protected app calculates this value by means of a native function (C/C++ code). The \texttt{char} type in standard C can either be signed [-128, +127] or unsigned [0, 255]. We found that the native function uses a char (line 3 on the left side of Figure \ref{fig:hash_bytes}) while the corresponding Java function adopts an unsigned char  (line 4 on the right side of Figure \ref{fig:hash_bytes}). As a consequence, a char value that has a bit representation with a \texttt{1*******} pattern (where \texttt{*} stands for 0 or 1) is interpreted as an int value between [-128,-1] by C and between [127,255] by Java. % (line 4 on the right side of Figure \ref{fig:hash_bytes}).
Therefore, if some chars of the \longstring{classes.dex} file have the \texttt{1*******} format, the integrity check always fails
- independently from the app being tampered or not. % - thereby leading the protected app to crash. %\alessio{Where does this inconsistency lead to? Explain.} \antonio{char value that has a bit representation 1******* (where * stands for 0 or 1) are interpreted as int value between [-127,-1] by C and between [127,255] by Java. Due to this, if some char of classes.dex match this form (1*******) then the integrity checks never pass (even without tampering) and the protected app always crash}

\begin{figure}
.
\begin{minipage}[t]{0.48\textwidth}
\begin{lstlisting}[language=C,
    basicstyle=\scriptsize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
    emphstyle=\underline,
    escapechar=ä,
]
// XOR in native code
int32_t hash_bytes(const char *arr, size_t count) {
  ä\underline{char hash[4];}ä// <-- Should be u_char
  for(size_t read = 0; read < count; read++) {
    hash[read % 4] ^= arr[read];
  }
  return hash[0] + (hash[1] << 8) + (hash[2] << 16) + (hash[3] << 24);
}
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{.48\textwidth}

\begin{lstlisting}[language=Java,
    basicstyle=\scriptsize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
    emphstyle=\underline,
    escapechar=ä,
]
// XOR in Java code
private static int xorFile(Path p, int count, int offset) throws IOException {
  byte[] content = Files.readAllBytes(p);
  ä\underline{byte[] res = new byte[4];}ä
  for(int i = offset; i < (offset + count); i++ ) {
    res[(i - offset) % 4] ^= content[i];
  }
  return (0xff & res[0]) + ((0xff & res[1]) << 8) +
    ((0xff & res[2]) << 16) + ((0xff & res[3]) << 24);
}
\end{lstlisting}
\end{minipage}
\caption{On the left side: the C code used to calculate the hash sum at runtime. On the right side, the Java code used to precompute the hash sum, at compile-time.}
\label{fig:hash_bytes}
\end{figure}

Moreover, the translation of the Java bytecode into native code could introduce some new exception. For instance, any single instruction in the Java bytecode influence, or is influenced, by other instructions (for example the comparison between two variables). It is mandatory to manage this mutual relationship, and the program must behave soundly even if some instructions are executed under the native environment. We argue that this is a non-trivial and error-prone task, as no automatic tool currently exists to translate Java bytecode to native on Android. %\alessio{sentence rewritten. Please check.} 
Furthermore, NRP suffers from the same limitations of BombDroid, related to the use of hash functions to hide the decryption key. If a logic bomb is inserted in an  \texttt{if} statement with a small hash space, it could be rather quick to recover the decryption key by brute force. As the authors discuss, NRP suffers from this limitation, as most of the constant values in an $apk$ are in the interval [-1024, 1024]. Finally, and differently from BombDroid, the hash function in NRP is not salted. As a consequence, whenever a decryption key is recovered, it is possible to statically detect all logic bombs that have the same key by only comparing the hash values. In fact, if two candidate conditions have the same constant value (e.g., \texttt{if(a == 1) {...}} and \texttt{if (b == 1){...}}, the hardcoded values in the trigger condition are likewise the same (i.e., \texttt{if(hash(a) == 'xyz')} and \texttt{if(hash(b) == 'xyz')},  since no salt is used. 
%\alessio{I will explain it better. Why is this possible statically?} \antonio{if there is two candidate condition if(a == 1)\{...\} and if(b == 1)\{...\}, the hard-coded values are equals in both trigger condition (i.e. if(hash(a) == hash(1)) and if(hash(b) == 'hash(b)) ) because no salt is used.} % Therefore, if an attacker recovers the key of a candidate condition, she is able to find all logic bombs whose triggering condition has the same key = 1, by looking for the value \texttt{hash(1)} in the code.

\subsubsection{Protecting Antimine with NRP}

We applied NRP to Antimine: the process lead to the insertion of $315$ logic bombs. For the sake of explanation, we focus on a single protected candidate method, namely the \texttt{setButton()} one. This method is invoked each time the user clicks on a blind button in the minesweeper game, and changes the look and feel of the button and its neighbors, as well as the message to prompt to the user, according to the rule of the game (see Figure \ref{fig:antimine-fig}). As this method makes decisions, it contains several qualified conditions (e.g., \texttt{var == -1}). 


% shows the result of NRP applied to a candidate condition found in $setButton$ method of $androidx.appcompat.app.AlertController$ class. \alessio{I assume that the set button is the code responsible for the look and feel of the button representing a cell in the minesweeper game. Am I right?} \antonio{yes. Precisely this function is part of the androidx library (see https://developer.android.com/reference/androidx/appcompat/app/AlertDialog\#setButton(int,\%20java.lang.CharSequence,\%20android.graphics.drawable.Drawable,\%20android.content.DialogInterface.OnClickListener)).} 

\begin{figure}
  \includegraphics[width=1.1\textwidth]{figs/native-bombdroid-evolution-example.pdf}
  \caption{NRP applied to the \texttt{setButton()} method of Antimine.}
  \label{fig:native-bombdroid-evolution-example}
\end{figure}

Figure \ref{fig:native-bombdroid-evolution-example} describes the actual protection workflow, step-by-step. First, NRP parses the \texttt{classes.dex} file (Step 2.2) and selects all methods with at least a qualified condition as candidate methods (Step 2.3). NRP adds a logic bomb in any candidate methods and for each qualified condition. Concerning the \texttt{setButton()} method, it selects the condition \texttt{var == -1} and splits the original code of the corresponding block into two parts, namely \texttt{or\_code1} and \texttt{or\_code2}. 
In Step 2.4, NRP builds up the logic bomb by i) rewriting the if block in the candidate method, and ii) distributing the logic of the bomb among two encrypted files, namely a Java class (i.e., \texttt{encr\_cl.dex}) and a native C/C++ library (i.e., \texttt{nat\_encr.so}). Concerning the first point, the qualified condition is translated into a Boolean variable (i.e., \texttt{resultMatch}), whose value is calculated by comparing the \texttt{var} value with the hash of \texttt{-1} encoded as a byte array. In case the value of \texttt{resultMatch} is true, the block executes a \texttt{decryptAndInvokeMain(\ldots)} method. Such method takes as input the actual name of the encrypted Java class (i.e., \texttt{className = AlertController\_setButton...}), its binary representation (i.e., \texttt{cipherCode}, which is contained in the block), as well as the value of \texttt{var} and and the array of arguments (i.e., \texttt{args}) required by the main method of the encrypted Java class to execute properly. 
The invocation of such method leads to the decryption of \texttt{cipherCode}, using the value of \texttt{var} as decryption key, and to the execution of the main method of the class \texttt{AlertController...}. The main method contains the \texttt{native\_key} to decipher the native library (i.e., \texttt{nat\_encr.so}), a JNI call and the second part of the original block code (i.e., \texttt{or\_code2}). The JNI call triggers the execution of a deciphering function in the native library (i.e., \longstring{Java\_embedded\_native\_androidxappcompat(\ldots)}, which i) retrieves the encrypted native code from a memory location, ii) decrypts it using the \texttt{native\_key}, and iii) launches the execution of the decrypted function. This latter function (i.e., \longstring{Java\_embedded\_native\_androidxappcompat[\ldots]\_KEY(\ldots)}) contains the anti-tampering check (i.e., \texttt{hash\_file\_in\_apk(\ldots)}) that verifies the integrity of the first 100 bytes of the \texttt{classes.dex} file. If the integrity is verified, the function executes the first part of the original block code (i.e., \texttt{or\_code1}). Finally, the JNI call terminates and the main method in the Java class executes the last part of the original block (i.e., \texttt{or\_code2}).   

\subsubsection{Dismantling NRP bombs}
The attacker has to bypass the integrity checks performed by the protected app in the \longstring{Java\_embedded\_native\_androidxappcompat[\ldots]\_KEY(\ldots)} function to dismantle the NRP logic bombs.
To achieve such result, the attacker can either i) override \texttt{encr\_cl.dex} or \texttt{nat\_encr.so} for all the triggered logic bombs, by leveraging code deletion and binary patching, or ii) bypass the integrity check performed by the native code, by relying on a replay attack.

\paragraph{Bytecode and Native Code Overriding:}
The attacker can instrument the code to intercept the invocations to the \textsl{decryption functions} both in the Java and the native code, in order to retrieve i) the encrypted code and the decryption key passed as argument to the function, and ii) the decrypted code at the end of that function. Code instrumentation can also be used to change the implementation (or just the return value) of the tamper check function in the native code.

The Java decryption method requires two input values, namely the encrypted code (\texttt{param2}) and the decryption key (\texttt{param1}), and returns the decrypted code. % \alessio{not sure to leave or embed this sentence in other sentences.}
Figure \ref{fig:linear-dump-frida} shows the Frida script that instruments the Java decryption method (i.e., \texttt{SDCloaderr.decryptAndInvoke(\ldots))}
%\alessio{There is a lack of precision here. Till now, we threated this method as double, where both decryption and invocation are executed. Nonetheless, it seems here that the Frida script only focuses on decryption. Do you mean that you instrumented just a - the decryption - part of such method? We must clarify.} \antonio{Frida can be use in both scenarios. For example, if we intercept the invokation of the InMeryDexClassLoader we can retrive the bytes of the decrypted dex that we are going to load into memory. Alternatively, we can hook/intercept directly the invocation of the integrity check function in order to change the returned value and pass the check. In this case (bytecode overriding), we are interested to retrieve both the encryption/decryption key and the decrypted bytes of the dex (or native code) that we are going to call. For this purpose, we identified the hook of the decryption function (both in Java and C code) as the most useful technique. Moreover, we can intercept the invokation of the decrypted function for other purposes, such as change input parameter or return value}
for a given encrypted code \texttt{encr\_cl}, represented by \texttt{ciphered\_byte} (i.e., the \texttt{cipherCode} byte array in the \texttt{setButton} method), that we will analyze using Jadx \cite{Jadx}). 
The script begins by selecting (lines 1 and 2) the class (i.e.,  \longstring{embedded.SDCLoader}) and the decryption method (i.e., \texttt{decrypt}) to overload. Frida hooks at the start of the overloaded function and executes the customized code (lines 3 to 19) instead of the original code.
The customized code calls the original Java \texttt{decrypt} method (line 6) and stores the returned value in a variable. Since the attacker's aim is to get access to a specific decrypted function, the script (lines 7-13) compares the encrypted method passed as the input parameter \texttt{param2} with \texttt{ciphered\_bytes}. If the decryption function is correct, the script writes down the decrypted bytecode (line 16). It is worth noticing that the script also dumps the key inside the \texttt{param1} variable. The return value of the overloaded function is the return value of the original decryption function (line 19).


\begin{figure}[!htbp]
\begin{lstlisting}[language=Java,
    basicstyle=\scriptsize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
var SDCLoader = Java.use("embedded.SDCLoader");
SDCLoader.decrypt.overload("[B", "[B").implementation = function(param1, param2) {
  var arr_bytes = Java.array('byte', param2);
  var ciphered_bytes = [107, 30, -22 [..] 18];
  var found = true;
  var dexBytesDecrypted = this.decrypt(param1, param2);
  if(arr_bytes.length == ciphered_bytes.length) {
  	for(var i = 0; i < ciphered_bytes.length; i++) {
  	  if(ciphered_bytes[i] != arr_bytes[i]){
  	    found = false;
  		break;
  	  }
  	}
    if (found) {
  	  console.log("### FOUND");
  	  // Write to file dexBytesDecrypted
    }
  }
  return dexBytesDecrypted;
}
\end{lstlisting}
\caption{Frida script to dump the result of decrypted function.}
\label{fig:linear-dump-frida}
\end{figure}

Concerning the native decryption function, it can be reversed using a decompiler (i.e., Ghidra \cite{ghidra}), and analyzed to detect the decryption function, and to infer the decryption logic (e.g., it is possible to analyze the body of the \texttt{Java\_embedded\_native\_androidxappcompat[...]} function). 
Here, the \texttt{decrypt\_code} function is responsible for decrypting $n$ bytes of machine code starting from a pointer to the memory. Such function can be overloaded and dumped through the scripts described in Figure \ref{fig:native-dump-frida} and Figure \ref{fig:native-dump-frida2}, which allow retrieving both the plain code and the key, as in the case of the Java decryption function. 
%\autoref{fig:native-dump-frida} shows the Frida script that we used to intercept the call to $decrypt\_code$ function and dump the bytes decrypted from memory.
%In this case we want to overload a native function instead of a Java function. 
In detail, the script in Figure \ref{fig:native-dump-frida} aims to detect the location in which the target function to dump will be decrypted and executed. It starts by retrieving the \texttt{libnative-lib.so} (line 2) - which is the shared object containing all native functions implemented by NRP and then it enumerates each function therein (lines 6-10) to detect the \texttt{decrypt\_code} functions. Then, the script sets up an interceptor for the function (line 13). Whenever a \texttt{decrypt\_code} function executes, the script verifies whether the decryption function is the expected one (lines 14-30), by comparing the key passed as a parameter to the \texttt{native\_key} hardcoded in the \texttt{encr\_cl.dex} file. 
If this is the case, the script invokes the \texttt{AES\_CTR\_xcrypt\_buffer} function that decrypts the code, write the plain machine code in a writable page, and makes it executable. More specifically, the script in Figure \ref{fig:native-dump-frida2} attaches Frida to the \texttt{AES\_CTR\_xcrypt\_buffer} function (lines 5-14). Then, when the function starts (i.e., OnEnter, lines 15-18), the script retrieves the memory address (i.e., \texttt{args[1]}) and the size (i.e., \texttt{args[2]}) of the write buffer for the code. After the decryption phase terminates (i.e., OnLeave (from line 19 to line 24), the script checks whether the decrypted code is correct (line 20): in case, the script retrieves the pointer to the starting address (line 21) and dumps \texttt{len} bytes (lines 22-24).

\begin{figure}[!htbp]
\begin{lstlisting}[language=Java,
    basicstyle=\scriptsize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
function inspectModule(module) {
  var m = Process.getModuleByName(module);
  var targetFunction = true;
  var functionToBeIntercepted = "";
  var exports = m.enumerateExports();
  exports.forEach(function(exp){
    if (exp.name.indexOf("decrypt_code")>=0){
      functionToBeIntercepted = exp.name; 
    }
  });

  // Intercept decrypt_code function
  Interceptor.attach(m.getExportByName(functionToBeIntercepted), {
    onEnter: function(args) {
      var pointer = new NativePointer(args[2]);
      var buff = pointer.readByteArray(16);
      buff = new Int8Array(buff);
      var key = [-63, [...], -9]; // native_key hardcoded in encr_cl.dex
      targetFunction = true;
      for(var i = 0; i < buff.length; ++i){
        if(buff[i] != key[i]){
          targetFunction = false;
          break;
        } 
      }
      if(targetFunction) {
	    console.log("##### FOUND");
      } 
    }
  });

  // Intercept AES_CTR_xcrypt_buffer function
  [...]
}
\end{lstlisting}
\caption{Frida script that searches for the target \texttt{decrypt\_code} function.}
\label{fig:native-dump-frida}
\end{figure}

\begin{figure}[!htbp]
\begin{lstlisting}[language=Java,
    basicstyle=\scriptsize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
function inspectModule(module) {
  [...]
  // Intercept AES_CTR_xcrypt_buffer function
  // Dump the return bytes
  functionToBeIntercepted = "";
  exports = m.enumerateExports();
  exports.forEach(function(exp){
    if (exp.name.indexOf("AES_CTR_xcrypt_buffer")>=0){
      functionToBeIntercepted = exp.name; 
    }
  });
  var outAddr = "";
  var len = 0;
  Interceptor.attach(m.getExportByName(functionToBeIntercepted), {}
    onEnter: function(args) {
      outAddr= args[1];
      len = parseInt(args[2]);
    },
    onLeave: function(retval) {
      if(targetFunction) {
        var pointer = new NativePointer(outAddr);
        var buff = pointer.readByteArray(len);
        // DUMP buff
        send("Readed byte", buff);
      }
    }
  });
}
\end{lstlisting}
\caption{Frida script that dumps the assembly code decrypted by the native function.}
\label{fig:native-dump-frida2}
\end{figure}

\newpage

The decrypted code is a hex string that encodes the x86 assembly instructions. Such instructions can be extracted using a disassembler. 
The analysis of the disassembled instructions allows detecting a hardcoded tamper check on the \texttt{classes.dex} file 
%\begin{lstlisting}[language=c]
\begin{center}
    \texttt{cmp eax, 0xb543c475}
\end{center}
%\end{lstlisting}
where \texttt{$0xb543c475$} is the checksum of the original \texttt{classes.dex} file of Antimine.

Once the original codes and the decryption keys are recovered, an attacker can easily bypass the tamper check by overriding the hardcoded value with the one of the repackaged app, and then re-encrypting the assembly code and substituting the original code in the $.so$ file. As an alternative, the attacker can modify the decrypted \texttt{nat\_enc.so} and the \texttt{encr\_cl.dex} to execute \texttt{op\_code1} in Java rather than in the native code, and remove the JNI call that would trigger the tamper check.  

\begin{figure}[!htbp]
  \includegraphics[width=\textwidth]{figs/sochanged.jpg}
  \caption{The original (top side) and the tampered (bottom side) library file.}
  \label{fig:sochanged}
\end{figure}

\paragraph{Bypass the integrity check:}
An alternative attack to bypass the tamper check is to leverage a reply attack by modifying the file on which the tamper check is executed. This attack can be carried out since the path of the checked file is hardcoded in the native library in clear text. 

We carried out this attack as follows: we added a new file (i.e., \texttt{cla.dex}) to the $apk$, that has the same content of the original \texttt{classes.dex} of Antimine. Then, we manually patched the hardcoded path in the \texttt{elf} file to point to \texttt{cla.dex} instead of the \texttt{classes.dex} which is modified by the attacker before repackaging. In this way, the tamper check passes as it calculates the expected value, despite the app content has been modified. Figure \ref{fig:sochanged} shows the original library (top side), and the tampered one (bottom side) in which the hardcoded path is modified to point to $cla.dex$.

Previous attacks allowed to successfully bypass the NRP protection on Antimine. The repackaged version of Antimine, with all the 315 bombs de-activated, is available at:
\begin{center}
\url{https://www.csec.it/projects/antimine-800011-protected-and-repacked.apk} \\
\end{center}
for further studies, analysis and testing activities. 

%\paragraph{Conclusion}
%This attacks are based on the fact that code instrumentation have no effect on the $classes.dex$ file and the anti\-tampering controls are not influenced by this attack.

%Contrary to Bombdroid, once the machine code is retrieved, it is harder to completely remove the logic bomb due to it is implemented in native code. This was not a problem because we could still bypass the AT checks (as we see above) and add anyway the malicious code.

\begin{comment}
Some useful code
\begin{figure}[!htbp]
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
public void setButton(int i, CharSequence charSequence,
DialogInterface.OnClickListener onClickListener,
Message message, Drawable drawable) {
  if (message == null && onClickListener != null) {
    message = this.mHandler.obtainMessage(i, onClickListener);
  }
  if (i == -3) {
    this.mButtonNeutralText = charSequence;
    this.mButtonNeutralMessage = message;
    this.mButtonNeutralIcon = drawable;
  } else if (i == -2) {
    this.mButtonNegativeText = charSequence;
    this.mButtonNegativeMessage = message;
    this.mButtonNegativeIcon = drawable;
  } else if (i == -1) {
    this.mButtonPositiveText = charSequence;
    this.mButtonPositiveMessage = message;
    this.mButtonPositiveIcon = drawable;
  } else {
    throw new IllegalArgumentException("Button does not exist");
  }
}
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{.45\textwidth}
\begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
public void setButton(int i, CharSequence $r3,
DialogInterface.OnClickListener onClickListener,
Message $r2, Drawable $r1) {
  if ($r2 == null && onClickListener != null) {
    $r2 = this.mHandler.obtainMessage(i, onClickListener);
  }
  if (i == -3) {
    this.mButtonNeutralText = $r3;
    this.mButtonNeutralMessage = $r2;
    this.mButtonNeutralIcon = $r1;
  } else if (i != -2) {
    Integer $r7 = Integer.valueOf(i);
    boolean $z0 = SDCLoader.match($r7, new byte[]{-39, -66, 101, 36, -91, -11, 4, 125, -75, -122, 104, 19, -84, -13, 39, 120, -110, -89, -93,10});
    byte[] $r10 = {107, 30, -22 [...] 18};
    Object[] $r12 = {this, $r2, $r1, $r3};
    if ($z0) {
      ResultWrapper $r9 = SDCLoader.decryptAndInvokeMain("androidx.appcompat.app.AlertController_setButton_1fa3710f-3cce-4365-8c84-811bf490e68d", $r10, $r7, $r12);
      int $i1 = $r9.jumpTarget;
      if ($i1 != -1) {
        Object[] $r13 = $r9.savedPrimitivesAndReferences;
        AlertController alertController = (AlertController) $r13[0];
        Message $r22 = (Message) $r13[1];
        Drawable drawable = (Drawable) $r13[2];
        CharSequence charSequence = (CharSequence) $r13[3];
        if ($i1 != -2) {}
      } else {
        return;
      }
    }
    throw new IllegalArgumentException("Button does not exist");
  } else {
    this.mButtonNegativeText = $r3;
    this.mButtonNegativeMessage = $r2;
    this.mButtonNegativeIcon = $r1;
  }
}
\end{lstlisting}
\end{minipage}
\caption{On the left side the original code. On the right side the protected method.}
\label{fig:if-protected}
\end{figure}
\clearpage

\begin{figure}[!htbp]
\begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
var SDCLoader = Java.use("embedded.SDCLoader");
SDCLoader.decrypt.overload("[B", "[B").implementation = function(param1, param2) {
  var arr_bytes = Java.array('byte', arr2);
  // Ciphered "androidx.appcompat.widget.LinearLayoutCompat_" 
  // "measureHorizontal_1a173610-a602-41f6-a1e5-6133fbbd9903" method
  var ciphered_bytes = [88, 23, -64, 30, 122, 57,[..], -114];
  var found = true;
  var dexBytesDecrypted = this.decrypt(param1, param2);
  if(arr_bytes.length == ciphered_bytes.length) {
  	for(var i = 0; i < ciphered_bytes.length; i++) {
  	  if(ciphered_bytes[i] != arr_bytes[i]){
  	    found = false;
  		break;
  	  }
  	}
    if (found) {
  	  console.log("### FOUND");
  	  // Write to file
    }
  }
  return dexBytesDecrypted;
}
\end{lstlisting}
\caption{Frida script to dump  $androidx.appcompat.widget.LinearLayoutCompat_measureHorizontal_1a173610-a602-41f6-a1e5-6133fbbd9903$ decrypted function.}
\label{fig:linear-dump-frida}
\end{figure}

\begin{figure}[!htbp]
\begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
public class LinearLayoutCompat_measureHorizontal_1a173610a60241f6a1e56133fbbd9903 {
  public static ResultWrapper main(boolean z, boolean z2) {
    native.androidxappcompatwidgetLinearLayoutCompatmeasureHorizontal1a[...](
    new byte[]{-63, [...], -9});
    Object[] objArr = new Object[2];
    return new ResultWrapper(0, restoreLocals(true, true));
  }

  public static Object[] restoreLocals(boolean z, boolean z2) {
    return new Object[]{Boolean.valueOf(z), Boolean.valueOf(z2)};
  }
}
\end{lstlisting}
\caption{The decrypted  $androidx.appcompat.widget.LinearLayoutCompat_measureHorizontal_1a173610-a602-41f6-a1e5-6133fbbd9903$ method.}
\label{fig:linear-dumped}
\end{figure}

\begin{figure}[!htbp]
\begin{lstlisting}[language=C,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
void Java_embedded_native_androidxappcompatwidgetLinearLayoutCompatmeasureHorizontal1a173610a60241f6a1e56133fbbd9903 (JNIEnv *env,jbyteArray jni_decryption_key)
{
  char decrypted;
  int iVar1;
  uchar *key;
  jbyteArray in_RDX;
  char *pcVar2;
  if (decrypted == '\0') {
    key = (uchar *)(*env->functions->GetByteArrayElements)((JNIEnv*)env,in_RDX,(jboolean *)0x0);
    iVar1 = decrypt_code(Java_embedded_native_android[...],0xa0,key);
    pcVar2 = "DECRYPT: FAIL";
    if (iVar1 == 0) {
      pcVar2 = "DECRYPT: Success";
    }
    (*env->functions->ReleaseByteArrayElements)((JNIEnv *)env, in_RDX,(jbyte *)key,2);
    decrypted = '\x01';
    pcVar2 = "Entering decrypted segment...";
  }
  else {
    pcVar2 = "Code already decrypted. Jumping to decrypted code!\n";
  }
  _DAT_ef2f54c83f3bec25 = (int)register0x00000020 + -4;
  return;
}
\end{lstlisting}
\caption{Native function inside the .so library.}
\label{fig:linear-native}
\end{figure}

\begin{figure}[!htbp]
\begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
function inspectModule(module) {
  var m = Process.getModuleByName(module);
  var targetFunction = true;
  var functionToBeIntercepted = "";
  var exports = m.enumerateExports();
  exports.forEach(function(exp){
    if (exp.name.indexOf("decrypt_code")>=0){
      functionToBeIntercepted = exp.name; 
    }
  });

  // Intercept decrypt_code function
  Interceptor.attach(m.getExportByName(functionToBeIntercepted), {
    onEnter: function(args) {
      var pointer = new NativePointer(args[2]);
      var buff = pointer.readByteArray(16);
      buff = new Int8Array(buff);
      // our method key
      var key = [-63, [...], -9];
      targetFunction = true;
      for(var i = 0; i < buff.length; ++i){
	    if(buff[i] != key[i]){
	      targetFunction = false;
	      break;
	    } 
	  }
	  if(targetFunction) {
	    console.log("##### FOUND");
	  } 
    }
  });

  // Intercept AES_CTR_xcrypt_buffer function
  // Dump the return bytes
  functionToBeIntercepted = "";
  exports = m.enumerateExports();
  exports.forEach(function(exp){
    if (exp.name.indexOf("AES_CTR_xcrypt_buffer")>=0){
      functionToBeIntercepted = exp.name; 
    }
  });
  var outAddr = "";
  var len = 0;
  Interceptor.attach(m.getExportByName(functionToBeIntercepted), {}
    onEnter: function(args) {
      outAddr= args[1];
      len = parseInt(args[2]);
    },
    onLeave: function(retval) {
      if(targetFunction) {
        var pointer = new NativePointer(outAddr);
        var buff = pointer.readByteArray(len);
        // DUMP buff
        send("Readed byte", buff);
      }
    }
  });
}
\end{lstlisting}
\caption{Frida script to dump native function decrypted bytecode.}
\label{fig:native-dump-frida}
\end{figure}

\begin{figure}[!ht]
\begin{lstlisting}[language=C,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
static bool alreadyChecked;
static bool passed;
if(!didCheck){
  if(0x5d434c4a == hash_file_in_apk("classes.dex", 100)){
	passed = true;
  } else {
	passed = false;
  }
  alreadyChecked = true;
}
if(passed) {
  // exec code
} 
\end{lstlisting}
\caption{Native function decrypted and decompiled from bytecode.}
\label{fig:native-flow}
\end{figure}

We are going to propose two different approaches to bypass the AT controls based on changing the hard-coded values in the so file.
In the first one, we inserted inside the apk a new file that has the same content of the \emph{classes.dex} and manually patched the hard-coded path in the elf file. In this way, the AT control computes the right value despite the app content has been modified. In fig \ref{fig:sochanged} we show the original library (top side), and the tampered one (bottom side). Inside the tamepred apk we inserted the $cla.dex$ file, that is the $classes.dex$ file taken from the protected app.
Beside this value, the expected hash value is hard-code inside the so file. Modify this value is more difficult because the code is ciphered. We intercepted the decrypted machine code we disassembled it to analyze its content. This snippet contains the expected value of the integrity check in an hard-coded way and an we were able to change this value with his desired one. 
Once the expected value is replaced, we re-encrypted the function and substitute it in the so file.

Contrary to Bombdroid, once the machine code is retrieved, it is harder to completely remove the logic bomb due to it is implemented in native code. This was not a problem because we could still bypass the AT checks (as we see above) and add anyway the malicious code.

\end{comment}

%\clearpage


%\paragraph{Example}
%\todo{metto qua gli esempi (in un paragrafo diverso) o li metto inline nel paragrafo security issues ?!}

==> [PMC] ARMAND Anti-Repackaging/sections/old paper files/attackingmodels.tex <==
\section{Attacking Anti-Repackaging} \label{sec:attacking_model}
In this section, we discuss the \textsl{weapon rack} of repackaging, i.e., the main set of techniques that an attacker can leverage to analyze a protected $apk$ in order to detect and dismantle anti-repackaging protections (Steps 8 and 9 in Figure \ref{fig:threat-model-design}). They can be divided in two main categories, namely \textsl{static} and \textsl{dynamic}. The first category refers to the set of techniques that analyze the $apk$ without executing it (static analysis), while the latter category is composed by techniques that apply to an $apk$ while executing on an actual or emulated Android device (dynamic analysis). 

On one hand, static analysis aims at systematically reverse engineering the $apk$ (e.g., White Box Reverse Engineering  ~\cite{mitre_white_box_reverse_engineering}) in order to reconstruct and analyze the original source code. There exist a lot of tools that support this type of analysis and help an attacker to decode, rebuild and inspect both the app code and the resources, such as apktool~\cite{apktool} and dex2jar~\cite{dex2jar}.
On the other hand, dynamic analysis aims at inferring the app behavior during execution, to retrieve, e.g., actual values of variables, and monitor the execution of the code. 

Static and dynamic analysis are complementary: the first aims at building a comprehensive model of the app behavior by systematically exploring all the code and the resources of the app; the latter focuses on inferring a model of the app behavior by repeatedly executing the app. In principle, the static model is a superset of all possible behaviors of the app, meaning that at runtime the app will exhibit only a subset of the behavior of the static model. The dynamic model is partial by definition (as it is impossible to stimulate all possible executions of the app at runtime) but contains only behaviors that the app actually exhibits. As a consequence, static analysis suffers from \textsl{false positives} (e.g., a statically detected behavior could not be executed at runtime), while dynamic analysis suffers from \textsl{false negatives} (a behavior which has not been recognized during the dynamic analysis phase could be assumed as non-existent). %\luigi{Anziché "is assumed", preferirei "could be assumed"}. 

Concerning anti-repackaging, static analysis aims to detect the pieces of code where logic bombs could potentially hide (e.g., blocks with hash values in the qualified condition), while dynamic analysis allows to check the actual triggering and execution of the bombs at runtime. Furthermore, the repeated execution of the app on several setups allows the attacker to carry out \textsl{cumulative attacks}~\cite{8368344}\footnote{See the AppIS approach in Section \ref{subsec:appis-2017}}.  
%Finally, static and dynamic analysis suffer from opposite features and weaknesses. Concerning features, static analysis is exhaustive, i.e., it allows to explore all code branches  and resources at once, and detect all potential bombs, while dynamic analysis allows to repeatedly execute the app many times to detect differences among execution (and carry out ). Weaknesses are directly related to the previous features: static analysis suffers from false positives,  (i.e., pieces of original code with a qualified condition with hash values can be wrongly recognized as potential bombs) while dynamic analysis is subject to false negatives (it detects bombs only when they are triggered; therefore, untriggered bombs are not recognized).
Within the ``try and error'' cycle, the attacker builds up an analysis workflow of the $apk$ which fruitfully combines static and dynamic analysis techniques.

Hereafter, we briefly introduce the main static and dynamic analysis techniques to detect anti-repackaging. %Table \alessio{Add table and reference.} summarizes...




%\begin{itemize}
 %   \item \textbf{Static analysis} i analysis of software that is performed without executing programs.
  %  This approach is possible because the current structure of an apk file could allow . In other words, an attacker could retrieve useful information and sensitive data inspecting files inside the apk.
        
   % \item \textbf{Dynamic analysis} is the investigation of software (in our case Android application) that is performed by executing programs on real or virtual devices. 
%    In particular, the main issue to mitigate is what is called : an attacker could, with enough time and resources, run n-times the same app to retrieve many information such as which calls are performed, where an app crashes, etc.
    
%\end{itemize}

\subsection{Text Search and Pattern Matching} \label{sec:text_search_and_pattern_matching}
This technique statically analyzes the decompiled $apk$ to detect keywords or expressions that may hide logic bombs. The search and detect phase relies on heuristics and regular expressions defined by the attacker herself, or on pre-defined patterns defined in static analysis tools that support this technique. For instance, this technique may allow recognizing explicit anti-tampering function calls, as well as qualified conditions containing hash values. As any other static analysis approach, all detected anti-tampering checks must be evaluated at runtime to filter true positives (i.e., the checks which actually hide some logic bombs). 

The efficacy of this technique is rather limited, as it can be easily circumvented by anti-repackaging techniques. For example, SSN and BombDroid~\cite{7579771, 10.1145/3168820} are resilient to this threat as they rely on Java reflection or obfuscation~\cite{Norboev2018OnTR}; the first allows hiding function calls inside the code, while the latter avoids text search as obfuscation modifies the syntax of the code (e.g., method renaming).

\subsection{Fuzzing}\label{sec:fuzzing}
Fuzzing is an automated testing technique that provides pseudo-random input to a running program. There exist three different types of approaches, namely:
\begin{itemize}
    \item \textbf{Blackbox fuzzing}: it generates input data without having any knowledge of the app code and structure \cite{10.1145/2491411.2491450};
    \item \textbf{Whitebox fuzzing}: it  is also known as \textsl{symbolic execution} \cite{10.1145/2382756.2382798, 4223228}
    and it applies to the app code, which is supposed to be accessible by the attacker. 
    The main goal of whitebox fuzzing is to provide input data which allows exploring as many execution paths as possible, in order to detect which data could match specific condition (e.g., the trigger of a logic bomb). Moreover, whitebox fuzzing could allow revealing the destination of a suspicious call executed through Java reflection. 
    From a technical standpoint, the main difference between blackbox and whitebox fuzzing is that the latter adopts a (symbolic) input which evolves according to the program analysis and to reach certain critical program location; the first one, instead, does not rely on the program structure. 
    \item \textbf{Graybox fuzzing}: this approach mixes blackbox and whitebox fuzzing, i.e., it generates symbolic input for the sole subpart of the program which is known to the attacker, while the unknown part of the app is stimulated according to blackbox fuzzing data generation.
\end{itemize}
Fuzzing is suitable for assessing an $apk$ protected with SSN or Bombdroid, as it allows to trigger (and detect) the bombs (repackaging detection nodes) or to perform analysis of hash values. However, these techniques do not grant a complete path exploration and a full input data coverage. Therefore, they cannot find and trigger all bombs~\cite{Norboev2018OnTR}. 

\subsection{Debugging and Code Emulation}\label{sec:debugging_and_code_emulation}
The most common way to deeply analyze the behavior of an app is to use a debugger. In the general case, a debugger allows a developer to dynamically test a software in order to find and resolve bugs. Concerning the attack to anti-repackaging, a debugger allows bypassing all static countermeasures like obfuscation, and understand how the app behaves at runtime.
More in detail, an attacker can intercept critical calls, find out repackaging detection and understand the type of anti-tampering checks.
However, debugging strongly relies on manual intervention, which has the drawback to scale badly, i.e., debugging an app to try tracing back all bombs has been proven to be unfeasbile~\cite{Norboev2018OnTR, 10.1145/3168820}.

In addition, the debuggable flag inside the app manifest file has to be set to true, in order to attach a debugger to an Android app. Developers that apply anti-repackaging techniques trivially set this flag to false. Therefore, an attacker should first modify the app manifest~\cite{owasp_mobile_security_testing_guide} and repackage it before debugging. This first repackaging step can itself trigger proper logic bombs in the app and make the execution of the app fail. 

An alternative to debugging is \textsl{code emulation} in \cite{180237, BHANDARI2017392}: %\alessio{Do we really need both references? why?}\luigi {Yes, because unlike debugging with code emulation the attacker can modify device behavior ie modify return values of system calls. In this way it is possible to explore more paths}
 the idea is that the target app is executed on some virtual machine, where the hardware, the Android OS and the Dalvik VM layers are replicated. During app execution, the virtual machine performs call tracing \cite{10.1145/1966445.1966460}. 
However, both approaches follow specific execution paths that depends on input data and could not reach the candidate methods in which logic bombs are hidden.

\subsection{Process Exploration}\label{sec:process_exploration}
\textsl{Process Exploration} refers to a set of techniques allowing the attacker to deeply inspect the app process memory at runtime~\cite{owasp_mobile_security_testing_guide}. There exists several tool to support memory exploration, most of which are Frida-based\footnote{We will discuss Frida in Section  \ref{subsec:code_instrumentation_and_code_injection}}, and rely on \textsl{dynamic code instrumentation}.
Currently, the most widespread tools are:
\begin{itemize}
    \item \textbf{Fridump}: an open source memory dumping tool for both Android and iOS ~\cite{fridump}. From a memory dump, it is possible to access to memory addresses where, for example, decryption key of anti-repackaging tools are stored at runtime;
    \item \textbf{Objection}: a runtime mobile exploration toolkit for both Android and iOS, that does not require a rooted device. Two interesting features of Objection are the ability to i) circumvent SSL pinning, i.e., a technique allowing apps to authenticate the server and avoid man-in-the-middle-attacks), and ii) dump and patch  memory locations~\cite{objection};
    \item \textbf{R2frida}: a tool that merges the reverse engineering capabilities of \textsl{radare2}~\cite{Radare} (a reverse engineering framework) with Frida (a dynamic instrumentation toolkit). In this way, an attacker can carry out runtime reverse engineering and memory related tasks, such as memory inspection~\cite{r2frida}.
\end{itemize}
The adoption of  such tools allows an attacker to analyze the runtime behavior of an app without debugging it (i.e., without the need to force the set of the debuggable flag to true and repackage.).

%Process exploration suffers from the lack of exhaustiveness of other dynamic tool. \alessio{maybe add a final sentence, but we see in the final version} \luigi{Maybe remove this last sentence}

\subsection{vtable Hijacking}\label{sec:vtable_hijacking}
In Java, a virtual table (vtable) dynamically maps function calls, i.e., a Java object points to some records of the vtable which contains the link to the actual method implementation. In Java, all methods are virtual by default, unless they are declared as \textsl{final} or \textsl{static}.
An attacker can modify the values in the vtable in order to invoke an arbitrary method and change the behavior of the original method. 
The limitation of this approach is that it works properly only on rooted devices, as the attacker needs root privileges to change the entries of the vtable~\cite{artdroid}.

An example of vtable hijacking is proposed in~\cite{7579771}: here, the vtable mapping is modified to redirect all invocation to the \emph{getPublicKey} method to a spoofed function which returns the public key of the original developer, instead of the public key of the attacker that repackaged the app. %\alessio{The sentence was unclear. I did my interpretation but it is pssibily wrong. Please explain here in detail how this work. }\luigi{The attacker repack the original app, and the public key obviously changes; the anti tampering control calls a getPublicKey method, the attacker modify the vTable in order that getPublicKey method points to a attacker-controlled method that return the original publicKey}

%, thereby bypassing the standard anti-repackaging check based on the user. As a consequence, any invocation of the  If an attacker has root privilege and changes the vtable’s entry related to \emph{getPublicKey}, he could bypass the anti repackaging controls (the app believes to call the right function, but calls the attackers one). 

%We assume the attacker has no access to users vtable ~\cite{Norboev2018OnTR, 10.1145/3168820}.\alessio{I do not understand which is the meaning of this assumption. Please explain.} \luigi{to modify the vTable the attacker should have root access in the user device, in this case the repackaging problem is meaningless for the user}
%However, this technique could be used by an attacker to bypass some checks in order to retrieve more information about the application.

\subsection{Code Manipulation}\label{subsec:code_manipulation}
There exist three main techniques to affect the app code in order to remove  anti-repackaging checks or to add malicious code, namely \textsl{code deletion}, \textsl{binary patching} and \textsl{code instrumentation and injection}. The first two techniques are static, while the latter is dynamic.

\paragraph{Code deletion:}\label{subsec:code_delection}
This technique aims at removing proper part of the app source code (if available), or smali code in order to deactivate specific controls. It can be partially circumvented: for instance, the anti-repackaging checks may be hosted in methods that cannot be straightforwardly removed, i.e., many other parts of the app depend on them. Alternatively, fake controls resembling logic bombs can be added in the code to fool the attacker which exploits code deletion \cite{10.1145/3168820}. In case the attacker remove them from the code, the app will not work properly.

\paragraph{Binary patching:}\label{paragraph:binary_patching}
It refers to the process of modifying a compiled executable to change its behavior. Differently from code deletion, binary patching does not need to retrieve or reconstruct the app source code, and it is, for instance, independent from code obfuscation.
It is worth pointing out that it is far easier and more reliable to apply binary patching  to Java than native code (e.g., C, C++, \ldots). Therefore, this technique is promising for an attacker, as current apps still contain most of the business logic in the Java/Kotlin part of the app (see Section \ref{sec:background}) rather than in the native part.

To counteract binary patching, the anti-repackaging checks need to be protected, i.e., through encryption applied at Java (see Sections \ref{subsec:dyn-self-prot-encrypt-2015}, \ref{subsec:sdc-2018},  \ref{subsec:bombdroid-2018}) or native level (Section \ref{subsec:bombdroid-native-2019}).
As an alternative, checks can be hidden by exploiting Java reflection~\cite{7579771}, however, once the attacker understands the protection pattern, he could patch the executable and remove checks with minimum effort, as discussed in~\cite{Norboev2018OnTR, 10.1145/3168820}.

\paragraph{Code Instrumentation and Injection:} \label{subsec:code_instrumentation_and_code_injection}
Such techniques allow to dynamically modify the code of a running process. In this way, the attacker is able to analyze functions or system calls, as well as their parameters and return values, and modify the behavior of the original functions. 

There exist a lot of tools that support code instrumentation and injection, as well as the corresponding runtime analysis. Nonetheless, Xposed \cite{xposed} and Frida \cite{frida}  are currently the \textsl{de-facto} standards.
Xposed is a framework that applies add-ons (called \textsl{modules}) directly to the Android OS ROM and requires root privileges. Such modules may allow, e.g., customizing the script that spawns any new process from the  Zygote one\footnote{The Zygote process is responsible for spawning new process to host launching apps.}, in order to add a jar file that allows hooking. % To achieve this, Xposed needs root privileges.

Frida is a dynamic code instrumentation tool that allows an attacker to hook functions by injecting a JavaScript engine into the instrumented process; the engine then allows injecting executable code by directly modifying the process memory. Frida can work on both rooted and unrooted devices in three different modes:
\begin{itemize}
    \item \textsl{Injected mode}: this is the most common deployment in which the user installs and runs the frida-server (i.e., a daemon) into a rooted device that exposes the frida-core module over TCP (usually on port 27042). 
    \item \textsl{Embedded mode}:  the user repackages the app with the frida-gadget (i.e., a shared library). This library allows instrumenting the app on an unrooted device.
    \item \textsl{Preloaded mode}: the frida-gadget shared library is injected inside the operating system layer instead of the application layer (as in the embedded mode). It works on rooted devices only.
\end{itemize}

Code instrumentation and injection allow stealing the actual values of program variables from a running application.
For example, the attacker could hook the function that decrypts some portion of code. In this way, he is able to recover the key for that specific chunk and the plain text. 
Then, the attacker can replace the encrypted code of an anti-repackaging check with a crafted one, by exploiting the binary patching technique previously discussed~\cite{owasp-mstg}.  

From the anti-repackaging standpoint, it is a hard task to safely hide checks that are resilient to code instrumentation and injection. As a matter of fact, system call hooking allows in principle to detect and attack any anti-repackaging check even if it is based on some kernel-provided functionality. In fact, Frida allows hooking tampering detection functions,  and makes them return the attacker's desired value. In addition, some “anti-frida” controls (e.g. simply check if the tcp port 27042 is open) relies on system call and can be circumvented by Frida itself.

An attempt to limit function hooking is proposed in \cite{10.1007/978-3-030-45371-8_12}, where some Java instructions are translated into native code to elude Java code instrumentation and avoid an attacker to recover the original statements. % However, code instrumentation is as difficult in native as it is in java code. 

\subsection{Network-based attacks}\label{subsec:network-attacks}
Previous attacking techniques focus on the device, the OS and the app. However, it is also possible to attack anti-repackaging at network level. Such attacks can be passive, i.e., the attacker does not affect the network traffic (e.g., \textsl{sniffing attack}) or active, i.e., the attacker willingly affect and spoof the traffic, (e.g., \textsl{replay attack}). 

\paragraph{Sniffing attack.}\label{paragraph:sniffing_attack}
It refers to the interception and the analysis of data exchanged by two parties on a communication channel (e.g., an app interacting with a remote server)~\cite{capec-157, capec-609}. 
This attack is relevant as some anti-repackaging checks are executed at server side. If an attacker understands the communication pattern and which data are sent between parties, he could be able to detect and circumvent these controls~\cite{owasp-m3}. %\luigi{al posto di "and circumvent these controls, inserirei "and retrieve critical information"}
For instance, an attacker is able to read the client-server communication if it is over \textsl{http}.

\paragraph{Replay Attack.}\label{paragraph:replay_attck}
The replay attack (or Man in the Middle attack - MitM) extends the sniffing attack by actively interacting with the two parties.  The attack dynamically affects the data exchanged during the communication, by relying on a MitM proxy~\cite{capec-94}.
Concerning anti-repackaging, if the signature check of an $apk$ is carried out at server side, then the client has to send the checksum of its certificate and an attacker could change the communication data in order to trick the server, or spoof a fictitious response from the server. Albeit all anti-repackaging techniques discussed in Section \ref{sec:sota} leverage local checks only, there exists some proprietary solutions which provides remote anti-repackaging detection, like Google safetyNet~\cite{safetynet}. The safetyNet API is provided by Google to Android developers, and can be included in any app. Such API provides functionalities against several security threats and specific checks against repackaging, which are applied both locally e.g., emulator detection, and remotely, e.g., signature detection on the server side. In this case, the attacker can try modifying the network traffic generated by the safetyNet API calls, to bypass server-side checks or spoof a fake answers from the server. Furthermore, the attacker can remove the invocation to safetyNet API functions by directly patching the smali code (or native one) by leveraging code deletion (Section \ref{subsec:code_delection}).

It is worth pointing out that MitM attacks can be carried out also inside the $apk$ itself: in this scenario, the attacker could modify at runtime some data using some of the code/data manipulation techniques previously discussed, with the aim to bypass specific anti-repackaging checks. The main idea is that an attacker could replace some resource file in order to bypass specific controls which rely on the app data
%\alessio{its: who are you referring to?}\luigi{the app} data
 (e.g., modify the path from the repackaged resource into the original one)~\cite{Norboev2018OnTR, 8186215}.

%\alessio{We need to decide whether to add the table or not. If it is too redundant, maybe we can drop it out.}


%\subsection{Google safetyNet notes}\label{sec:overview}

%\alessio{The following sentences need to be placed in previous subsection. TBD.}



%Some techniques explained above are very hard to prevent even with an anti repackaging defense. One possible approach is to make that “attacks” impractical and too costly. This solution doesn't solve the problem, but matches with the assumption that an attacker repacks an application only if it is more convenient than developing a new version of that application from scratch. 


==> [PMC] ARMAND Anti-Repackaging/sections/old paper files/background.tex <==
\section{App Repackaging: Backgroud and Threat Model}\label{sec:background}

In this section we briefly recap the basics of app development and distribution in Android. Then, we discuss a threat model for app repackaging, and we summarizes the main categories of repackaging detection and anti-repackaging techniques.

\subsection{Android App life-cycle}

\paragraph{App development.} A native Android app is developed in Java or Kotlin, and leverages XML files to represent the graphical user interface of the app. From now on, we will explicitly refer to Java code, although the same techniques are valid also in case of Kotlin-based apps. There are other ways to develop Android apps, for example hybrid apps. Hybrid apps are mainly built using web technologies and run over a WebView (e.g., Apache Cordoba\footnote{https://cordova.apache.org/}), and are likewise weak against repackaging. 
%Hybrid apps present the same vulnerability about repackaging as native apps. 

Each Android app is distributed and installed as an Android Package ($apk$) file. Until 2018, developers had to build their $apk$ file to distribute their app.
Since 2018 Google provides a new publishing format, i.e., the Android Application Bundle (AAB) \cite{android-app-boundle}, which allows building optimized $apk$ for each device configuration\footnote{Hereafter we will refer to $apk$ only, as the distinction between AAB and $apk$ is irrelevant for the problem at stake.}. 

In a nutshell, an $apk$ file is a zip archive containing all the necessary files to run the first execution of the app.
Each $apk$ is signed with its developer's private key and also contains the corresponding public certificate of the developer. This mechanism grants the integrity of the $apk$, but cannot provide any authentication, as the developer certificate does not need to be issued by a trusted certificate authority. Therefore, Android performs only basic verification on the $apk$ structure and its integrity, thereby leaving the decision to install the app (and, consequently, to trust the source of the app) to the final user. 

Regarding app repackaging, the most relevant files and folders contained in the $apk$ are:
\begin{itemize}
  \item \emph{META-INF/}: it contains the developer's public certificate and the app signature;
  \item \emph{lib/}: it contains the native libraries for each specific architecture (e.g., x86, armeabi\-v7a). An app could excute native C/C++ code through the Java Native Interface (JNI)\footnote{https://developer.android.com/ndk};
  \item \emph{res/}: it contains the binary resources, such as images or hybrid apps content;
  \item \emph{AndroidManifest.xml}: it describes the structure of the app and its components. In this file the developer defines app permissions, entry points, intent filters, and more;
  \item \emph{classes.dex}: it contains the compiled Java/Kotlin code in the form of bytecode, i.e., a high level representation of the machine code, that could be converted into Smali code, i.e., a human readable format, with off-the-shelf tools like Backsmali \cite{backsmali}. 
\end{itemize}

\paragraph{Application distribution.}
Android apps are mainly delivered through proper software repositories, called \textsl{app stores}, which allow developers to publish their $apk$. iOS relies on a single, centralized market  (i.e., the Apple Store), which is directly controlled by Apple. On the contrary, a distinctive feature of Android is the possibility to distribute the same app on dozens of different app stores beyond the official one (i.e., the Google Play Store\footnote{\url{https://play.google.com/store}}).  The most popular app stores differ from region to region. In Europe and US, the Google Play Store has the greatest market share \cite{android-markets-2019}. However, in 2019, in China, \textsl{Tencent My App} was the biggest Android app store with up to 25.5\% of the market share, followed by the \textsl{360 Mobile Assistant} and \textsl{Xiaomi App Store}; in this country the Google Play Store is just tenth place \cite{china-markets, android-markets-2019}. 

Whenever a user downloads an app from any store, Android carries out a soft check on the app certificate before installation, with the final decision left to the user~\cite{android-publish-app}: we recall that an $apk$ has to be signed by the developer, but Android continues the installation even if the signer of the developer's certificate is unknown~\cite{android-apk-authenticity}.
Since the only constraint is a valid signature, it is also possible to distribute the $apk$ directly (e.g., through email or urls) without the need to upload the app on an app store. %For example, a developer can publish his app over the web. This process is possible if user enable app installation from unknown sources in system settings. 

\begin{comment}
Io metterei qua l'immagine del flusso blu senza step 2 e direi una qualcosa del tipo (prendendo spunto da quello che hai detto tu nel capitolo dopo).
The common distribution process is briefly described below:
\begin{itemize}
    \item An individual or a company develop and build an Android app;
    \item An android app (apk or aab) is published in one or more application markets;
    \item An user can access to the published app in severall of different modes, the most common is searching on markets;
    \item An user can download and install the apk directly from the markets. The installed apk files are stored in \emph{/system/app/} or \emph{/data/app/} and can be execute by users
\end{itemize}
\end{comment}

\subsection{App Repackaging: Threat model}\label{sec:threat-model}

\begin{figure*}[!ht]
  \includegraphics[width=\textwidth]{figs/threat-model.pdf}
  \caption{App repackaging: Threat model.}
  \label{fig:threat-model-design}
\end{figure*}

In this section we discuss a threat model for app repackaging. The model is depicted in Fig. \ref{fig:threat-model-design}. 

The threat model involves three actors, namely the developer, the attacker and the user. The developer implements the app (Step 1), and may also add some anti-repackaging protection in the code before building the $apk$ (Step 2), in order to counteract repackaging attempts. In general, applying an anti-repackaging technique means to add some extra code that may lead, for instance, the repackaged app to crash. Then, the developer builds and signs the $apk$ and delivers it to the app store (Step 3). 

In an ideal (i.e., attack-free) scenario, the user fetches the store for apps (Step 4), then chooses and downloads the original $apk$. The validity of the signature and the integrity of the $apk$ is verified automatically by Android, by leveraging the developer's public key certificate provided in the $apk$. Then, the $apk$ is installed successfully and the user can execute the app (Step 6).

In an actual use case, an attacker can download the developer's $apk$ by behaving as any normal user. Then, the attacker decompiles and analyzes the $apk$ (Step 7), and tries to detect the anti-repackaging protections (Step 8). More in details, the attacker can decompile the $apk$ using Apktool~\cite{apktool} and perform static analysis on the smali source code. Smali is a human-readable format that can be obtained from the Dalvik bytecode contained in the $classes.dex$ file. Most of the smali code could be further decompiled back into Java code~\cite{10.1007/3-540-45937-5_10}. If static analysis is not sufficient, an attacker can dynamically infer the app behavior at runtime, by relying, for instance, on Frida \cite{frida}. A fruitful combination of static and dynamic analysis can allow the attacker to detect the anti-repackaging protections added by the developer in the app code.
In case some protections are detected, the attacker tries to neutralize them (Step 9) by deactivating the corresponding extra code, accordingly. Then, he can add some malicious code (Step 10) and build and signs a repackaged version of the $apk$ (i.e., $Rep_{apk}$) with a valid self-generated public key certificate. Finally, the attacker tests $Rep_{apk}$ on her own devices (Step 11). In case it works, the attacker can try distributing $Rep_{apk}$ (Step 12) both on official channels (i.e., app stores) and side-channels (e.g., by email, on website, through phishing attacks, \ldots). Otherwise, the 
attacker needs to carry out further analysis on the $apk$, and repeat Steps 7 to 11 (also known as the \textsl{try and error cycle}) until she obtains a working $Rep_{apk}$. 
%Then, the attacker redistributes $Rep_{apk}$ (Step 12) in order to reach the user, by trying to i) upload it on an app store, or ii) send it directly to the user by means of phishing attacks.

The attack succeeds whether some users install $Rep_{apk}$ instead of the original $apk$. In this case, the execution of $Rep_{apk}$ leads the user to execute the malicious code on her own device. The malicious code may have different aims, like e.g., access the app premium features for free or redirect revenue to cause financial loss to the developer, gain access to the user's private in app data (e.g., credentials), or make the app willingly unstable to affect the reputation of the original app.
%The attacker get access to the public store and retrieve the $apk$ provided by the developer. 

%ndividual or a company who develops an Android app (step 1). Once the app is ready to be published, it is possible but not necessary, to apply different protections with different goals (step 2). In our case we focus on repackaging avoidance protections (also known as anti repackaging or anti tampering). Once the application is built, developer can publish the APK (or the Android App Bundle) on various markets (step 3). 

%Users can now access to the app in dozens of different modes, the most common is searching on markets (step 4). An app it's downloaded and installed in the device as APK file. (step 5). Installed APK file are store in /system/app/ or /data/app/ and can be execute by users (step 6). 

%This first part of the process, represented in blue in the image, is the expected developing and consuming app flow. In addiction to that, we highlighted in red the process of an attacker who wants to repack the app.

%We assume that an attacker has full access to his device, including root access. The first stage for an attacker is to analyze the target APK (step 7).  (step 8). 
%The purpose of the analysis process is to find out the application logic, to inject the attackers code, such as ads or malicious code (step 10).
%In order to make the repackaging process more difficult, a developer can an apply different controls and protection to the application (step 2). This additional code aims to crash the app if some tampering is detected.
%With tampering controls the attacking process in more difficult. In the analysis phase, an attacker should detects repackaging controls (step 8).To neutralize these protections (step 9), the evil subject modify the source code and the resources of the app, injecting, modifying or removing code. 
%Only once repacking detection is defused, it is possible to add malicious code (step 10).
%Now the evil app is ready to be distributed on the market (step 11). The APK file should be build and signed by the attacker using its own certificate (which is different from the original app's owner certificate). Now we have the presence of a malicious APP1, repacked from APP, inside some app stores. Many users have now access to APP1. 
%The final step for an attacker is to force to download APP1 instead of APP (step 12). Phishing techniques can be applied to trick the final user to download and execute APP' instead of APP. Furthermore the evil subject can send directly the APP1 APK file to his victim using instant messaging or emails. 

%In the rest of the paper we will focus on discussing the state of the art of anti-repackaging on Android (Step 2). %, with a specific focus on \textsl{repackaging avoidance} techniques. 
%Furthermore, we will analyze the main attack vectors (Steps 8 and 9) against such techniques, with the aim to point out their weaknesses. %The attacker can always bypass these techniques using a "try and error" approach and achieve APP' step 6 successfully. Find and neutralize implemented defenses, however, could be harder than add malicious code. In our threat model we highlighted this difficulty with step 13, where the attacker has to evaluate the goodness of his repack. Eventually it may be necessary to return to step 7.
%Then, we will discuss a model for the optimal anti-repackaging technique, which is expected to be resilient to the current attack vectors. It is worth noticing that the more reliable is the anti-repackaging technique, the lower is the probability for the attacker to obtain a working repackaged app (Step 11). In this case, the attacker may find repackaging as a non cost-effective activity to target mobile users. 

\begin{comment}
\paragraph{Motivation}\label{par:threat-motivation}
Legitimate app can be repacked with different purposes:
\begin{enumerate}
	\item Access app premium features for free or redirect revenue, for example changing ads owner, causing financial loss for developers ~\cite{}.
	\item Change app behavior in order to gain users private or in app data, such as credentials.
	\item Use app as malware carrier.
	\item Make the app unusable to damage the company image.
\end{enumerate}
Only in scenario 1 the attacker is obliged to remove or bypass every control to be sure that the repack works perfectly.
On the other hand, in scenarios 2,3,4, the attacker needs that the repackaged app runs for a sufficient period of time to perform the attack (e.g. steal the credential).

Moreover, the repacking threat allows an attacker to hide malware under popular and well ranked apps. In this way, he could camouflage his evil application as the original and benign one, easily spreading it to a huge number of people.

\end{comment}

\subsection{Repackaging Detection vs. Anti-Repackaging}\label{sec:threat-mitigation}

This section points out the main features of both \textsl{repackaging detection} and \textsl{anti-repackaging} techniques. 
%pro and cons of different approaches to repackaging threat. 
%Repackaging detection and avoidance are two different techniques %that wants to achieve different goals. In the following paragraphs we are going to discuss both in depth. Note that our focus is repackaging avoidance state of the art review.

\subsubsection{Repackaging Detection}\label{subsec:repackaging-detection}
Repackaging detection focuses on recognizing repackaged apps in app stores or on user's devices, with the aim to limit the spread of repackaged app (i.e., Step 12 in Figure \ref{fig:threat-model-design}).
Repackaging detection techniques can be divided into static and dynamic approaches \cite{10.1016/j.procs.2016.02.006}, and further grouped into five different categories (see \cite{10.1109/TSE.2019.2901679}). 
\begin{itemize}
    \item \textbf{Static or offline techniques} are adopted on \textsl{app stores} to identify uploads of repackaged apps which are clones of original apps. 
    Such techniques strongly relies on \textsl{symptom discovery} or \textsl{app similarity}. Symptoms \cite{10.1109/TSE.2019.2901679} are tracks, such as strings, left by the repackaging process itself. Similarity checks usually involve a two-step process in which each app is first profiled according to a set of distinctive features; then, apps with almost identical feature profiles are identified.  Such techniques make strong use of machine learning, both supervised \cite{0.1109/SPW.2016.33, Lin2013IdentifyingAM} and unsupervised~\cite{10.1007/978-3-319-23829-6_30}. 
    Static analysis needs a considerable amount of resources both in order to generate the decision model and to make the final decision, and can be efficiently applied only on server side.    
    \item \textbf{Dynamic or online techniques} are directly executed on the user's device to evaluate the app.
    These approaches extract specific information both at install-time and at run-time. For instance, the technique discussed in \cite{10.1145/2484313.2484315} puts a watermark inside the app which is checked by a third authority at runtime.
\end{itemize}

\paragraph{Attacking Repackaging Detection.} An attacker successfully circumvents a repackaging detection technique once it is able to build repackaged apps that go undetected both on the app store and on the devices. According to the characteristics of the current detection techniques, this means that the repackaged app must appear very different from the original app (to bypass similarity checks), hide repackaging identifiers (to avoid symptom discovery), and behave as the original app to circumvent dynamic analysis.  
It is also worth pointing out that the granularity of the Android ecosystem - which allows to deliver apps through an undefined number of app stores and side channels (e.g., apps available at some URIs or delivered by email) - makes hard to build up a reliable, pervasive and full-fledged repackaging detection deployment. In fact, this would require to deploy static analysis mechanisms on each source of apps (i.e., app stores and servers), as well as dynamic analysis solutions on each mobile device.
%in fact, enforcing repackaging detection in a pervasive and exhaustive way is tricky, as the granularity of the Android ecosystem 

%In a detection techniques an attacker should focus on how the detection model could be bypassed. If the perfect model, the one with 100\% accuracy and recall, 0\% false positive and false negative, existed then there would be no hope for attackers. 

%Due to the vast granularity of Android ecosystem, as already show in \autoref{sec:background}, is impossible to impose a central authority that guarantees repackaging detection to every Android device.

\subsubsection{Anti-Repackaging}\label{subsec:repackaging-avoidance}
Anti-Repackaging - also known as \textsl{repackaging avoidance} or \textsl{self-protection}
%\footnote{Hereafter, we use these names interchangeably.}
 - aims to protect an app from being successfully repackaged. As opposed to repackaging detection, anti-repackaging is applied by the developer to the app code before building the $apk$ (Step 2) and aims to make any repackaged version of the same app crash. On the bad side, the attacker aims to detect and neutralize the anti-repackaging protection after reversing the $apk$ (Steps 8 and 9). 
From a technical standpoint, anti-repackaging techniques insert some logic controls (i.e., \textsl{anti-tampering} checks) inside the $apk$. %\alessio{From here.} 
%These integrity controls are called anti tampering (AT) checks. 
%An attacker in step 8 of our threat model can detect these protections, and eradicate them in step 9. 
Since the first aim of the attacker is to recognize anti-repackaging, the requirements of anti-tampering checks are i) to go undetected and hide inside the app code, and ii) in case of detection, to avoid being de-activated. To achieve such results, anti-tampering checks may rely on code obfuscation, code virtualization and anti-debugging techniques.  We briefly introduce anti-tampering checks and such techniques.%In our scope make the attacker process hard is not sufficient, the optimal repackaging avoidance technique does not allow the control to be removed. 

\paragraph{Anti-tampering.} In a nutshell, anti-tampering checks are self-protecting functions which aim to detect any modification on the original app. There exist several methods to detect tampering in mobile apps, as highlighted in \cite{BERLATO2020102463}. 
The most relevant anti-tampering techniques are:
\begin{itemize}
    \item \textbf{Signature checking}: the most trivial control, which checks the certificate contained in the $apk$. This approach could detect any modification applied to the original $apk$;
    \item \textbf{Code integrity}: it checks whether some specific part of the code has been tampered with, by computing its signature at run-time. As an example, the first bytes of the \emph{.dex} file contains the hash of its content. This method detects a tampering only if the attacker has modified the checked methods;
    \item \textbf{Resource integrity}: it checks the signature of some resources at run-time. 
    This technique differs from the previous ones as it checks tampering attempts in the app resources (e.g., images and other binary files) instead of the code;
    \item \textbf{Installer verification}: it checks if the installing app comes from trusted app stores. This technique is applied under the assumption that tampered apps are more likely to be distributed on unofficial app stores.
\end{itemize}
Anti-tampering checks dynamically react to any modification either in the app or in the executing environment. 
Once some checks are detected by the attacker (Step 8 in  Figure \ref{fig:threat-model-design}), the same attacker tries to bypass them by following the \textsl{try and error} approach, i.e., she modifies the app (in order to try removing checks), then she repackages and tests the app to check whether it works properly. If the attempt fails, then the attacker may try to search for other checks and/or modify the app in a different way.

\paragraph{Code obfuscation.} Obfuscation approaches modify the bytecode or the source code of an app, without changing its behavior, in order to make some manual or automatic analysis more difficult. There exist a lot of off-the-shelf obfuscation tools both open source \cite{aonzo2020obfuscapk} and commercial \cite{proguard}. %In \cite{10.1016/bs.adcom.2017.09.004} Banescu et al. presented the MATE (Man At The End) attack model. This model is applicable in repackaging threat. Authors  proposed a list of techniques, based on code obfuscation, that protect from MATE attack model.   %These techniques aims to make harder the step 9 \autoref{fig:threat-model-design}.

\paragraph{Code virtualization.}
Code virtualization is a specific obfuscation scheme. In this approach, instructions are mapped to semantically-equivalent virtual instructions. A virtual machine (VM) executes inside the app and interprets the virtual instructions. Two different approaches are proposed in \cite{10.1145/2557547.2557558, 2019-exploiting-binary}; the first one works at DEX level, while the latter focuses on native libraries. %These works proposed themselves as effective countermeasures against static analysis, dynamic analysis, and specific analysis for virtual machines.
Similarly to obfuscation, this approach aims at complicating the reverse engineering process of an app, but it does not introduce any anti-tampering check.

\paragraph{Anti-debugging.} Anti-debugging controls aim to detect and avoid dynamic analysis checks (e.g., debugger). Differently from passive obfuscation techniques, where the app code is syntactically modified to make it harder to understand, anti-debugging controls allow an app to actively react against malicious reverse engineering  at run-time \cite{BERLATO2020102463}.
The most widespread anti-debugging techniques are:
\begin{itemize}
    \item \textbf{Emulator detection}: it checks whether an application is running on a real device or in an emulated environment;
    \item \textbf{Time check}: when an app executes with a debugger, its execution slows down. Time checks can be specific functions whose execution depend on the execution time: in case the execution time is higher than a given threshold, such functions take the app to an inconsistent state;
    \item \textbf{Check debuggable}: the \emph{AndroidManifest} contains a flag that enables the debugging mode: if this flag is set to false, an user is not able to attach any debugger to the application. The attacker can bypass this check by changing the manifest accordingly. Nonetheless, such modification could trigger some other anti-tampering checks.
\end{itemize}
Recently, more complex anti-debugging techniques have been put forward~\cite{10.3390/s19112625}. Among these, the most promising one is discussed in \cite{article}: the intuition is to exploit proper features of the Android Runtime to hide anti-debugging instruction at runtime. As any other solution relying on version-specific features of the Android OS, also this approach quickly became obsolete, as it worked properly only up to API 25 (i.e., Android v. 7.1).

%In this section we briefly introduce some basic concepts related to both anti-repackaging detection and avoidance; in the following section, we will analyze in detail the state of the art related to the latter category. %\ref{sec:sota}.
\begin{comment}
A logic bomb is a piece of code which will bring the app in some undefined behavior, such as crash or inconsistency, when specific trigger conditions are satisfied \cite{10.1145/3168820}.
Logic bombs use a combination of what has been described above to achieve the repackaging avoidance purpose.

\begin{figure}[H]
  \includegraphics[width=\linewidth]{images/repack.png}
  \caption{Logic bombs design}
  \label{fig:bombs-design}
\end{figure}

The last formal definition of logic bombs is proposed in \cite{10.1007/978-3-030-45371-8_12}. 
\figref{fig:bombs-design} shows how to generate a basic cryptographically obfuscated bomb. The left box contains the original code. Firstly the trigger condition "v == constant" is transformed into "Hash(v) == Hc", where Hc = Hash(constant). The value of variable v is then used to decrypt the original code. As shown in right box inside the original code could be performed various checks in order to evaluate app and environment integrity.
In this structure, where the hash function is used to hide the encryption key, the logic bombs can be inserted only in specific portion of code where are present the trigger condition.

A set of logic bombs represents an anti repackaging technique: a methods that allows the developer to protect his app from the repackaging and all attacks that we will explain in the \autoref{sec:attacking_model}. In addition, these logic controls rely on AD and AT controls to detect any environment or application alteration.


\end{comment}





==> [PMC] ARMAND Anti-Repackaging/sections/old paper files/bestdefensetecnique.tex <==
\section{Utopian defense technique} \label{sec:best_defense_technique}
In this section we propose the characteristic of different approaches which aim to prevent the repackaging threat. In all this tree cases, we base our assumption on the fact that users are not colluded with attackers. Our goal is to show the characteristic of these features without considering if they are achievable or not.

\paragraph{Part I}
As shown in \ref{sec:background} in Android is possible to install apps from different sources. In other operating systems the only place to download apps is from unique central repository, called store. iOS apply this policy. There are several techniques to bypass this restriction \cite{doi:10.5465/ambpp.2013.13947abstract}, however we can assume a user not colluded with attackers won't overcome these type of protections.

Inside the unique store is possible to implement the perfect static repackaging detection techniques. When a user submit an application to the central repository, controls are performed to identify similarities with all the other apps present inside the store. In this way repacked applications are detected and not published. 
It is out of our scope evaluate a perfect repackaging detection technique. Thanks to this central control, repackaging protection inside the app would be useless.

Unfortunately, this is in contrast with the openness Android philosophy and fragmentation in mobile devices market.

\paragraph{Part II} 
% gli attacchi sono sempre possibili, ma cerco di proteggere tramite controlli server-side (come se mi costruissi la mia CA)
% Parte di analisi generale su eventuali caratteristiche
In this paragraph we want to study which protection could be implemented inside apps that rely on network communication. We will therefore discuss self-defending technique based on a client-server architecture. 

We assume that all attacks presented in \autoref{sec:attacking_model} can be performed. In this scenario, our goal is to design a defense architecture that is resistance (against repackaging, not the above attacks) and that relies on server integrity controls: the server works as authority that detect possible tampering.
With this structure, the application hides any AT or AD functions server side. Moreover, the app flow depends on the server response, which should be different at each new request.

The apk (client side) have to send some app or environment information to its backend in the safest possible way. For example an application could encrypt the payload of each request with different communication keys, or could use custom communication protocols. In other words, the main goal related to this design is to make the attacks described in \autoref{paragraph:sniffing_attack} and \autoref{paragraph:replay_attck} ineffective.

% Breve analisi su vantaggi/svantaggi
With a client-server architecture, all static analysis are bypassed and the goal for an attacker is to understand call pattern. This task could be very time consuming because the server side functions are a blackbox and its services cannot be reverse engineered.
Furthermore, this approach could allow developer to update the AD and AT functions without any impacts to the client side.

This area of research has already been deepened in other studies, such as \cite{10.1145/1230040.1230087, 10.1145/2991079.2991119, 10.1145/2043628.2043633}. In online video game attackers try to modify the game client in order to cheat, or play without paying. This situation is similar to that of repackaging in Android apps.
From another point of view, this technique doesn't solve some of the common attacks, but tries to create an architecture that can limit them. This means that an attacker could still create a working repackaged app with an hard and time consuming work. Contrary to the state of the art defending methodologies, this architecture allow a developer to change the API interface in order to lose backward compatibility with old version of an app. In this way, the app users are forced to update their version, but a repackaged app will stop working.

Another possibility that involves the presence of a central authority (CA) is that app developers can share a secret between their app server and the central authority itself. A scheme that includes CA, device operating system and developer server could guarantee that the communication to developer server can only happen through the legitimate app. In this way repackaged apps can't reach the server.

\paragraph{Parte III} 
In order to ideally protect apps from repackaging, we have to mitigate the underling problem. An attacker could apply different attacks (presented in \autoref{sec:attacking_model}) to analyze, understand and circumvent the app AD and AT controls. Once the attacker understand the protection model, he is able to remove this controls patching the bytecode. This is the required step to create a fully working app bundle (apk) that could be shared in an app store. 
Due to this, if a developer is able to avoid the code manipulation threat \autoref{subsec:code_manipulation} (both code deletion and binary patching), the repackaging threat could be exceeded. 

Unfortunately, this threat cannot be solved with the state of the art anti repackaging techniques. These approaches implement several strategies which aim to make more difficult some attacking models.
In this way, the best defending technique is the methodology that mitigate the largest number of threats and makes more difficult the attacking process. 

For example, the technique implemented by Bombdroid (introduced in \autoref{subsec:bombdroid-2018}) is strong against static analysis and a trivial code deletion. We have shown as dynamic analysis procedures such as code instrumentation \autoref{subsec:code_instrumentation_and_code_injection}, could be used to recover deciphered code and the encryption key. With these information, an attacker is able to create a repackaged version from the original app.
In order to make Bombdroid the perfect self-defending technique, authors should mitigate all possible dynamic analysis. Is out of our scope to determine whether this task is achievable or not .

As described in \autoref{sec:background}, the repackaging threat id due to the possibility to decompile and analyze an apk. Another technique to avoid this threat is to prevent the file extraction from the app bundle: if is impossible to get out the files in an apk, an attacker could not recover the source code and resources. In this way is not able to create a repackaged version of the original app.

\begin{comment}
Scaletta / Considerazioni
 -) Analisi statica: obfuscation, cifratura o scaricare il codice solo quando serve (ad esempio con dynamic delivery -> https://developer.android.com/guide/app-bundle/dynamic-delivery)
 -) Fuzzing/Symbolic execution -> ?!? -> non so neanche se avrebbe senso, posso sempre inserire e runnare l'app quante volte mi va!
 -) Debugging -> in teoria se un apk ha la flag debuggable a false non può essere debuggato nel modo classico. La flag però puo essere cambiata on the fly con tool come Xposed (ma lo metterei in un altro capitolo). In aggiunta check tempo o altri metodi classici.
 -) Process Exploration -> ?!? -> si potrebbe vedere come funzionano i singoli tool per fare avoid del singolo tool (tipo per frida), ma non è una cosa generica che mi piace.
 -) vtable Hijacking -> esistono lavori che analizzano e mitigano il problema (come VTPin - https://download.vusec.net/papers/vtpin_acsac16.pdf - https://github.com/uberspot/VTPin) -> Io credo che questo più che un problema legato al repackaging, può essere visto come un problema "strutturale" del come vengono richiamati i metodi virtuali nella VM di Java e quindi non lo considererei nel nostro lavoro
 -) Code deletion -> il flusso deve dipendere da quella "porzione di codice" e il suo risultato non deve essere si/no o predeterminabile, altrimenti può essere facilmente hardcodato
 -) Binary patching -> ?!? -> Credo che evitare questo sia davvero impossibile. In generale pensavo che se il bytecode è cifrato il patching è impossibile finchè non viene recuperata la chiave di decifratura. In alternativa si può offuscare pesantemente il codice (sarebe piu difficile da modificare). In generale mi piacerebbe trovare qualche considerazione più "forte" di questa
 -) Code Instrumentation -> ?!? -> In generale ci vorrebbe una tecnica che non richiama funzioni e/o che non faccia syscall (come se fosse un modulo in mutua esclusione rispetto tutto il resto). Non esiste neanche un tecnica generica perchè esistono tanti tool diversi (e.g. frida, xposed) che lavorano in maniere differenti. Possono aiutare i check dell'environment, ma non risolvono!
 -) replay attack variante -> ?!? 

In generale contro ogni analisi dinamica (e cumulative attack) si può aggiugere "randomicità" ai controlli effettuati

Altra cosa se avevamo detto era quella di aggiungere una soglia di "bontà" delle trigger condition, e.g. non ci piacciono trigger condition nelle librerie o per valori che sono compresi in piccoli range.

NB: tratto da https://stackoverflow.com/questions/17225590/prevent-make-it-difficult-to-patch-binary-assembly
Write self modifying code
Again this thwarts static analysis. For example if your jump into the verification function does not exist in the binary but is patched everywhere as part of some init() function in the .so
\end{comment}



==> [PMC] ARMAND Anti-Repackaging/sections/old paper files/conclusion.tex <==
\section{Discussion, Conclusion and Future Work}
\label{sec:conclusion}
In this paper, we discussed the state of the art of anti-repackaging techniques, unveiling their limitations and the way to attack them.
Such techniques are far from being robust against the available attacking vectors.   We argue that improving the reliability of anti-repackaging on Android demands for developing novel methodologies that can discourage an attacker from trying to deactivate them. Future anti-repackaging approaches should follow some guidelines, derived from the lesson learned:
\begin{enumerate}
    \item \textbf{Use multiple patterns}. Current techniques adhere to a common pattern (i.e., qualified conditions, adoption of hash functions, \ldots), which we showed to be rather easy to detect and de-activate by an attacker. The same anti-repackaging scheme should implement several distinct patterns to disseminate logic bombs in the app. 
    Furthermore, as we shown in NRP, a single anti-tampering control could be easily bypassed by an attacker. Therefore, several heterogeneous anti-tampering controls must be distributed thorughout the app.
    \item \textbf{Rely on native code}. As reversing and instrumenting native code is more complicated than bytecode, both logic bombs and their triggering conditions should be moved to native as much as possible. 
    \item \textbf{Optimized pervasiveness of the logic bombs}. Some approaches implement few controls in the name of performance, while others embed a lot of bombs which are not actually triggered at runtime. In this respect, there is the need for a more effective deployment of logic bombs, also at the cost of higher time and space overheads.
    \item \textbf{Honeypot bombs}. Proper fake bombs can be added to disguise the attacker to remove them. The removal of such bombs should trigger the real ones and lead the app to crash. This idea has been proposed in literature but never actually applied in current proposals, where the focus is more on generating stealthy logic bombs. 
    \item \textbf{Hiding anti-repackaging protection}. It is fundamental to improve the stealthiness of anti-repackaging to make hard for the attacker to understand that the reverse-engineered app actually contains some protection. Therefore, obfuscating anti-repackaging and anti-tampering controls may help.
    \item \textbf{Mixed Client-side and Server-side controls.} Most of the proposals check the app directly on the device (client-side) while others adopt remote controls (server-side) only. A more effective anti-repackaging protection must combine both of them. Furthermore, runtime-generated server-side controls can improve undetectability.
\end{enumerate}

As a future extension of this work, we plan to implement an anti-repackaging solution that we already designed according to the previous guidelines. We plan to assess it on a high number of Android apps, and to make both the source code and the experimental results available to the research community.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:




==> [PMC] ARMAND Anti-Repackaging/sections/old paper files/intro.tex <==
\section{Introduction}
\label{sec:intro}
During the last five years, Android strengthened its leadership among mobile operating systems with more than 75\% of market share on average~\cite{statcounter:2019}.
Most of this success is due to the app development process, which  is easier compared to other mobile operating systems: in fact, Google currently offers a plethora of platforms that support the developer in designing, implementing, testing and sharing her application~\cite{android-developer-guide}.
As a consequence, the number of Android apps in the Google Play Store reached 2.8M in 2020\footnote{https://www.appbrain.com/stats/number-of-android-apps}. 

From a security standpoint, Android apps are the main target for attackers, as they allow to reach a large number of mobile users. In fact,
%Because of the large number of applications and their usage, attackers are encouraged to write exploits against the Android OS and its apps in order to attack a large numer of users.  
since a mobile app is available in public app markets (e.g., Google Play Store, Samsung App Store, \ldots), an attacker can easily retrieve the app bundle (i.e., the $apk$ file, which is basically an archive containing the app). Then, the attacker can reverse engineer the $apk$ \cite{2011-android-reversing}, inject some malicious code, and re-distribute a modified version of the original app. This kind of attack is called \textsl{repackaging}.

%Once the app is obtained, then reverse engineering can be performed to extract sensitive information or to craft a modified version and share it in app stores or over the internet . This type of attack is known as repackaging. 

Android repackaging is a serious problem that may affect any unprotected app. A repackaged app can cause money losses for developers as the attacker can re-distribute paid apps for free, remove/redirect ads earnings, or make the app willingly unusable to negatively impact the reputation of the developer.
%Furthermore malicious code can be added inside the apk in order to cause damages to user devices. 
Furthermore, recent studies~\cite{10.1145/3017427} demonstrated that the 86\% of Android malware is contained in repackaged apps. This is indeed a promising strategy for malware developers, as embedding the malicious code in a repackaged version of popular and well-ranked app speeds up its spread.

It is worth pointing out that repackaging is intrinsically related to the Android development life-cycle, where an $apk$ just needs to have a valid signature in order to be successfully installed and execute properly, without requiring any guarantee on the actual identity of the signer (i.e., the developer does not need a valid public key certificate issued by a trusted certificate authority). Therefore, an attacker can modify an existing $apk$ and then repackage and sign it with her own self-generated private key. 

In order to make the repackaging phase more challenging for attackers, in recent years several techniques have been proposed in literature. Such techniques can be divided into two sets, namely \textsl{repackaging detection} and \textsl{anti-repackaging}: the first set aims at recognizing repackaged apps, while the latter one focuses on inserting proper controls in the app, such that a repackaged version of the same app would not work properly. 

%The threat model will be discussed in deep in \autoref{sec:threat-model}.
While repackaging detection techniques have been widely discussed and analyzed in literature \cite{Zhan2019ACS, 10.1109/TSE.2019.2901679}, no systematic analysis of anti-repackaging techniques is still available. To this aim, in this paper we provide an extensive analysis of such techniques. More in details, the contribution of the paper is three-fold: %\alessio{Modify this following part at the end.}. 
after introducing some background and the threat model related to app repackaging in Section \ref{sec:background}, we first discuss the state of the art of anti-repackaging techniques in Section \ref{sec:sota}. Then, in Section \ref{sec:attacking_model} we summarize the attacking techniques that can be used to circumvent anti-repackaging. Finally, in Section \ref{sec:attack} we will show how existing anti-repackaging techniques can be circumvented to produce a fully-working repackaged version of a protected app. 
%Moreover, in Sec \ref{sec:best_defense_technique}, we provide some solutions to recurrent security issues in repackaging avoidance techniques. 
We also discuss a full-fledged attack to the most recent anti-repackaging technique to date, which is the only one whose source code is publicly available. More in detail, we show how to bypass the protections and successfully repackage a real app (i.e., Antiminer \cite{antimine-android}).
Finally, in Section \ref{sec:conclusion} we draw some conclusions, pointing out some guidelines to improve the robustness and the reliability of the next-generation anti-repackaging techniques. 

\begin{comment}
With this approach we want to overcame the assumption made in the state of the art works, that an attacker repackage an app if and only if it is more convenient then reimplement the app from scratch \cite{8186215}.

\end{comment}


%More in details, the contribution of the paper in four-fold:
%\begin{enumerate}
%    \item A review of the main repackaging avoidance techniques in Android, with a specific focus on their implementation (Section \ref{sec:sota}) when available;
 %   \item A categorization of all possible attacks to the repackaging avoidance techniques (Section \ref{sec:attacking_model})
  %  \item For each repackaging avoidance techniques, 
%\end{enumerate}

%Our contribution is an in deep survey of the main anti repackaging techniques proposed over these years, with focus on their implementation. Furthermore, we are also going to analyze to which attacks they are resilient and how to circumvent these techniques in order to produce a fully working repackaged app. Our scope is to identify which approaches are more safe and how much effort is required to implement these anti repackaging methodologies.
%After that, we are going to provide some solutions to recurrent security open issues in some self-defending approach in the state of art works. 
%Finally, we are going to propose a model to utopically ac




%In this paper we want to analyze in details Android repackaging avoidance techniques proposed over the years. 
 
%\subsection{Goal}\label{sec:goal}
%To our knowledge, there is no systematic review of anti repackaging techniques yet. 
\begin{comment}
The first anti repackaging proposal, Divilar \cite{10.1145/2557547.2557558}, tried to introduce a virtualization based protection scheme to secure Dalvik bytecode. Future works tried to implement this technique over native code \cite{2019-exploiting-binary}. 
In 2015 a novel technique \cite{7299906} presented the use of native code to encrypt and decrypt the source code at runtime.
Starting from 2016 a new approach based on insertion of "repackaging detection nodes" inside the original app was proposed in different works \cite{7579771, 8368344}.  The purpose of a detection node is to control the app integrity and to detect any tampering using different techniques, such as assets or code checksum. One of the main issue with this approach is the ease with which a guard can be deleted or bypassed. To overcome this problem, researcher proposed to insert inside this detection nodes some application code, so an attacker can not remove guards without compromising the app functionality \cite{10.1145/3168820, 8186215}. However, with dynamic analysis techniques is possible to circumnavigate this protection. The approach proposed in \cite{10.1007/978-3-030-45371-8_12} tried to make guards more complex using native code. 
Finally, we are going to propose a model to utopically achieve  the perfect anti repackaging technique. 
With this approach we want to overcame the assumption, from state of art works, that an attacker repackage an app if and only if it is more convenient that reimplement the app from scratch \cite{8186215}.

\end{comment}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

%  LocalWords:  biometrics cryptographic parallelized lossy


==> [PMC] ARMAND Anti-Repackaging/sections/old paper files/results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation}
\label{sec:eval}


The results section should have the results of your experiments and
measurements. Evaluation is the most important part of the research. Sometime
you might want to split it into more than one section depending on the type of the project.



Again make sure you give enough details so that the reader can reproduce your
evaluation. Your GitHub code is not a replacement of the details, GitHub will
perish, your paper will remain in this world for centuries to come. Of course,
you need strike a balance between mundane details vs what makes your evaluation
unique.









==> [PMC] ARMAND Anti-Repackaging/sections/old paper files/sota.tex <==
\section{Anti-Repackaging: State of the art}\label{sec:sota}
This section presents the state of the art of anti-repackaging techniques on Android, ordered chronologically. For each proposal, we will describe the idea, the protection scheme applied on the app before release, the runtime protection during the app execution, as well as the experimental results. In Section \ref{sec:attack} we will discuss limitations and effective attacks against these works.

\subsection{Self-Protection through \texttt{dex} Encryption} 
\label{subsec:dyn-self-prot-encrypt-2015}
In 2015, M. Protsenko et al. in \cite{7299906} proposed an anti-repackaging technique aimed at complicating both the reverse engineering and the repackaging process. The main idea is to encrypt the \texttt{classes.dex} file in the $apk$, and dynamically decrypt and execute it at runtime. 

\begin{figure}[!ht]
  \includegraphics[width=\textwidth]{figs/self-protecting-encrypted-dex.pdf}
  \caption{The Dynamic Self-Protection and Tamperproofing scheme.}
  \label{fig:dynamic-scheme}
\end{figure}

\paragraph{Protection scheme:}

The approach, depicted in Fig. \ref{fig:dynamic-scheme}, applies to the compiled $apk$, that is modified according to the following steps: 
\begin{enumerate}
    \item A XOR key is generated (Step 2.1) and applied to encrypt the whole \texttt{classes.dex} file(s) (Step 2.2);
    \item An native activity\footnote{An activity is an app window containing the UI.} is automatically built (Step 2.3) and compiled in a shared library. Such activity is called native, as it is written in native code (C/C++ code) instead of Java/Kotlin code as the other activities. The XOR key is added to the native activity;
    \item The native activity is obfuscated using the OLLVM tool \cite{obfuscator-llvm} (Step 2.4);
    \item The Android Manifest is configured to execute the native activity (written in C/C++) rather than the original main activity\footnote{The Main Activity is the first activity prompted to the user when the app is executed.} when the app starts executing (Step 2.5).
\end{enumerate}
Finally, the $apk$ file is generated, signed and delivered (Step 3).
    
\paragraph{Runtime behavior:}
When the app executes, the protection scheme behaves as depicted in Fig. \ref{fig:dynamic-scheme-runtime}. At first, the modified manifest forces the execution of the native activity (Step 6.1). The native activity begins by extracting the XOR key (Step 6.2) and launches the main activity (step 6.3). As the execution of the main activity requires access to the plain bytecode, the XOR key is applied to decrypt only the part of the code required for the proper execution of the main activity. Then, after the execution is completed, the same bytecode is re-encrypted using the same key (Step 6.4). The approach is time-sliced, thereby decrypting parts of the \texttt{classes.dex} file on-demand, i.e., maintaining the bytecode unencrypted only when it needs to execute (Step 6.4).  

\begin{figure}[!ht]
  \includegraphics[width=\textwidth]{figs/self-protecting-encrypted-dex-runtime.pdf}
  \caption{Dynamic Self-Protection and Tamperproofing: runtime behavior}
  \label{fig:dynamic-scheme-runtime}
\end{figure}



%\paragraph{Tampering detection and response}
%In the paper implementation a simple XOR-based hash is used as tamperproofing checksum. If the decryption key is invalid it is not possible to decrypt the correspondent encrypted method.

\paragraph{Evaluation:}
The adoption of a XOR-based encryption of the bytecode is aimed at implementing a tamper-proof checksum.  
This work has been evaluated on 749 apps from the F-Droid app store \cite{f-droid}. Due to implementation and process choices, only 312 apps can be properly protected. For instance, it was not possible to protect apps which make use of Java reflection. The experimental setup leveraged several Android devices equipped with Android 4.4.2, and stimulated through the Android Monkey UI Exerciser framework \cite{monkey} at runtime. Clearly, the adoption of encrypting/decrypting cycles, as well as the addition of extra code, negatively impacts the app time and space complexity. In fact, the experiments indicate a mean execution overhead of 440\% and an increased $apk$ size by 183\% on average. 

The reliability of the proposed protection scheme is evaluated according to four metrics: method exposure (both absolute and percent value), and instructions exposure (both absolute and percent value). A method or a instruction is \textsl{exposed} when it is decrypted. Experimental results show a wide variance. On average, about 83\% of methods - which amount to the 80\% of the bytecode instructions - are exposed. %However, some apps have a relative instruction exposure around 2\%, or in some cases 100\%.

\subsection{Stochastic Stealthy Networks} 
\label{subsec:ssn-2016}
% Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/Repackage-proofing%20Android%20Apps%20~%20Stochastic%20Stealthy%20Network.pdf
% https://cse.sc.edu/~lluo/papers/ssn-robustness-2017.pdf, riassunto nel capitolo 2.1 di bombdroid

In 2016, Lannan Luo et al. put forward another self-protecting approach against repackaging, named Stochastic Stealthy Network (SSN) \cite{7579771}. 
%This work was presented in 2016. 

\begin{figure}[!ht]
  \includegraphics[width=\textwidth]{figs/SNN-scheme.pdf}
  \caption{The SSN protection scheme}
  \label{fig:ssn-scheme}
\end{figure}

\paragraph{Protection scheme:}
The idea is to distribute (and hide) a set of guards (i.e., \textsl{repackaging detection} nodes) into the app source code. When executed, such guards trigger proper decision points (i.e., \textsl{repackaging response} nodes) that, in case a tampering is detected, make the app crash. 
More in detail, the protection workflow, depicted in Figure \ref{fig:ssn-scheme}, begins by selecting a set of candidate methods in the Java code, according to some heuristics (Step 2.1). Then, a set of repackaging detection nodes are injected in such methods (Step 2.2), as well as the set of repackaging response nodes (Step 2.3). Such latter nodes take decisions according to a stochastic function. Moreover, a communication channel is added in the code to allow both kinds of node to communicate at runtime (Step 2.4). The communication channel is made by extra variables and methods added in the app code. Finally, SSN builds, signs and delivers an $apk$ with code extended with the repackaging nodes.

It is worth noticing that the selection of candidate methods must take into consideration the overhead due to the execution of detection and response nodes: to this aim, good candidate methods must be seldom invoked at runtime. Furthermore, the detection nodes must be strongly distributed over the set of candidate methods, to increase stealthiness. 

%\paragraph{Node construction}
%Detection nodes are injected inside candidate methods. Candidate methods are invoked for a few times during the execution of the app. In this way the overhead is lower. 
%Detection nodes are split into several parts in order to achieve better stealthiness. 

\begin{figure}[!htb]
  \includegraphics[width=\textwidth]{figs/SSN-scheme-runtime.pdf}
  \caption{The SSN behavior at runtime.}
  \label{fig:ssn-scheme-runtime}
\end{figure}


\paragraph{Runtime behavior:}
Fig. \ref{fig:ssn-scheme-runtime} depicts the SSN behavior during app execution. Whenever a candidate method executes (Step 6.2) and activates a repackaging detection node (Step 6.3), then the same node connects to the corresponding response node(s) through the communication channel. If the stochastic function recognizes the method as repackaged (i.e., modified) then some execution is triggered. Such execution may lead to modify specific variable values or raise specific exceptions\footnote{Unfortunately, the paper does not provide such details.} that can result in program crashes or delayed logical malfunctions. 

\paragraph{Evaluation:}

The SSN approach only verifies the integrity of candidate methods by relying on the developer's public key verification. However, SSN supports several other predefined templates. For instance, reflection is used to call functions such as \longstring{getPublicKey()} and \longstring{generateCertificate()}. 

The viability of the SSN approach has been empirically evaluated on a set of 600 apps, belonging to ten app categories in F-Droid. Experiments were conducted on emulators equipped with Android 4.1.
The average time overhead is between 6.4\% and 12.4\%, which is far lower than the time overhead of the previous approach, discussed in Section \ref{subsec:dyn-self-prot-encrypt-2015}. Furthermore, each protected app works properly, and no space overhead is noticed. %Authors asked three humans to make a repacked app (previously protected with their prototype) work properly for one hour. They had 24 hours. None of he apps was successfully repackaged. Results show that between 75.3\% and 89.6\% of nodes survived.  

\subsection{AppIS: Protect Android Apps Against Runtime Repackaging Attacks}\label{subsec:appis-2017}
%Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/AppIS-%20Protect%20Android%20Apps%20Against%20Runtime%20Repackaging%20Attacks%20-%20ICPADS_2017.pdf
In 2017, Song et al.\cite{8368344} proposed an app reinforcing framework, named AppIS. The idea of AppIS is to add security units as guards with interlocking relationship between each other, in order to build redundant and reliable anti-repackaging checks.

\begin{figure}
  \includegraphics[width=\textwidth]{figs/AppIS-scheme.pdf}
  \caption{The AppIS protection scheme.}
  \label{fig:appis-scheme}
\end{figure}

\paragraph{Protection scheme:}
Fig. \ref{fig:appis-scheme} depicts the protection workflow of AppIS. The AppIS workflow begins by parsing the compiled $apk$ to extract its corresponding function call graph (Step 2.1), leveraging static analysis techniques at the state of the art. From such graph, AppIS selects a set of sensitive methods, resources or data to protect (Step 2.2), named \textsl{goals}.  Then, AppIS generates a set of guards aimed to protect goals (Step 2.3). Guards can be hosted both in the bytecode (i.e., \longstring{J\_Guard}) and the native code (i.e., \longstring{N\_Guard}). Each goal must be controlled at least by a guard (\longstring{Guard-Goal}) and each guard must be likewise controlled by at least two other guards (\longstring{Guard-Guard}) to improve redundancy and reliability to attacks. According to previous rules, AppIS generates a set of Guard-Goal and Guard-Guard constraints (Step 2.4), which are taken into consideration to build a set of \textsl{guarding nets} among goals and guards, that satisfies all constraints. Moreover, such set is used to construct a scheduling engine that at runtime chooses which guarding net to activate, according to the triggered goal and the execution status. Finally, AppIS builds and delivers the protected $apk$, containing goals, guarding nets and the scheduling engine.

\paragraph{Runtime Behavior:} At runtime the scheduler generates a guarding net (Step 6.1). In this way, a different guarding net is generated at each execution, in order to make the app resilient against cumulative attacks (i.e., multiple execution of the app in a sandboxed environment to detect guards). 
During the execution (Step 6.2), whenever a guard is triggered (Step 6.3), the corresponding guards check the integrity of the goal (i.e., \longstring{J\_Guard}) or the guard (i.e., \longstring{N\_Guard}) (Step 6.4) by comparing the checksum of the goal calculated during the static construction (i.e., Steps 2.3 to 2.5) with the checksum obtained at runtime on the same goal (Step 6.4). If the two checksums do not match, each guard detects a repackaging and the app is directly terminated.

\begin{figure}[!ht]
  \includegraphics[width=\textwidth]{figs/AppIS-scheme-runtime.pdf}
  \caption{AppIS: runtime behavior.}
  \label{fig:appis-runtime}
\end{figure}


%\paragraph{Node construction}
%Guards assure that certain goals (methods, resources or data) are not tampered. Each goals is protected by at least one guard. Goal guard are written in Java (J\_Guard), and their security is monitored by at least other two nodes called guard-guard. These can both written in Java or C/C++ language (N\_Guard) triggered calling the JNI interface.
%To protect against cumulative attack, the guards net is computed when the app is started. In each execution the guards construction net will be totally different. 

%\paragraph{Tampering detection}

%\paragraph{Repackaging response}
%When a repackaging is detected the program is terminated directly.

\paragraph{Evaluation:}
AppIS improves the previous proposals by adding networks of guards and a non-deterministic behavior at runtime, that complicates the attacker analysis activity. AppIS has been evaluated on a very reduced set of only 8 apps, collected from different sources, on almost outdated Android versions (spanning from 4.4 to 6). Experimental results indicate that no app fails, and overheads are reasonable w.r.t. the previous proposals; in fact,  the space overhead is up to 2\% in the worst case, while time overhead spans from 2\% to 140\%. However, we argue that the reduced number of apps is statistically insignificant. %\luigi{Quanto è piccolo il campione lo dobbiamo dire? è composto da sole 8 apps}
The reliability of AppIS has been tested against two threats, namely the possibility for an attacker to i) obtain the collection of the guarding nets, and ii) to carry out cumulative attacks. According to the authors, in both cases the AppIS approach revealed to be reasonably robust.  
%The effectiveness of the protection is evaluated using Microsoft's risk assessment model (DREAD), to quantify the risk of attack. The following two threats were considered: 
%\begin{itemize}
 %   \item Attacker obtains static guarding net collection by reversing engineering. Rating: Medium
  %  \item Attacker launches cumulative attack to AppIS. Rating: Low
%\end{itemize}

\subsection{Self-Defending Code through Information Asymmetry}
\label{subsec:sdc-2018}
% Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Other%20Anti-Repack%20techniques/Leveraging%20Information%20Asymmetry%20to%0ATransform%20Android%20Apps%20into%20Self-Defending%0ACode%20Against%20Repackaging%20Attacks.pdf

In 2018, Kai Chen et al. in \cite{8186215} proposed a self-defending code (SDC) approach, leveraging the information asymmetry between the developer and the attacker on the app code, i.e., it is reasonable to assume that the attacker has far more less information than the developer on the app code, on average. Similarly to the approach discussed in Section \ref{subsec:dyn-self-prot-encrypt-2015}, the idea is to encrypt pieces of source code and decrypt (and properly execute) them at runtime only in case the app has not been repackaged. Unlike the previous work, each piece of code is encrypted with a different key.
The approach provides two schemes, where the first one requires to customize the Android OS, and the second one can work on unmodified OSes. We will focus on the latter one, as we argue that the first scheme cannot scale in the wild, due to the customization needs. 

\paragraph{Protection scheme:}
\begin{figure}
  \includegraphics[width=\textwidth]{figs/SDC-scheme.pdf}
  \caption{The SDC protection scheme.}
  \label{fig:sdc-scheme}
\end{figure}
The scheme (see Figure \ref{fig:sdc-scheme}) begins by analyzing the source code (Step 2.1) and selecting some qualified conditions (i.e., branches containing an equality check, where one of the operands is a constant value: i.e., \longstring{v==const}) in the code that need to be protected. A qualified condition is then substituted by a self-defending code (SDC) (Step 2.2) that hosts the encrypted version of the original code contained in the body of the qualified condition. Once all the pieces of code have been encrypted, a component named \textsl{runtime supporter} is built. Such component contains all the encryption routines which allow understanding how the modified code has been generated (Step 2.3); such routines are useful for reconstructing the original code at runtime.
It is worth pointing out that the encryption scheme is XOR-based and the key is related to the checksum of the original piece of code. Therefore, the original code can be decrypted correctly if and only if the app has not been modified. More in detail, w.r.t. to the sample code at Step 2.1 in Figure \ref{fig:sdc-scheme}, %\luigi{Forse non si capisce quale parte del sample code, quella dello step 2.1}
the information asymmetry between the developer and the attacker is the knowledge of the value \texttt{const}, removed from the source code at compiled time in Step 2.2, and the \longstring{encr\_code}. Furthermore, \longstring{encr\_code} is redundantly protected by a set of other - randomly selected -  SDC segments, some of which implement part of their functions as native code.  
Finally, the protected apk, composed by the DEX code extended with the SDC, the non-code resources and the runtime supporter, is built and delivered.

\paragraph{Runtime Behavior:} At runtime, whenever an SDC is executed, the encrypted code is decrypted by leveraging the app checksum xored with the \texttt{v} value as shown in Step 2.2. If one of these differs from the original values, the decryption fails and the original code is not retrieved, thereby leading the app to crash.
%\begin{figure}
%  \includegraphics[width=\textwidth]{images/sdc.png}
 % \caption{SDC encryption step}
  %\label{fig:sdc}
%\end{figure}
 
 

\paragraph{Evaluation:}
Differently from previous proposals, SDC has been validated on a significant set of apps (i.e., 20,000) taken from Anzhi \cite{anzhi} and belonging to 15 categories. For each app, a set of more than 100 candidate branches has been selected and substituted with SDC segments. The testing phase involved both real users and automatic testing. In the first case, ten  SDC segments where triggered in an hour, while, in the latter case,  five segments were triggered within 24 hours. The time overhead is below 4\% for each app tested, while the space overhead is negligible.

\subsection{BombDroid: Decentralized Repackaging Detection through Logic Bombs} \label{subsec:bombdroid-2018}
% Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/Resilient%20Decentralized%20Android%20Application%20Repackaging%20Detection%20Using%20Logic%20Bombs%20-%20CGO%202018.pdf
In 2018, Zeng et al. in \cite{10.1145/3168820} introduced the concept of \textsl{logic bombs} which are hidden (i.e.,  cryptographically obfuscated) pieces of code that execute once proper triggers (i.e., logical conditions) are activated. The authors implemented the approach in a tool called BombDroid. Like SDC (Section \ref{subsec:sdc-2018}), logic bombs are injected in qualified conditions.

\paragraph{Protection scheme:}
\begin{figure}[!ht]
  \includegraphics[width=\textwidth]{figs/BombDroid-scheme.pdf}
  \caption{The BombDroid protection scheme.}
  \label{fig:bombdroid-scheme}
\end{figure}
The protection scheme of BombDroid (see Figure \ref{fig:bombdroid-scheme}) is very similar to the SDC one, and the idea is to selectively find some candidate condition in the app methods to inject logic bombs. The first difference is that BombDroid works directly on the $apk$ at the bytecode level, and not on the source code. The BombDroid protection scheme begins by reversing the $apk$ (Step 2.1), and parsing the \longstring{classes.dex} file (Step 2.2) through static analysis techniques to identify suitable methods (Step 2.3). In each selected methods, BombDroid identifies at least a qualified condition containing an equality between a variable and a constant value (\longstring{v==const}, see Figure \ref{fig:bombdroid-scheme}). The original code - contained in the corresponding block - is extended with some checks aimed at detecting tampering, and then, encrypted. The encrypted code will be  decrypted at runtime according to the hash value of the variable plus a salt, selected by BombDroid. The decryption key is the value of the constant \texttt{v}. The use of a salt, instead of the checksum of the original method, is the main difference with SDC. The robustness of the scheme is likewise given by the robustness of the hash function, that do not allow guessing the value of \texttt{v}. Moreover, it is worth pointing out that the selected methods can have no qualified condition in principle: in this case, BombDroid can inject artificial qualified conditions to protect. Finally, BombDroid allows nesting logic bombs to improve stealthiness: for instance, with reference to the logic bomb in Step 2.4 of Figure \ref{fig:bombdroid-scheme}, another encrypted logic bomb can be inserted in the decrypted code between the original code and the tampering detection function. 

\begin{comment}
\paragraph{Node construction}

BombDroid rely on logic bombs to detect repackaging. Logic bomb idea, as shown in the original paper, is presented in \autoref{fig:logic-bomb}. 
Logic bombs are i%3CmxGraphModel%3E%3Croot%3E%3CmxCell%20id%3D%220%22%2F%3E%3CmxCell%20id%3D%221%22%20parent%3D%220%22%2F%3E%3CmxCell%20id%3D%222%22%20value%3D%22Step%202.4%22%20style%3D%22text%3Bhtml%3D1%3BstrokeColor%3Dnone%3BfillColor%3Dnone%3Balign%3Dcenter%3BverticalAlign%3Dbottom%3BwhiteSpace%3Dwrap%3Brounded%3D0%3BfontSize%3D12%3BfontStyle%3D0%22%20vertex%3D%221%22%20parent%3D%221%22%3E%3CmxGeometry%20x%3D%22317.78%22%20y%3D%22394.5%22%20width%3D%22144.48%22%20height%3D%2222.5%22%20as%3D%22geometry%22%2F%3E%3C%2FmxCell%3E%3C%2Froot%3E%3C%2FmxGraphModel%3Enserted inside \textit{qualified condition} (QC). A QC is a peace of code where a equality check between two operands (one of which is a constant value) is performed. QC can be found in original code, or artificial ones can be inserted.  
The constant value could be a string, integer or boolean values considering the obfuscation strong, medium or weak respectively. It is calculated the constant hash value using an hash function. In addiction, the original constant value is used to encrypt the QC content. Due to the one-way hash function property, it is hard for a reverse engineer guess the decryption key from the hash value. SHA-128 is the chosen hash function, and AES-128 the encryption function. The logic bomb encrypted payload is stored in a $.dex$ file. 

In order to hide bombs from attackers, authors proposed double-trigger bombs \autoref{fig:double-bomb}, where a second logic bomb is nested inside another one. The trigger condition and the payload of inner bombs are encrypted. The second trigger condition is based on environment parameters such as boot loader versions, brand names, API levels, OS versions, GPS position, and temperature value. With this features authors tried to protect from whitebox fuzzing for high code coverage.
\end{comment}

\paragraph{Runtime behavior:} At runtime, the logic bomb is executed, and the code is properly decrypted only if the value of the variable in the qualified condition is equal to \texttt{const} \footnote{This condition triggers the execution of \longstring{or\_code} in the original code of the candidate method.} and the logic bomb activates. 
Then, a tampering detection function is executed. BombDroid applies three anti-tampering techniques, i.e., at app level, at file level and at code snippet level. 
At compile time, BombDroid stores the original public key in the $apk$, as well as the values of some digests concerning resources and the \longstring{classes.dex} file, and some code snippets. At runtime, tampering functions calculate the digests of such resources and compare them with the stored one: tampering is detected whether one of such value differs from the stored one. In case a tampering is detected, the user could be warned or the app could cause negative user experience.

\paragraph{Evaluation:}
Authors assessed the reliability and the performance of BombDroid on a set of apps (i.e., 963) taken from F-Droid. They exploited Dynodroid \cite{10.1145/2491411.2491450} to execute each app for an hour, repeating the experiment 50 times per app. The execution time overhead is almost negligible (i.e., <2.7\%). The space overhead ranges from 8\% to 13\%. On average, the first logic bomb is triggered between 75 and 164 seconds after the app starts executing, and on average, only the 9.3\% of logic bombs are triggered. 

\subsection{Native Repackaging Protection}
\label{subsec:bombdroid-native-2019}
%Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/Repackaging_Protection__FPS_Paper%20-%202019.pdf
In 2019, 
Simon Tanner et al. in \cite{10.1007/978-3-030-45371-8_12} proposed an evolution of previous techniques. A prototype of this work is available on GitHub \cite{repackaging-protection}. Like BombDroid, this work is based on cryptographically obfuscated logic bombs, inserted in candidate methods with a qualified condition (i.e., \longstring{v==const}). However, the main difference is that integrity checks and a part of the original app code of the block are executed in native code. We refer this scheme as \textsl{Native Repackaging Protection}\footnote{Authors do no provide a name for this scheme.} (NRP). %The paper was published in 2019.

\paragraph{Protection scheme:} %\alessio{Re-write after modification of the corresponding figure.}
The NRP protection scheme, which mostly resembles the BombDroid and SDC ones, is depicted in Figure \ref{fig:native-bombdroid-evolution}.
\begin{figure}
  \includegraphics[width=\textwidth]{figs/native-bombdroid-evolution.pdf}
  \caption{The Native Repackaging Protection scheme.}
  \label{fig:native-bombdroid-evolution}
\end{figure}
Also in this case, NRP reverses the $apk$ (Step 2.1), parses the \longstring{classes.dex} file (Step 2.2), and finds (or builds artificial) blocks with a qualified condition. Then, it modifies each selected block as follows: i) given the standard condition \longstring{v==const}, NRP calculates the hash value of the constant (i.e., \longstring{HASH = H(const)}) using SHA-1 as the cryptographic hash function. Then, ii) the instructions of the block code (i.e., \longstring{or\_code}) are inserted in a new Java class which is encrypted using AES-128 in CTR mode, using the $const$ value as key. NRP applies several workarounds to preserve the semantic equivalence between the original code and the code contained in the encrypted Java class. Such class (i.e., \longstring{encr\_cl}) contains a single method \longstring{invoke()} which splits the original block code into two parts, namely \longstring{nat\_encr} and \longstring{or\_code2}. The first part refers to a native library which is likewise XOR-encrypted with a random symmetric key (i.e., $native\_key$). Such key is stored in the same encrypted Java class. To decrypt and execute the function \longstring{or\_nat\_code()}, stored in the \longstring{nat\_encr} library, a JNI call is required. \longstring{nat\_encr} contains an anti-tampering check that executes the first part of the original block code only if no tampering is detected. In current implementation, the integrity check verifies the signature of the first 100 bytes of the \longstring{classes.dex} file, whose path is hard-coded in the native library.

\begin{comment}
\paragraph{Node construction}

Like in Bombdroid and SDC, authors search for candidate blocks. A candidate block is an equality check between two operands (one of which is a constant value). The candidate block constant value is transformed in the correspondent hash value using SHA-1 function.
The code block instructions are extracted in a new Java class and encrypted using AES-128 in CTR mode. The key used is the candidate block constant value. Different workarounds are performed to preserve semantic equivalence between the original code and the ciphered corresponding class. Inside the extracted ciphered class a call to a native method is done using Java Native Interface (JNI). Integrity checking is performed inside the native code. In order to make mandatory the execution of the native code, a statement from the extracted block is translated and performed inside the native code. 
The native program code is encrypted with a random symmetric key stored in the encrypted Java class. Xor encryption is used to decode native code. The xor key is a resource, in their implementation case the first 100 bytes of classes.dex file.
\paragraph{Tampering detection}
In authors implementation, the signature of the first 100 bytes of the file \emph{classes.dex} is computed as integrity check. The path of that file is hard-code inside the native library.

\paragraph{Repackaging response}
In the published prototype, when tampering is detected the original ciphered code is not executed, leading to undefined behavior, .
\end{comment}


\paragraph{Runtime behavior:} During execution, the triggering of a logic bomb, depicted in Step 2.4 in Figure \ref{fig:native-bombdroid-evolution}, leads to the following execution: i) once the condition on the hash value is verified (i.e., \longstring{hash(v)==HASH}), the encrypted Java class (\longstring{encr\_cl}) is decrypted according to the constant value, and then the \longstring{invoke()} method is executed through Java reflection. The first statement (\longstring{nat\_encr}) is executed, and leads to the decryption of the native library (\longstring{nat\_encr}) and the execution of the \longstring{or\_code\_nat} block. Then, the signature of the first 100 bytes of the \longstring{classes.dex} file are checked. If the verification succeeds (i.e., \longstring{tamper\_check()==true}), then the first part of the original block code is executed (\longstring{or\_code1}), otherwise the app crashes. After the proper execution of \longstring{or\_code1}, the execution flow is returned to the \longstring{invoke()} method which executes the second part of the original block code (i.e., \longstring{or\_code2}).


\paragraph{Evaluation:}
NRP has been tested against 100 apps downloaded from the Google Play Store and F-Droid. Tests were performed on an LG Nexus 5X device, running Android 8.1.0. In their implementation, authors leverage the \longstring{dalvik.system.InMemoryDexClassLoader} to load the new Java class of each encrypted block. This functionality is available starting from Android 8.0, only. The empirical assessment showed that 47\% of apps could be transformed without runtime exceptions. Each app has been tested through Monkey \cite{monkey} to generate random user's input:  the time overhead is from 1.42\% up to 10.42\% (the space overhead is negligible), while on average, from 11 to 35 logic bombs have been activated. %\alessio{I would move the discussion on the implementation (it is commented now) in the attacking section. Thoughts?}

\begin{comment}
\textbf{Discussion}: We evaluated the tool starting from the source code and we recognized some issues that the authors did not took into consideration in their analysis. First of all, there is an undefined behavior in a native code tampering detection function, where a signed $char$ type is used, instead of an unsigned one which would have been consistent with the Java method. This leads to app instability. \alessio{Please explain why.} 
Furthermore, the authors did not verify the integrity of the user interface (UI). In some apps we encountered UI differences between the original and the protected app. \alessio{Again: what does it imply? Please explain.}
\end{comment}


==> [PMC] ARMAND Anti-Repackaging/sections/old_methodology.tex <==
\section{Methodology} \label{sec:methodology}
\begin{comment}
Main assumptions (description + advantages):
- multiple patterns
    - Things to avoid (e.g. which AT should be implemented and whats is its goals)
    - more QC in different location (non only for if stmt)
    - add also server checks -> ?!?
    - AT in logic bombs 
    - honeypots
- rely on native code
- Optimized pervasiveness of the logic bombs
    insert logic bomb with a criteria -> e.g. there are a lot of logic bombs in library, but not all are triggered or logic bombs in library can easily decrypted (an attacker can easily detected the encryption key) 
    - hash space -> ?!
- hiding (e.g. nested bombs/nested encryption,  obfuscation)
\end{comment}

In this work, we present \schema{}, a novel methodology that overcomes the main limitations of the current state-of-the-art approaches, by addressing the following challenges - already pinpointed in \cite{merlo2020you} - namely:

\begin{enumerate}
    \item \textbf{Use of multiple patterns} to disseminate and hide detection nodes in the app. Current techniques adhere to a common pattern (i.e., qualifying conditions and adoption of hash functions), which we showed to be rather easy to detect and de-activate by an attacker. To this aim, a novel approach must several - distinct - patterns for the detection nodes to harden the defusing and detection phase. Moreover, the content of the detection node must vary, i.e., use different anti-tampering controls, must be distributed throughout the entire app.
    \item \textbf{Rely on native technologies (C/C++)} to hide detection nodes, as reversing and instrumenting native code significantly increase the detection phase.
    \item \textbf{Optimize the effectiveness} of the detection nodes. Some approaches implement few controls in the name of performance, while others embed many bombs that are not actually triggered at runtime. In this respect, there is a need for more effective deployment of detection nodes, also at the cost of higher time and space overheads.
    \item \textbf{Use Honeypot bombs}. Proper fake bombs can be added to disguise the attacker to remove them. The removal of such bombs should trigger the real ones and lead the app to crash. This idea has been proposed in literature but never actually applied in current proposals, where the focus is more on generating stealthy logic bombs. 
    \item \textbf{Hide the anti-repackaging protection}. It is fundamental to improve the stealthiness of anti-repackaging controls and detection nodes to make it hard for the attacker to understand that the reverse-engineered app includes a protection scheme. Therefore, the new scheme must rely on hiding techniques like obfuscation \cite{} or packing \cite{}. \luca{TODO add citation}
\end{enumerate}

In the rest of this Section, we highlight the main features of \schema{} and detail the protection behavior at runtime. 


\subsection{Multi-patterning \& Anti-Tampering checks} \label{subsec:spatternization} 
% Multiple Patterns and Multiple Anti-Tampering Checks
The distribution of logic bombs affects the robustness of the anti-tampering technique. Unfortunately, current proposals rely on the sole pattern summarized in Section \ref{sub:anti-repackaging}, in which any qualified condition is systematically substituted with on some hash value and the body code encrypted according to the \texttt{const} value. Such pattern can be straightforwardly detected by the attacker through static analysis based on pattern matching (see \cite{merlo2020you} for further detail on attack vector to anti-repackaging). As a consequence, current anti-repackaging proposals are more concerned on spreading a high number of logic bombs rather than hiding the portion on code in which an anti-tampering check can be contained. 
From an attacker's point of view, the knowledge of this well-known pattern allows revealing the potential location of the anti-tampering detection nodes (i.e., all branching containing hash values in their condition) and automate their removal. 

We argue that adopting a multi-pattern distribution of logic bombs can increase the effort of the attacker and reduce the likelihood to remove the whole set of logic bombs.

\paragraph{Multiple logic bomb patterns:}  As introduced above, an attacker can leverage a single combination of function calls to detect the hash-based logic bombs. To counteract this threat, we build logic bombs according to the classical pattern, but we modify their inner code. In this way, even if an attacker detects several logic bombs, she is not able to decrypt them and recover the original code with a single procedure because each bomb has a different inner structure.
More in detail, we adopt six different types of logic bombs:
\begin{enumerate}
    \item \textbf{Honeypots} are fake logic bomb, which do not contain any anti-tampering check. Honeypots aim at tricking the attacker to spend time and effort to uselessly decrypt them.
    \item \textbf{Java bombs} that contain one or more Java anti-tampering checks. 
    \item \textbf{Native-key bombs} are made by encrypted inner code where the decryption key is the return value of an anti-tampering check that is implemented in the native code. 
    \begin{figure}[!ht]
      \includegraphics[width=1.05\textwidth]{figs/native_encryption_procedure.pdf}
      \caption{Creation process of a native key bomb}
      \label{fig:native_encryption_procedure}
    \end{figure}
    Figure \ref{fig:native_encryption_procedure} shows the creation process of this type of bomb. Here, the qualified condition is transformed into the form of the logic bomb (Step 1). Inside the qualified condition a native call is embedded (Step 2) and its return value is used to encrypt the \texttt{or\_code} (Step 3). Then, proper instructions to decrypt and run \texttt{or\_code\_encr} are added (Step 4). In this way, the \texttt{inner\_code} contains the native invocation, the decryption process and the invocation of \texttt{or\_code}. Finally, the \texttt{inner\_code} is encrypted with the \texttt{const} value in the qualified condition (Step 5).  
    \item \textbf{Native AT bomb} implements an anti-tampering check inside the native code. Differently from the previous cases, if the native AT check fails the normal app workflow is broken (i.e. an exception is thrown). In future versions, different actions can be implemented once a tampering is detected.
    \item \textbf{Java AT \& Native key bomb} are bomb analogous to the previous type, but \texttt{or\_code} contains at least one Java anti-tampering check.
    \item \textbf{Java \& Native AT bombs} contain both Java and native anti-tampering checks.
\end{enumerate}
% \antonio{In future work and enhancement section cite that the native call can inserted randomly inside the inner\_code}

\paragraph{Beyond logic bombs:} In addition to logic bombs, it is necessary to embed heterogeneous anti-tampering controls throughout the app. We inserted some detection nodes which check the application integrity. These nodes, called \textbf{Java AT}, are spread through the Java bytecode.
If all detection nodes rely on the same anti-tampering control, an attacker would bypass it to create a working repackaged app.
In our work, each anti-tampering node checks different things, and it detects a \emph{specific type} of repackaging. 
For example, file integrity checks detect a repackaging if and only if the verified file is changed during the repackaging process.
More in general, checking the signature can potentially detect all repackaging: an attacker have to re-sign the repackaged version of the app with his private key (that is different from the developer one).
Furthermore, these checks can be implemented both in Java and native code, in order to increase the amount of work an attacker need to carry out to circumvent these controls.

\paragraph{Deployment of logic bombs:} Another important aspect is where logic bombs are deployed and how anti-tampering checks are inserted. 
In our previous analysis, we notice that some logic bombs could be decrypted only by relying on reverse engineering and open-source information. An example is a logic bomb inserted inside an external open-source library. From the point of view of the defensive technique, these bombs do not add security but only increase the time overhead in the repackaging process.
One of the powerful technique that an attacker can use in the repackaging process is \emph{code instrumentation and injection}\footnote{discussed in \cite{merlo2020you}}, which allow dynamically modification of the code, intercepting function calls, and changing input or return values.
To make the reversing process harder, an anti-tampering control (both in Java and native code) is inserted replicating its bytecode (or assembly code) each time. In this way, we do not rely on a static anti-tampering function that is called from each detection node, despite there is and higher size overhead.



\subsection{Rely on native code}
The reverse engineering and the instrumentation process of native code (assembly code) are more complicated than Java bytecode. Due to this, interacting with native code can increase the difficulty of the repackaging process. 
To interact with native functions, a Java class has to load the shared object (usually with the directive \longstring{System.loadLibrary} \cite{android-jni}) and declare a method with the \texttt{native} keyword (this method tells the virtual machine that the function is implemented in the shared library). Moreover, there are several constraints to be respected (e.g., the name of a native function) when dealing with JNI. Due to this, a native function call could be detected easily. To avoid that an attacker easily removes the call to a native anti-tampering check (e.g., through \emph{code deletion}), the Java code should be dependent on the result of the native function.
To this aim, we identified two kinds of native invocation: \textbf{native key} and \textbf{native AT} (described above in Section \ref{subsec:spatternization})

%JNI spec: https://docs.oracle.com/javase/7/docs/technotes/guides/jni/spec/jniTOC.html

\subsection{Hiding protection}
Logic bombs are a first attempt to hide detection nodes, in which one or more anti-tampering controls can be embedded. Furthermore, logic bombs can be nestedly hidden, i.e., the content of a logic bomb hides another encrypted payload. In this way, an attacker has to decrypt all nested logic bombs to recover and remove the anti-tampering checks.
As we mention above, logic bombs and anti-tampering controls have common patterns that help an attacker in the detection of anti-tampering controls. Obfuscation can be applied to the protected app to hide common features and make hard the repackaging process for an attacker (i.e., detection of logic bombs or anti-tampering checks). 
In our work, we implemented this solution by relying on Obfuscapk \cite{aonzo2020obfuscapk}. 

In conclusion, these considerations lead us to create a protection scheme in which i) there are multiple patterns for logic bombs, ii) logic bombs are inserted through the code with specific and semi-stochastic criteria, iii) other heterogeneous detection nodes are inserted \emph{randomly} in the code and not only inside the logic bombs and iv) there are multiple anti-tampering checks (e.g., signature check, file integrity, package name check) in both Java and native code. % and v) detection nodes are hidden.

\subsection{Runtime behavior}
At runtime, the Java anti-tampering spread out the Java code and the logic bombs are executed. The code in logic bombs is properly decrypted only if the value of the variable (\texttt{v}) in the qualifying condition is equal to \texttt{const}. Then, if the logic bomb contains at least one anti-tampering function, a tampering check is executed. These functions calculate some digests and compare them with the stored one: tampering is detected whether one of such value differs from the stored one. In case tampering is detected, the app crashes and throws an exception. The type of the exception depends on which anti-tampering is executed.

As an example, for native key logic bombs, the native anti-tampering returns the key to decrypt the next code. If tampering is detected, the native function returns a wrong value (i.e., return a wrong decryption key). In this scenario, the $AES$ decryption function fails, throwing an exception.

==> [PMC] ARMAND Anti-Repackaging/sections/relatedworks.tex <==
\section{Related Works} \label{sec:related_works}

In recent years several anti-repackaging schemes have been proposed to protect Android apps from repackaging, relying on external AT checks or internal AT agents.

The proposals based on external AT agents include all the techniques that leverage a third-party entity to carry out anti-tampering checks. Examples are remote servers \cite{10.1145/2995306.2995315}, some third-party $apk$ or OS kernel modules \cite{10.1007/978-3-030-05234-8_16}. Albeit promising, those schemes suffer from communication-based vulnerabilities \citep{7299933, 8068748} that could interfere with the protection mechanisms. Furthermore, app developers cannot assume the presence of third-party solutions installed on the device, thus limiting the efficacy of such anti-repackaging proposals in the wild.

Regarding the anti-repackaging solutions based exclusively on internal AT checks, the scientific community proposed six different protection schemes, as surveyed in \cite{merlo2020you}.
The first proposal appeared in 2015 by Protsenko et al. \cite{7299906}. The authors put forward an anti-repackaging scheme that encrypts the \texttt{classes.dex} files in the $apk$, and dynamically decrypts and executes them at runtime. The adoption of a XOR-based encryption of the bytecode is aimed at implementing a tamper-proof checksum. 
In 2016, Luo et al. \cite{7579771} proposed the Stochastic Stealthy Network (SSN). The SSN scheme distributes (and hides) a set of guards into the app source code. When executed, such guards trigger some decision points that use stochastic functions to detect tampering.
Song et al. (2017) \cite{8368344} proposed an app reinforcement framework, named AppIS. The idea of AppIS is to add security units as guards with an interlocking relationship between each other to build redundant and reliable anti-repackaging checks. The guards can be included both in Java and native code.
Chen et al. (2018) \cite{8186215} proposed a self-defending code (SDC) scheme, leveraging the information asymmetry between the developer and the attacker on the app code. The idea is to encrypt pieces of source code and decrypt (and properly execute) them at runtime only in case the app has not been repackaged. Unlike the previous works, each piece of code is encrypted with a different key.
Zeng et al. (2018) \cite{10.1145/3168820} introduced the concept of \textsl{logic bombs} as anti-repackaging protections for Android apps. The approach consists of adding cryptographically obfuscated pieces of code that are executed once proper triggers (i.e., logical conditions) are activated. The authors implemented the approach in a tool called BombDroid.
Tanner et al. (2019) \cite{10.1007/978-3-030-45371-8_12} proposed an evolution of previous schemes. Like BombDroid, this work is based on cryptographically obfuscated logic bombs, inserted in candidate methods with a qualified condition. However, the main difference is that integrity checks - and parts of the original app code - are executed in native code.

Unfortunately, we discovered \cite{merlo2020you} that all the prevision proposals can be potentially circumvented by leveraging static and dynamic detection and neutralization techniques such as code analysis and pattern matching, dynamic testing, and symbolic execution. Moreover, we conducted a full-fledged attack on the latest - and more advanced - anti-repackaging scheme whose code is available on GitHub. 

==> [PMC] ARMAND Anti-Repackaging/sections/results.tex <==
\section{Empirical Evaluation} \label{sec:experimental_result}
 
We empirically assessed the reliability of \toolname{} by applying the tool over a set of 30.000 real-world Android apps downloaded from F-Droid \cite{f-droid} and Google Play \cite{google-play-store} between August and October 2020 (cf. Section \ref{sec:experiments}). Then, we evaluated the best set of input parameters using a subset of 1.000 randomly-selected apps (cf. Section \ref{sec:parameter_tuning}). Finally, we compared the run-time performance between the standard and the protected version on a subset of 220 apps to evaluate the computational overhead and the effectiveness of the \schema{} protection scheme (cf. Section \ref{subsec:effectiveness}).

%Then, we assessed the time and space overhead of the protections inserted by \toolname{} by testing 220 apps at run-time. 

\subsection{Experimental results}\label{sec:experiments}

The experiments were conducted on a Virtual Machine running Ubuntu 20.04 with 16 dual-core processors and 32GB of RAM. The experimental evaluation used the following parameters: $P_{Java\_AT}=10\%$, $P_{native\_encryption}= 40\%$, $P_{native\_AT}=60\%$, and $PN=ApplicationId$. During our test, we enforced a timeout of 1.200 seconds for the protection process.

\toolname{} was able to successfully protect 27.656 out of 30.000 apps (i.e., 92.2\%) in nearly 14 days and 5 hours (1.228.009 seconds). 
%In the experimental evaluation we setted $P_{Java\_AT}=10\%$, $P_{native\_encryption}= 40\%$, $P_{native\_AT}=60\%$, and $PN = ApplicationId$.
The analysis of the 2.344 remaining apps (i.e., 7.8\%) failed due to the following reasons: 

\begin{itemize}
    \item 986 apps (3.28\%) failed due to well-known issues of the Soot library\footnote{\url{https://github.com/soot-oss/soot/issues/1413}, \url{https://github.com/soot-oss/soot/issues/1474}};
    \item 963 apps (3.21\%) crashed during the tool transformation process;
    \item 229 apps (0.76\%) reached the timeout for the processing;
    \item 166 apps (0.55\%) crashed due to an issue of the Axml library \footnote{\url{https://github.com/soot-oss/soot/issues/1070}}.
\end{itemize}

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/javaAT-lb.pdf}
  \caption{Java AT \& logic bomb}
  \label{fig:protection-values-recap-java-at}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/nesting.pdf}
  \caption{Nesting level}
  \label{fig:protection-values-recap-nesting}
\end{subfigure}
\caption{Distribution of Java AT, logic bombs and nesting level of the protected apps (30.000 apps).}
\label{fig:protection-values-recap}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/graph-processing-time.pdf}
  \caption{Processing time (sec)}
  \label{fig:overhead-recap-time}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/graph-size-overhead.pdf}
  \caption{Size overhead (MB)}
  \label{fig:overhead-recap-space}
\end{subfigure}
\caption{Distribution of processing time and size overhead throw of the protected apps (30.000 apps).}
\label{fig:overhead-recap}
\end{figure}

\paragraph{\textbf{Protection Level.}} 
Figure \ref{fig:protection-values-recap} presents the distribution of the protection mechanisms (i.e., Java AT, logic bombs, and the nesting level) injected by \toolname{} over the set of the protected apps.
The results show that \toolname{} successfully includes a fair amount of logic bombs (i.e., 173 on average - distributed among the six possible types) and Java AT checks (i.e., 355 on average). 
Furthermore, the average nesting level of the logic bombs is greater than two (i.e., 2.3), as shown in Figure \ref{fig:protection-values-recap-nesting}.

%Furthermore, the average nesting level of those bombs is more than two (i.e, 2.3), thus enhancing the difficulty for their removal. In addition, Figure \ref{fig:protection-values-recap-nesting} shows that the majority apps have a nesting level higher than 2 (i.e, 2.3).
\begin{comment}
% di nuovo questa parte la metterei nella parte delle limitazioni
Nevertheless, there are a few exceptions. Indeed, for apps with a limited set of qualified conditions, the tool may introduce a small set of bombs that do not cover all the six possibilities. To this aim, there are a lot of apps with the number of Java AT and logic bombs in the first range of Figure \ref{fig:protection-values-recap-java-at} and Figure \ref{fig:protection-values-recap-lb}.
However, it is worth noticing that such a problem can be overcome by using a more permissive package name to cover, for instance, the entire app (i.e., setting \texttt{PN} to \emph{none}) and not only the $ApplicationID$ package.
\end{comment}

\paragraph{\textbf{Processing Time.}} 
\toolname{} took 1.228.009 seconds (14 days and 5 hours) for protecting all the apps, with an average time of 48 seconds per app (cf. Figure \ref{fig:overhead-recap-time}), thereby suggesting that the approach is viable. 
The building time is mostly under 2 minutes for most of the analyzed apps (i.e., 26.103 apps), even for those containing many qualified conditions. 
During the experimental evaluation, only 229 reached the timeout. 

\paragraph{\textbf{Space Overhead.}}
%Figure \ref{fig:overhead-recap-space} depicts the size overhead distribution of processed apps.
The total space overhead is due to two factors: a fixed amount (calculated as less than 1MB) introduced by the transformation and packaging processes of \toolname{} and a dynamic one related to the number of added detection nodes. 
As expected, the number of introduced Java AT controls and logic bombs is directly proportional to the space overhead since each security control contributes to increase the payload size of each method. 
Furthermore, since native functions are compiled into a shared object for each architecture and embedded into the app, the space overhead is also affected by the number of native controls. 

Still, Figure \ref{fig:overhead-recap-space} shows that the vast majority of apps (i.e., 25.938 out of 27.656) have a size overhead less than 6MB, with 4.3 MB on average. All in all, it is worth noticing that only 41 apps violate the size limit of 100MB, imposed by several app stores, such as Google Play \cite{limit-size-android-apk}. For these apps, the average size overhead is 7.5MB, which means that the original apps already have a size near the limit (i.e., the average initial size is 96.7MB).

\subsection{Parameters Tuning}
\label{sec:parameter_tuning}

As \toolname{} uses three input parameters (i.e., $P_{Java\_AT}$, $P_{native\_key}$, and $P_{native\_AT}$) to determine the probability to include the Java AT checks and the six types of logic bombs, 
we conducted tuning tests to detect the on-average best combination of parameters to ensure a reasonable trade-off between the space and time overhead and the protection level. 

To do so, we computed fifteen different combinations of $P_{Java\_AT}, P_{native\_key}$, $P_{native\_AT}$. We used a testbed of 1.000 randomly-selected Android apps to evaluate i) the average number of injected Java AT and logic bombs, ii) the average nesting level, iii) the time required for the computation, and iv) the size overhead of the protected apk.
The results of the assessment, reported in Table \ref{table:params_compare}, lead to some considerations. For the evaluations, we set the $PN$ as $ApplicationID$. 

\begin{table}[]
\begin{tabular}{|c|c|c||c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{\cellcolor[HTML]{CCFFFF}\begin{tabular}[c]{@{}c@{}}\% Java\\ AT\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{CCFFFF}\begin{tabular}[c]{@{}c@{}}\% Native\\ key\end{tabular}}} &
  \multicolumn{1}{c||}{\textbf{\cellcolor[HTML]{CCFFFF}\begin{tabular}[c]{@{}c@{}}\% Native\\ AT\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Avg. Java\\ AT\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}Avg. LB}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Avg. \\Nesting\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Avg. Protection \\ time (s)\end{tabular}}}&
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Avg. Size \\ overhead (MB)\end{tabular}}} \\ \hline
\multirow{4}{*}{5} & 30 & 30 & 87 & 95 & 2.4 & 22 & 2.44 \\\cline{2-8}
     & 80 & 20 & 86 & 92 & 2.2 & 23 & 2.73 \\\cline{2-8}
     & 60 & 40 & 86 & 94 & 2.1 & 23 & 2.66 \\\cline{2-8}
     & 40 & 60 & 87 & 95 & 2.1 & 22 & 2.67 \\\cline{2-8}
     & 20 & 80 & 87 & 95 & 2.1 & 23 & 2.66 \\\hline
\multirow{4}{*}{10} & 30 & 30 & 174 & 92 & 2.2 & 23 & 2.56 \\\cline{2-8}
     & 80 & 20 & 172 & 88 & 2.1 & 24 & 2.72 \\\cline{2-8}
     & 60 & 40 & 170 & 89 & 2.1 & 23 & 2.68\\\cline{2-8}
     & 40 & 60 & 174 & 91 & 2.1 & 23 & 2.67 \\\cline{2-8}
     & 20 & 80 & 171 & 90 & 2.1 & 23 & 2.66 \\\hline
\multirow{4}{*}{20} & 30 & 30 & 348 & 85 & 2.1 & 25 & 2.58 \\\cline{2-8}
     & 80 & 20 & 344 & 82 & 2.1 & 26 & 2.77 \\\cline{2-8}
     & 60 & 40 & 345 & 83 & 2.1 & 25 & 2.69\\\cline{2-8}
     & 40 & 60 & 349 & 84 & 2.1 & 25 & 2.68 \\\cline{2-8}
     & 20 & 80 & 345 & 84 & 2.0 & 24 & 2.68 \\\hline
\end{tabular}
\caption{Results of the input parameters tuning experiment (1.000 apps).}
\label{table:params_compare}
\end{table}

In all cases, the average nesting level of bombs is greater than 2, while the average number of included \toolname{} detection nodes (i.e., the sum of Java AT and the six types of logic bombs) ranges from 178 to 440. Such results ensure that all the apps are equipped with complex and hard-to-remove bombs despite the different input parameters. 
Regarding the space overhead, the results underline that the variation of the input parameters does not significantly affect the size of the protected apps: most apps have a size overhead of less than 6MB, with an average value around 3MB.

Finally, the experiments underline that most of the overhead in the processing time is due to the percentage of Java anti-tampering checks ($P_{Java\_AT}$). 
On the contrary, the percentage of native key ($P_{native\_key}$) and native AT ($P_{native\_AT}$) do not significantly affect the compilation time. 
To this aim, a reasonable configuration should use a low percentage value of Java AT (e.g., 10\%), but can set a higher percentage of native AT and native key bombs (e.g., between 40\% and 60\%).

\subsection{Runtime Performance}\label{subsec:effectiveness}

The last set of experiments aims at evaluating the effectiveness and usability of the \schema{} protection scheme in real-world Android apps.

To do so, we randomly-selected 200 apps protected with \toolname{}, and we analyzed them at runtime to check if the introduced protection does not affect the standard behavior of the app. The selected apps have an average of 95 Java AT and 50 logic bombs to ensure relevant results. 
Furthermore, we also tested the corresponding original apps to evaluate the runtime overhead introduced by the \schema{} protection.

For the testing phase, we used an emulated Android 8.0 phone equipped with a dual-core processor, 2GB of RAM, and the latest version of Google Play Services. We executed each app - original and protected one - for three minutes with the same high-level inputs (i.e., inputs that trigger an active element of the activity/view), and we retrieved the percentages of CPU and memory usages of each app every two high-level inputs. 

At the end of the experiments, 191 protected apps (i.e., 87\%) ran correctly without exceptions. The remaining 29 (i.e., 13\%) either thrown a new exception and crashed (i.e., 23 protected apps) or resulted in being unusable due to the high overhead introduced (i.e., 6 protected apps).

%Then, we executed the 191 protected apps and the 191 corresponding original ones to evaluate the run-time overhead introduced by the \toolname{} protection.
Figure \ref{fig:overhead-runtime-recap} reports the distribution of the CPU and memory overheads between the protected and the original app. 
The results show that the run-time overhead (i.e., CPU and memory usage) in the protected apps is negligible, with an average increase of 3\% in the CPU usage and 0.1\% in the memory usage and does not affect the user experience (i.e., no lags nor freezes).

Finally, it is worth noticing that the vast majority of the tested apps (i.e., 180 apps) have a CPU overhead less than 10\% and a memory overhead less than 0.5\%. 
%Due to this, the user does not notice relevant \antonio{non ho capito i commenti di Alessio} impact of the app usability, despite the execution of several \emph{Java AT} and \emph{logic bombs} (i.e., in the worst case 1669 Java ATs and 729 logic bombs).

%\antonio{Solo per chiarezza: l'overhead è calcolato come (overhead app protetta) - (overhead app originale) per tutti i campioni diviso il numero di campioni. Ad esempio - se per una app X ci sono 3 campioni e l'utilizzo per l'app orginale risulta [(1,10); (2,12); (3,8)], mentre per quella protetta [(1,16); (2,4); (3,9)], allora l'overhead per l'app X è = $((16-10)+(14-12)+(9-8))/3 = (6+2+1)/3 = 3\%$. Inoltre ci sono solo 3 app con overhead di cpu maggiore del 40\% ed il caso pessimo di overhead cpu è 77\% e di overhead memoria è di 0.9\%}


\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/cpu-overhead.pdf}
  \caption{CPU usage overhead (\%)}
  \label{fig:cpu-overhead}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/memory-overhead.pdf}
  \caption{Memory usage overhead (\%)}
  \label{fig:memory-overhead}
\end{subfigure}
\caption{Distribution of the CPU and memory usage overhead during the runtime experiments (220 apps).}
\label{fig:overhead-runtime-recap}
\end{figure}



==> [PMC] ARMAND Anti-Repackaging/sections/results_old.tex <==
\section{Experimental} \label{sec:experimental_result}
%In this section, we will focus on the experimental data we acquired during the testing and evaluating phases. 

We empirically assessed the reliability of \toolname{} by applying the tool over a set of 30.000 real-world Android apps downloaded from F-Droid \cite{f-droid} and Google Play \cite{google-play-store} between August and October 2020 (cf. \ref{sec:experiments}). Then we evaluated

We empirically assessed the reliability of \toolname{} by applying the tool over a set of 30000 apps . 


The experiments were conducted on a Virtual Machine running Ubuntu 20.04 with 16 dual-core processors and 32GB of RAM. The experimental evaluation used the following parameters: $P_{Java\_AT}=10\%$, $P_{native\_encryption}= 40\%$, $P_{native\_AT}=60\%$, and $PN=ApplicationId$.

%Then, we assessed the time and space overhead of the protections inserted by \toolname{} by testing 220 apps at run-time. 

\subsection{Experimental results}
\label{sec:experiments}
The tool was able to successfully process 27656 out of 30000 apps (i.e., 92.2\%) in nearly 14 days and 5 hours (1.228.009 seconds). 
%In the experimental evaluation we setted $P_{Java\_AT}=10\%$, $P_{native\_encryption}= 40\%$, $P_{native\_AT}=60\%$, and $PN = ApplicationId$.
The analysis of the remaining 2344 apps failed due to \toolname{} transformation errors (i.e., 963 apps), Soot library's well-known issue\footnote{https://github.com/soot-oss/soot/issues/1413, https://github.com/soot-oss/soot/issues/1474} (i.e., 1215 apps) and Axml issues\footnote{https://github.com/soot-oss/soot/issues/1070} (i.e., 166 apps), which resulted in crashes during the analysis of the Java bytecode.
In addition, some protected apps (6115 out of the 27656 apps) have not been equipped with any anti-tampering protection mechanism due to the fact the package name inside the \longstring{AndroidManifest.xml} file contains few lines of Java bytecode (e.g., hybrid app or obfuscated app). For this reason, the tool does not find any candidate qualified condition suitable to embed logic bombs. For these apps, the input package name parameter should be modified properly.

Figure \ref{fig:protection-values-recap} shows the distribution of the protection mechanisms (i.e., Java AT, logic bombs, and the nesting level) over the set of the protected apps. Figure \ref{fig:overhead-recap} depicts the processing time and size overhead distributions.

\begin{figure}
\centering
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/java-at.pdf}
  \caption{Java AT distribution}
  \label{fig:protection-values-recap-java-at}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/lb.pdf}
  \caption{Logic bombs distribution}
  \label{fig:protection-values-recap-lb}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/nesting.pdf}
  \caption{Nesting level distribution}
  \label{fig:protection-values-recap-nesting}
\end{subfigure}
\caption{Protection values}
\label{fig:protection-values-recap}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/graph-processing-time.pdf}
  \caption{Processing time distribution}
  \label{fig:overhead-recap-time}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/graph-size-overhead.pdf}
  \caption{Size overhead distribution}
  \label{fig:overhead-recap-space}
\end{subfigure}
\caption{Processing time and size overhead values}
\label{fig:overhead-recap}
\end{figure}

\paragraph{Protection Level.} 
The results show that \toolname{} successfully includes a fair amount of logic bombs (i.e., 173 on average) distributed among the six possible combinations and Java ATs (i.e., 355 on average). Furthermore, the average nesting level of those bombs is more than two (i.e, 2.3), thus enhancing the difficulty for their removal. In addition, Figure \ref{fig:protection-values-recap-nesting} shows that the main part of the apps have a nesting level higher than 2.
Nevertheless, there are a few exceptions. Indeed, for apps with a limited set of qualified conditions, the tool may introduce a small set of bombs that do not cover all the six possibilities. To this aim, there are a lot of apps with the number of Java AT and logic bombs in the first range of Figure \ref{fig:protection-values-recap-java-at} and Figure \ref{fig:protection-values-recap-lb}.
However, it is worth noticing that such a problem can be overcome by using a more permissive package name to cover, for instance, the entire app (i.e., setting \texttt{PN} to \emph{none}) and not only the $ApplicationID$ package.

\paragraph{Processing Time.} 
Concerning performance, \toolname{} took 1228009 seconds for protecting all the apps, with an average time of 48 seconds per app, thereby suggesting that the approach is viable. The building time is mostly under 2 minutes (i.e., 26103 apps), even for apps having a lot of qualified conditions. During our test, we setted a timeout of 1200 seconds for the protection process. The protection process of 229 of 2344 (i.e., 9.8\%) apps failed due to the timeout is reached. 

\paragraph{Space Overhead.}
The total space overhead is due to two factors: a fixed cost (calculated as less than 1MB), and a dynamic cost related to the number of added detection nodes. In particular, we noticed that the number of Java anti-tampering controls and Native Key or Native AT bombs are directly proportional to the space overhead since they contribute to increase the payload size of each method. Furthermore, since native functions are compiled into a shared object for each architecture and embedded into the application, space overhead is directly proportional to the number of native methods. Finally, it is worth noticing that the average size overhead of protected app in the testbet is limited (only 4.3 MB). Furthermore, Figure \ref{fig:overhead-recap-space} shows that the vast majority of apps (i.e., 25938 of 27656) have a size overhead less than 6MB. All in all, it is worth noticing that only 41 apps violate the size limit of 100MB, imposed by several application stores, such as Google Play \cite{limit-size-android-apk}. For these apps, the average size overhead is 7.5MB, which means that the original apps have already a size near to the limit (i.e., average initial size is 96.7MB).

\subsection{Parameters Tuning}
Since \toolname{} carried out the code transformation according to the probabilities of injection, we conducted a tuning tests to detect the on-average best combination of parameters to ensure a reasonable trade-off between the space and time overhead and the protection level. To do so, we computed fifteen different combinations of $P_{Java\_AT}, P_{native\_key}$, $P_{native\_AT}$. We used a test-bed of 1000 randomly selected apps to evaluate the resulting average number of inserted Java AT, logic bombs, the average achieved nesting level of these bombs, and the average computation values (i.e., time of protection process and size overhead). For the experiments, we used the $ApplicationID$ of the app as \texttt{PN} to be processed. The results of the assessment, reported in Table \ref{table:params_compare}, lead to some considerations.

\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}\% Java\\ AT\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}\% Native\\ key\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}\% Native\\ AT\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Avg. Java\\ AT\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}Avg. LB}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Avg. \\Nesting\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Avg. Protection \\ time (s)\end{tabular}}}&
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Avg. Size \\ overhead (MB)\end{tabular}}} \\ \hline
\multirow{4}{*}{5} & 30 & 30 & 87 & 95 & 2.4 & 22 & 2.44 \\\cline{2-8}
     & 80 & 20 & 86 & 92 & 2.2 & 23 & 2.73 \\\cline{2-8}
     & 60 & 40 & 86 & 94 & 2.1 & 23 & 2.66 \\\cline{2-8}
     & 40 & 60 & 87 & 95 & 2.1 & 22 & 2.67 \\\cline{2-8}
     & 20 & 80 & 87 & 95 & 2.1 & 23 & 2.66 \\\hline
\multirow{4}{*}{10} & 30 & 30 & 174 & 92 & 2.2 & 23 & 2.56 \\\cline{2-8}
     & 80 & 20 & 172 & 88 & 2.1 & 24 & 2.72 \\\cline{2-8}
     & 60 & 40 & 170 & 89 & 2.1 & 23 & 2.68\\\cline{2-8}
     & 40 & 60 & 174 & 91 & 2.1 & 23 & 2.67 \\\cline{2-8}
     & 20 & 80 & 171 & 90 & 2.1 & 23 & 2.66 \\\hline
\multirow{4}{*}{20} & 30 & 30 & 348 & 85 & 2.1 & 25 & 2.58 \\\cline{2-8}
     & 80 & 20 & 344 & 82 & 2.1 & 26 & 2.77 \\\cline{2-8}
     & 60 & 40 & 345 & 83 & 2.1 & 25 & 2.69\\\cline{2-8}
     & 40 & 60 & 349 & 84 & 2.1 & 25 & 2.68 \\\cline{2-8}
     & 20 & 80 & 345 & 84 & 2.0 & 24 & 2.68 \\\hline
\end{tabular}
\caption{Tuning of \toolname{} input parameters on protection level, computation and space overhead}
\label{table:params_compare}
\end{table}

In all cases, the average nesting level of bombs is greater than 2, while the average number of included \toolname{} detection nodes (i.e, the sum of Java AT and the six types of logic bomb) ranges from 178 to 440. Such results ensure that - despite the input parameters - all the apps are equipped with complex and hard-to-remove bombs. 
Regarding the space overhead, the results underline that the variation of input parameters does not affect significantly the size of the protected apps: most apps have a size overhead of less than 6MB, with an average value around 4MB.

Finally, the experiments underline that most of the overhead in the processing time is due to the percentage of Java anti-tampering ($P_{Java\_AT}$). In details, the average protection time is directly proportional to the number of embedded Java anti-tamperings as those bombs introduce additional bytecode that will be processed. On the contrary, the percentage of native key ($P_{native\_key}$) and native AT ($P_{native\_AT}$) do not significantly affect the compilation time. Changing these values, the percentages of each logic bomb type is altered, but each app has the same number of candidate qualified condition.

\subsection{Runtime Performance}\label{subsec:effectiveness}
We randomly selected 220 apps with at least 5 Java AT and 3 logic bombs from the test-set and we automatically tested both the original and the protected ones at runtime to evaluate the impact of the \toolname{} protection on the performances of the protected app.
These apps have an average of 95 Java AT and 50 logic bombs. For the testing phase, we used an emulated Android 8.0 phone equipped with a dual-core processor, 2GB of RAM, and the latest version of Google Play Services. We executed each app - original and protected one - for few minutes with the same high-level inputs (i.e., inputs that trigger an active element of the activity/view) \antonio{Abbiamo un citazione per il lavoro di Andrea?!?} and we retrieved the percentages of CPU and memory usages of each app every 2 high-level inputs. 

191 out of the 220 protected apps (i.e., 87\%) executed correctly and no new exceptions were thrown. The remaining 29 protected apps (i.e., 13\%) thrown a new exception and crashed during the execution for issue introduced by the protection of \toolname{} (i.e., 23 protected apps), or resulted to be unusable due to the high overhead introduced (i.e., 6 protected apps), e.g., too many logic bombs in a single code snippet.

We collected the execution data for the 191 apps (i.e., the apps without new exceptions), which are exported and compared to evaluate the run-time overhead introduced by the \toolname{} protection. In particular, Figure \ref{fig:overhead-runtime-recap} reports the distribution of the CPU and memory overheads between the protected and the original app. 
These values shows that the runtime overheads (i.e., CPU and memory usage) in the protected apps are negligible, with an average increasing of 3\% in CPU usage and 0.1\% in memory usage. Due to this, the user does not notice relevant \antonio{non ho capito i commenti di Alessio} impact of the app usability, despite the execution of several \emph{Java AT} and \emph{logic bombs} (i.e., in the worst case 1669 Java ATs and 729 logic bombs).
\antonio{Solo per chiarezza: l'overhead è calcolato come (overhead app protetta) - (overhead app originale) per tutti i campioni diviso il numero di campioni. Ad esempio - se per una app X ci sono 3 campioni e l'utilizzo per l'app orginale risulta [(1,10); (2,12); (3,8)], mentre per quella protetta [(1,16); (2,4); (3,9)], allora l'overhead per l'app X è = $((16-10)+(14-12)+(9-8))/3 = (6+2+1)/3 = 3\%$. Inoltre ci sono solo 3 app con overhead di cpu maggiore del 40\% ed il caso pessimo di overhead cpu è 77\% e di overhead memoria è di 0.9\%}

Furthermore, Figure \ref{fig:cpu-overhead} and \ref{fig:memory-overhead} show that the vast majority part of the tested apps (i.e., 180 apps) have a CPU overhead less than 10\% and a memory overhead less than 0.5\%.  

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/cpu-overhead.pdf}
  \caption{CPU overhead distribution}
  \label{fig:cpu-overhead}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/memory-overhead.pdf}
  \caption{Memory overhead distribution}
  \label{fig:memory-overhead}
\end{subfigure}
\caption{Runtime analysis result}
\label{fig:overhead-runtime-recap}
\end{figure}



==> [PMC] ARMAND Anti-Repackaging/sections/security.tex <==
\section{Security Analysis}\label{sec:security}

According to the threat model in Section  \ref{sub:threat-model}, the goal of anti-repackaging is to include robust security controls that the effort required to remove them (Step 9) may be great enough to discourage the attacker from repackaging.

In such a scenario, the attacker has only two strategies to repack an app successfully. In the first case, she needs to detect and remove all the detection nodes spread in the app code. The second possibility is to tamper with the AT checks to avoid the repackaging detection (e.g., by overriding the return value of an anti-tampering function). 
Both strategies can leverage a \textsl{weapon rack} of techniques to analyze a protected $apk$ to detect and dismantle anti-repackaging protections. 
The weapon rack includes several static and dynamic techniques such as code analysis and pattern matching, dynamic analysis \& testing, and code manipulation techniques \cite{merlo2020you}.

In the rest of this section, we evaluate the reliability and robustness of \schema{}, explaining the difficulties for an attacker to deactivate the protection.

\subsection{Detection Nodes: Identification and Removal} 

All the six types of logic bomb in \schema{} hide under the same structure ($hash(v, salt) == H$). Nonetheless, each bomb has a different content, i.e., it can optionally i) include one or more AT checks, ii) rely on native code, and iii) contain other nested logic bombs.
Thanks to such a diversity, the attacker cannot infer a common pattern for the logic bombs, making difficult the adoption of automated detection and/or removal process. 
Furthermore, even if the attacker has the ability to detect all the patterns related to the logic bombs, she still has to find and circumvent the AT checks that are randomly spread in the app code and are external to any logic bomb.

The \schema{} protection scheme increases also the resiliency against dynamic analysis and automated testing techniques.
For instance, an attacker can leverage code instrumentation to intercept the call to the decryption function (e.g., AES decrypt) inside a logic bomb to recover the decryption key and the \texttt{inner\_code}.
However, thanks to the multi-pattern strategy adopted by \schema{}, an attacker has to manually analyze the content of each logic bomb to neutralize or remove the nested Java and/or native AT controls. 
Furthermore, the inclusion of nested logic bombs provide a higher level of protection: even if an attacker decrypts the first level, she needs to iterate the process to remove AT checks until she reaches the \texttt{or\_code}.

Under previous conditions, the attacker has to \emph{manually} execute most of the app code to be sure that all detection nodes are removed and bypassed, making the repackaging process extremely time and resource consuming, in particular if the \schema{} implementation distributes a lot of bombs, pervasively.

\subsection{Deactivation of AT checks} 

The attacker may avoid looking for detection nodes, and focus on deactivating the AT checks they invoke to verify the app integrity. \schema{} relies on several types of anti-tampering controls (e.g., signature checking and file integrity) selected using a pseudo-random heuristic, which is adopted both for Java and native code. 
In this way, an attacker has to find a different approach for each type (and implementation) of an AT check. Furthermore, the reverse engineering and instrumentation process of native code (assembly code) requires additional technical skills that increase the difficulty of the attack w.r.t. the Java part.
Also, \schema{} relies on cross-language AT controls, where the computation is split in both Java and native code. Such a dependency avoids the usage of \emph{code deletion} attacks since removing a native call invocation would break the expected execution of the Java code, leading the app to crash.
Finally, the code of the anti-tampering controls is replicated for each usage. In this way, the attacker must detect and tamper with all the AT check invocations to bypass the anti-tampering control.


==> sections/old paper files/attacking.tex <==
\section{Disabling Anti-Repackaging} \label{sec:attack} 

In this section we discuss how the attacking techniques previously discussed can be leveraged to disable the anti-repackaging techniques presented in Section \ref{sec:attacking_model}, and to build a fully working repackaged app. 
%We will shortly describe the novelty introduced in each work, and eventually try to attack them. 

Unfortunately, the vast majority of the older anti-repackaging techniques (i.e., described in Sections \ref{subsec:dyn-self-prot-encrypt-2015}, \ref{subsec:ssn-2016}, \ref{subsec:appis-2017}, \ref{subsec:sdc-2018} and \ref{subsec:bombdroid-2018}) have no available implementation to date. We tried to contact their authors via institutional emails, but we did not receive any positive answer (i.e., neither the source code nor a sample of a protected app). %\luigi{forse nelle parentesi precedenti ci manca il predicato? Oppure in inglese va bene così?} 
For this reason, we will just provide some motivated guidelines on how such techniques can be circumvented. 

However, the source code of the  native extension of BombDroid \cite{10.1007/978-3-030-45371-8_12}, described in Section \ref{subsec:bombdroid-native-2019}, is available as source code on GitHub \cite{repackaging-protection}. For this latter and more recent proposal, we describe a full-fledged attack able to circumvent all the anti-repackaging checks.

It is also worth noticing that none of the anti-repackaging techniques carries out any anti-debugging or emulation check. This basically simplifies the execution of cumulative attacks because the attacker is able to perform tests without worrying about emulator or debugging detection.


\subsection{Self-Protection through $dex$ Encryption}
The encryption method used to cipher the \texttt{classes.dex} file is a XOR encryption. This method could be easily extended to adopt more secure ciphers, like, e.g., AES; nonetheless, this would increase the runtime overhead.

Independently from the cipher, the main drawback of the proposal is that the  decryption key of the ciphered bytecode (i.e., the \texttt{classes.dex} file) is hardcoded in an obfuscated (via LLVM/OLLVM) native activity.  However, there is no need to statically de-obfuscate the native code to retrieve the key, as three dynamic analysis attacking techniques can be leveraged:
\begin{itemize}
    \item symbolic execution could reveal the decryption key and how it is obtained. This technique allows tracking several execution flows showing the value of the variables, including the decryption key;
    \item the debugger allows to detect the actual value of the key at runtime. To debug the app, the only modification is to change the value of the debuggable flag into the \emph{AndroidManifest.xml} file. This tampering is not detected by the XOR-based checksum at runtime;
    \item code instrumentation could allow retrieving the decryption key which is passed as parameter to the decryption function. Function calls could be intercepted with different tools (e.g., see the Frida script in Figure \ref{fig:native-dump-argument-frida}) in order to report back the the values of its arguments. 
    \begin{figure}[!htbp]
    \begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
    ]
    function inspectModule(module) {
      var m = Process.getModuleByName(module);

      Interceptor.attach(m.getExportByName("decrypt"), {}
        onEnter: function(args) {
          // Dump arguments
          send("Argument 1 of decrypt function" , args[0]);
          send("Argument 2 of decrypt function" , args[1]);
          [...]
        }
      });
    }
    \end{lstlisting}
    \caption{Frida script to dump arguments provided as input to the native method $decrypt$.}
    \label{fig:native-dump-argument-frida}
    \end{figure}
\end{itemize}
The access to the decryption key allows the attacker to decrypt any slice of ciphered code.
Furthermore, cumulative attacks can be performed to retrieve all the decrypted code using runtime memory dumping and process exploration. In this scenario, the attacker can dump each decrypted bytecode at runtime, thereby recovering the original code and she can leverage code manipulation (e.g., code deletion or binary patching) to add malicious code or remove anti-tampering controls. 

Once the code is recovered and tampered, one of the following approaches can be leveraged to create a working tampered $apk$ based on code deletion and binary patching:
\begin{itemize}
    \item override the body with the encrypted tampered code. This approach can be used only if a symmetric-key algorithm is used to encrypt and decrypt the code. In this way, once the attacker recovered the encryption key, she can perform both encryption and decryption.
    \item replace directly the body with the tampered code. In this scenario, the final app does not contains encrypted code.
\end{itemize}

\subsection{Stochastic Stealthy Networks} 
% Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/Repackage-proofing%20Android%20Apps%20~%20Stochastic%20Stealthy%20Network.pdf
% https://cse.sc.edu/~lluo/papers/ssn-robustness-2017.pdf, riassunto nel capitolo 2.1 di bombdroid

Several works \cite{Norboev2018OnTR, 10.1145/3168820, 10.1007/978-3-030-45371-8_12} have already pointed out some weaknesses of SSN, as well as some attacks that can be used to circumvent this protection. %\alessio{What I do not understand is whether we are reporting such already discussed attack in the following sentences, or we are reporting our attacks. } \antonio{both, we imagine (we cannot test them) some attacks that is confirmed by other papers}
 There are two ways to circumvent SSN, namely i) deactivating the integrity check or ii) detect and remove all the detection nodes from the code.

Concerning the first strategy, recall that each detection node implements the same integrity check on any candidate method, based on the developer's public key. Therefore, it is sufficient to analyze a single detection node to define a de-activation strategy. To this aim, code injection or vtable hijacking allow replacing the target method (\textit{getPublicKey} and \textit{generateCertificate}) with a custom implementation, which returns the original developer's public key, instead of the attacker's one. % which repackaged the app. %In this way we overcame all integrity checks.

Regarding the latter strategy, blackbox fuzzing can be used to generate a massive number of pseudo-random input in order to trigger all repackaging detection nodes (which are invoked stochastically) to detect them. In addition, whitebox fuzzing (or symbolic execution) can reveal the destination of the reflection calls.
Once all detection nodes are detected, either code deletion (i.e., to remove the repackaging detection nodes) or binary patching (i.e., to make the repackaging detection node unreachable) can be leveraged.

\subsection{AppIS: Protect Android Apps Against Runtime Repackaging Attacks}
%Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/AppIS-%20Protect%20Android%20Apps%20Against%20Runtime%20Repackaging%20Attacks%20-%20ICPADS_2017.pdf
The simplest way to repack an AppIS-protected app is to modify only parts (methods, resources or data), which are not protected by guards. It is possible to recognize whether an app snippet is protected through static analysis, as no code obfuscation is applied by AppIS.
Static analysis also allows obtaining the set of guarding nets, and delete them from the code. This is made possible by the fact that each guard has a specific design pattern %\alessio{which one? Can we say something about it? As we do not say anything on this in Section 3.} \antonio{authors do not specify how to implements the guard, but only a guarding net from a general point of view} 
 which the attacker can detect through bytecode analysis. In future works, the authors put forward the possibility to encrypt the set of guarding nets and decrypt it at runtime. Nonetheless, the encrypted guarding nets would be likewise vulnerable to deletion attack, as it is sufficient for the attacker to remove the parts of code where the decryption is carried out.
%Once we have been careful to remove the deleted guards from the guard-net generation at runtime, repackaging can be performed. 

Beyond removing guarding nets, it is also possible to bypass the integrity detection on the goals, by exploiting cumulative attacks to collect a large number of the original hash values. Then, such values can be hardcoded in the corresponding integrity detection methods. In this way, the attacker is able to bypass the anti-tampering controls without deleting the guarding nodes. 

\subsection{Self-Defending Code through Information Asymmetry}
% Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Other%20Anti-Repack%20techniques/Leveraging%20Information%20Asymmetry%20to%0ATransform%20Android%20Apps%20into%20Self-Defending%0ACode%20Against%20Repackaging%20Attacks.pdf
Recall that this approach is an improvement of the previous one: it moves the integrity checks to the native code and uses cryptographic obfuscation to resist static analysis.
Nonetheless, it remains vulnerable to several dynamic analysis techniques: first, blackbox fuzzing allows triggering a large number of SDC segments. For each triggered segment, a code instrumentation tool like Frida can be leveraged to hook the \texttt{encrypt} function in the \texttt{if} statement in order to recover the correct value of the variable \texttt{v}. 
%\antonio{1) blackbox fuzzing allow to trigger a lot of SDC segment 2) While the app is blackbox fuzzed, a code instrumentation tool can hook the decrypt function -> attack = blackbox (or other techniques to run the app with a lot of input, such as monkey) + code instrumentation (e.g. frida)} 
 Once this data is obtained, it is possible to retrieve the decryption key of the encrypted code, in both modes supported by this anti-repackaging technique. Then, code deletion can be leveraged to substitute an SDC segment with the original code, thereby deactivating the protection.
Previous attacks succeed only if all SDC sufficient for repackaging succesfully are discovered. %\luigi{In realtà ha successo solo se sono trovate tutte le sdc che ci permettono di raggiungere il nostro scopo (se la app si rompe dopo chissene frega)} 
Therefore, the robustness of this anti-repackaging technique is directly dependent on the number and the distribution of SDC statements in the app.

Finally, if the attacker is able to locate the checksum method in the native code (the anti-tampering control), she would override the body of such method through binary patching, in order to force it returning the excepted value. In this way, we would be able to tamper an application and bypass all checks with low effort. 

\subsection{BombDroid: Decentralized Repackaging Detection through Logic Bombs} \label{subsec:attack-bombdroid}
% Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/Resilient%20Decentralized%20Android%20Application%20Repackaging%20Detection%20Using%20Logic%20Bombs%20-%20CGO%202018.pdf
In BombDroid, any logic bomb follows the same, well-defined, specific pattern (i.e., \longstring{hash(v)==const}). Text search and pattern matching can be used to statically analyze the app source according to this pattern, in order to locate potential pieces of codes hiding logic bombs. However, code obfuscation could complicate this pattern-based search.
%\alessio{Could we have some problem with obfuscated apps?} \antonio{yes, obfuscation can limit static binary analysis}

Once a potential logic bomb is detected, the attacker can try to retrieve the decryption key (which is the constant value of the qualified condition) through dynamic analysis by leveraging:
\begin{itemize}
    \item \textbf{Brute force}: The attacker can try all possible values for the integer value \texttt{v}. Potentially, this key space is huge (i.e., \texttt{$2^{32}$}, as Java stores integer values in 4 bytes). Nonetheless, the actual distribution of valid constant values is smaller \cite{repackaging-protection}. Furthermore, there is a small number of unique constant values (i.e., in the range [-1024, 1024], according to the authors). %\alessio{I don't get the point clearly, what does it mean in practice? How much small?}. \antonio{From NRP paper, most of constant value are in range [-1024, 1024] and an attacker can easily use brute force to guess the value of the trigger condition. Moreover, exists significant value for constants (e.g. 0x0 is a null variable)}
    \item \textbf{Extraction of information from open source code}: If an app includes external open source libraries, and the static analysis recognize some potential logic bombs on such libraries, then an analysis of the original source code can allow guessing the right constant value of  \texttt{v}. 
    \item \textbf{Code instrumentation}: Proper code instrumentation applied on the potential logic bombs can allow intercepting the call to the decryption function (e.g., AES), thereby recovering the decryption key or the plain code (once the logic bomb has been triggered). 
\end{itemize}

Another way to retrieve the value of \texttt{v} is by means of cumulative attacks. In fact, as authors showed that at most 9.3\% of bombs are triggered using both state of the art Android fuzzing tools and human analysis, the detection and de-activation of such few logic bombs can suffice to obtain a repackaged app that works properly in the most of the cases. Put another way, this fact indicates that albeit BombDroid can add a lot of logic bombs, only few of them actually trigger.  Therefore, it is unnecessary for an attacker to delete each logic bomb, but she needs to remove just the mostly triggered ones on average.

Once a constant value is retrieved from a single-trigger bomb, the logic bomb could be deleted (i.e., deletion attack) and replaced directly with the (original) decrypted code. The attacker can also add some extra code to the original one.
It is worth noticing that the previous attacking procedure applies on nested bombs if all constant values (i.e., contained in all nested qualified conditions) are discovered. 

Another possibility is to bypass the anti-tampering checks contained in the encrypted code of the bomb (i.e., the \longstring{tampering\_detection} function in Figure \ref{fig:bombdroid-scheme}):
\begin{itemize}
    \item leverage code injection to replace the tampering detection function with an attacker-defined one;
    \item try a replay attack to modify the MANIFEST.MF file used in the code digest comparison checks. In this scenario, the anti-tampering controls compare the hardcoded values with the one in the original MANIFEST.MF file.
\end{itemize}

Recall that the BombDroid prototype relies on a tampering detection function based on a public-key comparison. Such function can be dynamically rewritten by instrumenting the Dalvik bytecode in order to return the expected value (i.e., the public-key of the original developer). %\alessio{I lost myself here: after rewriting (through which technique?) we force the function to provide what exactly as output? the public key of the original developer?} \antonio {yes, the hooked function return the original key that correspond to the expected value}
%Authors left the inclusion of other detection methods in future work.

\subsection{Native Repackaging Protection}
%Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/Repackaging_Protection__FPS_Paper%20-%202019.pdf
The Native Repackaging Protection is the most recent and advanced repackaging avoidance technique to date, as it inherits and extends methodologies and techniques from the other proposals. 
For previous anti-repackaging techniques, we have pinpointed some high-level attack patterns by leveraging the attacking techniques described in Section \ref{sec:attacking_model}, since no source code, nor any protected app have been made available. 
However, as the source code of NRP is publicly available, we were able to analyze it in detail and carry out an actual and full-fledged attack to this technique.
We will describe the attack in details by relying on a real app, i.e., Antimine~\cite{antimine-android}, an open source, minesweeper-like game app available on F-Droid (see Figure \ref{fig:antimine-fig}).

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\textwidth]{images/antimine.pdf}
    \caption{A snapshot of the Antimine game.}
    \label{fig:antimine-fig}
\end{figure}


More specifically, we will i) apply NRP to Antimine, showing how a candidate method is protected, ii) prove how such protection can be circumvented and iii) build a full-working repackaged version of the protected Antimine app. 

%e have the tool source code. An attacker could not have access to it, anyway it’s just a more time consuming process to exploit this approach.
%We ... For our test examples we will use .

As a preliminary remark, we found an implementation bug by analyzing the NRP source code: the tool statically pre-computes the signature of the \longstring{classes.dex} file through a Java function, while at runtime the protected app calculates this value by means of a native function (C/C++ code). The \texttt{char} type in standard C can either be signed [-128, +127] or unsigned [0, 255]. We found that the native function uses a char (line 3 on the left side of Figure \ref{fig:hash_bytes}) while the corresponding Java function adopts an unsigned char  (line 4 on the right side of Figure \ref{fig:hash_bytes}). As a consequence, a char value that has a bit representation with a \texttt{1*******} pattern (where \texttt{*} stands for 0 or 1) is interpreted as an int value between [-128,-1] by C and between [127,255] by Java. % (line 4 on the right side of Figure \ref{fig:hash_bytes}).
Therefore, if some chars of the \longstring{classes.dex} file have the \texttt{1*******} format, the integrity check always fails
- independently from the app being tampered or not. % - thereby leading the protected app to crash. %\alessio{Where does this inconsistency lead to? Explain.} \antonio{char value that has a bit representation 1******* (where * stands for 0 or 1) are interpreted as int value between [-127,-1] by C and between [127,255] by Java. Due to this, if some char of classes.dex match this form (1*******) then the integrity checks never pass (even without tampering) and the protected app always crash}

\begin{figure}
.
\begin{minipage}[t]{0.48\textwidth}
\begin{lstlisting}[language=C,
    basicstyle=\scriptsize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
    emphstyle=\underline,
    escapechar=ä,
]
// XOR in native code
int32_t hash_bytes(const char *arr, size_t count) {
  ä\underline{char hash[4];}ä// <-- Should be u_char
  for(size_t read = 0; read < count; read++) {
    hash[read % 4] ^= arr[read];
  }
  return hash[0] + (hash[1] << 8) + (hash[2] << 16) + (hash[3] << 24);
}
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{.48\textwidth}

\begin{lstlisting}[language=Java,
    basicstyle=\scriptsize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
    emphstyle=\underline,
    escapechar=ä,
]
// XOR in Java code
private static int xorFile(Path p, int count, int offset) throws IOException {
  byte[] content = Files.readAllBytes(p);
  ä\underline{byte[] res = new byte[4];}ä
  for(int i = offset; i < (offset + count); i++ ) {
    res[(i - offset) % 4] ^= content[i];
  }
  return (0xff & res[0]) + ((0xff & res[1]) << 8) +
    ((0xff & res[2]) << 16) + ((0xff & res[3]) << 24);
}
\end{lstlisting}
\end{minipage}
\caption{On the left side: the C code used to calculate the hash sum at runtime. On the right side, the Java code used to precompute the hash sum, at compile-time.}
\label{fig:hash_bytes}
\end{figure}

Moreover, the translation of the Java bytecode into native code could introduce some new exception. For instance, any single instruction in the Java bytecode influence, or is influenced, by other instructions (for example the comparison between two variables). It is mandatory to manage this mutual relationship, and the program must behave soundly even if some instructions are executed under the native environment. We argue that this is a non-trivial and error-prone task, as no automatic tool currently exists to translate Java bytecode to native on Android. %\alessio{sentence rewritten. Please check.} 
Furthermore, NRP suffers from the same limitations of BombDroid, related to the use of hash functions to hide the decryption key. If a logic bomb is inserted in an  \texttt{if} statement with a small hash space, it could be rather quick to recover the decryption key by brute force. As the authors discuss, NRP suffers from this limitation, as most of the constant values in an $apk$ are in the interval [-1024, 1024]. Finally, and differently from BombDroid, the hash function in NRP is not salted. As a consequence, whenever a decryption key is recovered, it is possible to statically detect all logic bombs that have the same key by only comparing the hash values. In fact, if two candidate conditions have the same constant value (e.g., \texttt{if(a == 1) {...}} and \texttt{if (b == 1){...}}, the hardcoded values in the trigger condition are likewise the same (i.e., \texttt{if(hash(a) == 'xyz')} and \texttt{if(hash(b) == 'xyz')},  since no salt is used. 
%\alessio{I will explain it better. Why is this possible statically?} \antonio{if there is two candidate condition if(a == 1)\{...\} and if(b == 1)\{...\}, the hard-coded values are equals in both trigger condition (i.e. if(hash(a) == hash(1)) and if(hash(b) == 'hash(b)) ) because no salt is used.} % Therefore, if an attacker recovers the key of a candidate condition, she is able to find all logic bombs whose triggering condition has the same key = 1, by looking for the value \texttt{hash(1)} in the code.

\subsubsection{Protecting Antimine with NRP}

We applied NRP to Antimine: the process lead to the insertion of $315$ logic bombs. For the sake of explanation, we focus on a single protected candidate method, namely the \texttt{setButton()} one. This method is invoked each time the user clicks on a blind button in the minesweeper game, and changes the look and feel of the button and its neighbors, as well as the message to prompt to the user, according to the rule of the game (see Figure \ref{fig:antimine-fig}). As this method makes decisions, it contains several qualified conditions (e.g., \texttt{var == -1}). 


% shows the result of NRP applied to a candidate condition found in $setButton$ method of $androidx.appcompat.app.AlertController$ class. \alessio{I assume that the set button is the code responsible for the look and feel of the button representing a cell in the minesweeper game. Am I right?} \antonio{yes. Precisely this function is part of the androidx library (see https://developer.android.com/reference/androidx/appcompat/app/AlertDialog\#setButton(int,\%20java.lang.CharSequence,\%20android.graphics.drawable.Drawable,\%20android.content.DialogInterface.OnClickListener)).} 

\begin{figure}
  \includegraphics[width=1.1\textwidth]{figs/native-bombdroid-evolution-example.pdf}
  \caption{NRP applied to the \texttt{setButton()} method of Antimine.}
  \label{fig:native-bombdroid-evolution-example}
\end{figure}

Figure \ref{fig:native-bombdroid-evolution-example} describes the actual protection workflow, step-by-step. First, NRP parses the \texttt{classes.dex} file (Step 2.2) and selects all methods with at least a qualified condition as candidate methods (Step 2.3). NRP adds a logic bomb in any candidate methods and for each qualified condition. Concerning the \texttt{setButton()} method, it selects the condition \texttt{var == -1} and splits the original code of the corresponding block into two parts, namely \texttt{or\_code1} and \texttt{or\_code2}. 
In Step 2.4, NRP builds up the logic bomb by i) rewriting the if block in the candidate method, and ii) distributing the logic of the bomb among two encrypted files, namely a Java class (i.e., \texttt{encr\_cl.dex}) and a native C/C++ library (i.e., \texttt{nat\_encr.so}). Concerning the first point, the qualified condition is translated into a Boolean variable (i.e., \texttt{resultMatch}), whose value is calculated by comparing the \texttt{var} value with the hash of \texttt{-1} encoded as a byte array. In case the value of \texttt{resultMatch} is true, the block executes a \texttt{decryptAndInvokeMain(\ldots)} method. Such method takes as input the actual name of the encrypted Java class (i.e., \texttt{className = AlertController\_setButton...}), its binary representation (i.e., \texttt{cipherCode}, which is contained in the block), as well as the value of \texttt{var} and and the array of arguments (i.e., \texttt{args}) required by the main method of the encrypted Java class to execute properly. 
The invocation of such method leads to the decryption of \texttt{cipherCode}, using the value of \texttt{var} as decryption key, and to the execution of the main method of the class \texttt{AlertController...}. The main method contains the \texttt{native\_key} to decipher the native library (i.e., \texttt{nat\_encr.so}), a JNI call and the second part of the original block code (i.e., \texttt{or\_code2}). The JNI call triggers the execution of a deciphering function in the native library (i.e., \longstring{Java\_embedded\_native\_androidxappcompat(\ldots)}, which i) retrieves the encrypted native code from a memory location, ii) decrypts it using the \texttt{native\_key}, and iii) launches the execution of the decrypted function. This latter function (i.e., \longstring{Java\_embedded\_native\_androidxappcompat[\ldots]\_KEY(\ldots)}) contains the anti-tampering check (i.e., \texttt{hash\_file\_in\_apk(\ldots)}) that verifies the integrity of the first 100 bytes of the \texttt{classes.dex} file. If the integrity is verified, the function executes the first part of the original block code (i.e., \texttt{or\_code1}). Finally, the JNI call terminates and the main method in the Java class executes the last part of the original block (i.e., \texttt{or\_code2}).   

\subsubsection{Dismantling NRP bombs}
The attacker has to bypass the integrity checks performed by the protected app in the \longstring{Java\_embedded\_native\_androidxappcompat[\ldots]\_KEY(\ldots)} function to dismantle the NRP logic bombs.
To achieve such result, the attacker can either i) override \texttt{encr\_cl.dex} or \texttt{nat\_encr.so} for all the triggered logic bombs, by leveraging code deletion and binary patching, or ii) bypass the integrity check performed by the native code, by relying on a replay attack.

\paragraph{Bytecode and Native Code Overriding:}
The attacker can instrument the code to intercept the invocations to the \textsl{decryption functions} both in the Java and the native code, in order to retrieve i) the encrypted code and the decryption key passed as argument to the function, and ii) the decrypted code at the end of that function. Code instrumentation can also be used to change the implementation (or just the return value) of the tamper check function in the native code.

The Java decryption method requires two input values, namely the encrypted code (\texttt{param2}) and the decryption key (\texttt{param1}), and returns the decrypted code. % \alessio{not sure to leave or embed this sentence in other sentences.}
Figure \ref{fig:linear-dump-frida} shows the Frida script that instruments the Java decryption method (i.e., \texttt{SDCloaderr.decryptAndInvoke(\ldots))}
%\alessio{There is a lack of precision here. Till now, we threated this method as double, where both decryption and invocation are executed. Nonetheless, it seems here that the Frida script only focuses on decryption. Do you mean that you instrumented just a - the decryption - part of such method? We must clarify.} \antonio{Frida can be use in both scenarios. For example, if we intercept the invokation of the InMeryDexClassLoader we can retrive the bytes of the decrypted dex that we are going to load into memory. Alternatively, we can hook/intercept directly the invocation of the integrity check function in order to change the returned value and pass the check. In this case (bytecode overriding), we are interested to retrieve both the encryption/decryption key and the decrypted bytes of the dex (or native code) that we are going to call. For this purpose, we identified the hook of the decryption function (both in Java and C code) as the most useful technique. Moreover, we can intercept the invokation of the decrypted function for other purposes, such as change input parameter or return value}
for a given encrypted code \texttt{encr\_cl}, represented by \texttt{ciphered\_byte} (i.e., the \texttt{cipherCode} byte array in the \texttt{setButton} method), that we will analyze using Jadx \cite{Jadx}). 
The script begins by selecting (lines 1 and 2) the class (i.e.,  \longstring{embedded.SDCLoader}) and the decryption method (i.e., \texttt{decrypt}) to overload. Frida hooks at the start of the overloaded function and executes the customized code (lines 3 to 19) instead of the original code.
The customized code calls the original Java \texttt{decrypt} method (line 6) and stores the returned value in a variable. Since the attacker's aim is to get access to a specific decrypted function, the script (lines 7-13) compares the encrypted method passed as the input parameter \texttt{param2} with \texttt{ciphered\_bytes}. If the decryption function is correct, the script writes down the decrypted bytecode (line 16). It is worth noticing that the script also dumps the key inside the \texttt{param1} variable. The return value of the overloaded function is the return value of the original decryption function (line 19).


\begin{figure}[!htbp]
\begin{lstlisting}[language=Java,
    basicstyle=\scriptsize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
var SDCLoader = Java.use("embedded.SDCLoader");
SDCLoader.decrypt.overload("[B", "[B").implementation = function(param1, param2) {
  var arr_bytes = Java.array('byte', param2);
  var ciphered_bytes = [107, 30, -22 [..] 18];
  var found = true;
  var dexBytesDecrypted = this.decrypt(param1, param2);
  if(arr_bytes.length == ciphered_bytes.length) {
  	for(var i = 0; i < ciphered_bytes.length; i++) {
  	  if(ciphered_bytes[i] != arr_bytes[i]){
  	    found = false;
  		break;
  	  }
  	}
    if (found) {
  	  console.log("### FOUND");
  	  // Write to file dexBytesDecrypted
    }
  }
  return dexBytesDecrypted;
}
\end{lstlisting}
\caption{Frida script to dump the result of decrypted function.}
\label{fig:linear-dump-frida}
\end{figure}

Concerning the native decryption function, it can be reversed using a decompiler (i.e., Ghidra \cite{ghidra}), and analyzed to detect the decryption function, and to infer the decryption logic (e.g., it is possible to analyze the body of the \texttt{Java\_embedded\_native\_androidxappcompat[...]} function). 
Here, the \texttt{decrypt\_code} function is responsible for decrypting $n$ bytes of machine code starting from a pointer to the memory. Such function can be overloaded and dumped through the scripts described in Figure \ref{fig:native-dump-frida} and Figure \ref{fig:native-dump-frida2}, which allow retrieving both the plain code and the key, as in the case of the Java decryption function. 
%\autoref{fig:native-dump-frida} shows the Frida script that we used to intercept the call to $decrypt\_code$ function and dump the bytes decrypted from memory.
%In this case we want to overload a native function instead of a Java function. 
In detail, the script in Figure \ref{fig:native-dump-frida} aims to detect the location in which the target function to dump will be decrypted and executed. It starts by retrieving the \texttt{libnative-lib.so} (line 2) - which is the shared object containing all native functions implemented by NRP and then it enumerates each function therein (lines 6-10) to detect the \texttt{decrypt\_code} functions. Then, the script sets up an interceptor for the function (line 13). Whenever a \texttt{decrypt\_code} function executes, the script verifies whether the decryption function is the expected one (lines 14-30), by comparing the key passed as a parameter to the \texttt{native\_key} hardcoded in the \texttt{encr\_cl.dex} file. 
If this is the case, the script invokes the \texttt{AES\_CTR\_xcrypt\_buffer} function that decrypts the code, write the plain machine code in a writable page, and makes it executable. More specifically, the script in Figure \ref{fig:native-dump-frida2} attaches Frida to the \texttt{AES\_CTR\_xcrypt\_buffer} function (lines 5-14). Then, when the function starts (i.e., OnEnter, lines 15-18), the script retrieves the memory address (i.e., \texttt{args[1]}) and the size (i.e., \texttt{args[2]}) of the write buffer for the code. After the decryption phase terminates (i.e., OnLeave (from line 19 to line 24), the script checks whether the decrypted code is correct (line 20): in case, the script retrieves the pointer to the starting address (line 21) and dumps \texttt{len} bytes (lines 22-24).

\begin{figure}[!htbp]
\begin{lstlisting}[language=Java,
    basicstyle=\scriptsize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
function inspectModule(module) {
  var m = Process.getModuleByName(module);
  var targetFunction = true;
  var functionToBeIntercepted = "";
  var exports = m.enumerateExports();
  exports.forEach(function(exp){
    if (exp.name.indexOf("decrypt_code")>=0){
      functionToBeIntercepted = exp.name; 
    }
  });

  // Intercept decrypt_code function
  Interceptor.attach(m.getExportByName(functionToBeIntercepted), {
    onEnter: function(args) {
      var pointer = new NativePointer(args[2]);
      var buff = pointer.readByteArray(16);
      buff = new Int8Array(buff);
      var key = [-63, [...], -9]; // native_key hardcoded in encr_cl.dex
      targetFunction = true;
      for(var i = 0; i < buff.length; ++i){
        if(buff[i] != key[i]){
          targetFunction = false;
          break;
        } 
      }
      if(targetFunction) {
	    console.log("##### FOUND");
      } 
    }
  });

  // Intercept AES_CTR_xcrypt_buffer function
  [...]
}
\end{lstlisting}
\caption{Frida script that searches for the target \texttt{decrypt\_code} function.}
\label{fig:native-dump-frida}
\end{figure}

\begin{figure}[!htbp]
\begin{lstlisting}[language=Java,
    basicstyle=\scriptsize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
function inspectModule(module) {
  [...]
  // Intercept AES_CTR_xcrypt_buffer function
  // Dump the return bytes
  functionToBeIntercepted = "";
  exports = m.enumerateExports();
  exports.forEach(function(exp){
    if (exp.name.indexOf("AES_CTR_xcrypt_buffer")>=0){
      functionToBeIntercepted = exp.name; 
    }
  });
  var outAddr = "";
  var len = 0;
  Interceptor.attach(m.getExportByName(functionToBeIntercepted), {}
    onEnter: function(args) {
      outAddr= args[1];
      len = parseInt(args[2]);
    },
    onLeave: function(retval) {
      if(targetFunction) {
        var pointer = new NativePointer(outAddr);
        var buff = pointer.readByteArray(len);
        // DUMP buff
        send("Readed byte", buff);
      }
    }
  });
}
\end{lstlisting}
\caption{Frida script that dumps the assembly code decrypted by the native function.}
\label{fig:native-dump-frida2}
\end{figure}

\newpage

The decrypted code is a hex string that encodes the x86 assembly instructions. Such instructions can be extracted using a disassembler. 
The analysis of the disassembled instructions allows detecting a hardcoded tamper check on the \texttt{classes.dex} file 
%\begin{lstlisting}[language=c]
\begin{center}
    \texttt{cmp eax, 0xb543c475}
\end{center}
%\end{lstlisting}
where \texttt{$0xb543c475$} is the checksum of the original \texttt{classes.dex} file of Antimine.

Once the original codes and the decryption keys are recovered, an attacker can easily bypass the tamper check by overriding the hardcoded value with the one of the repackaged app, and then re-encrypting the assembly code and substituting the original code in the $.so$ file. As an alternative, the attacker can modify the decrypted \texttt{nat\_enc.so} and the \texttt{encr\_cl.dex} to execute \texttt{op\_code1} in Java rather than in the native code, and remove the JNI call that would trigger the tamper check.  

\begin{figure}[!htbp]
  \includegraphics[width=\textwidth]{figs/sochanged.jpg}
  \caption{The original (top side) and the tampered (bottom side) library file.}
  \label{fig:sochanged}
\end{figure}

\paragraph{Bypass the integrity check:}
An alternative attack to bypass the tamper check is to leverage a reply attack by modifying the file on which the tamper check is executed. This attack can be carried out since the path of the checked file is hardcoded in the native library in clear text. 

We carried out this attack as follows: we added a new file (i.e., \texttt{cla.dex}) to the $apk$, that has the same content of the original \texttt{classes.dex} of Antimine. Then, we manually patched the hardcoded path in the \texttt{elf} file to point to \texttt{cla.dex} instead of the \texttt{classes.dex} which is modified by the attacker before repackaging. In this way, the tamper check passes as it calculates the expected value, despite the app content has been modified. Figure \ref{fig:sochanged} shows the original library (top side), and the tampered one (bottom side) in which the hardcoded path is modified to point to $cla.dex$.

Previous attacks allowed to successfully bypass the NRP protection on Antimine. The repackaged version of Antimine, with all the 315 bombs de-activated, is available at:
\begin{center}
\url{https://www.csec.it/projects/antimine-800011-protected-and-repacked.apk} \\
\end{center}
for further studies, analysis and testing activities. 

%\paragraph{Conclusion}
%This attacks are based on the fact that code instrumentation have no effect on the $classes.dex$ file and the anti\-tampering controls are not influenced by this attack.

%Contrary to Bombdroid, once the machine code is retrieved, it is harder to completely remove the logic bomb due to it is implemented in native code. This was not a problem because we could still bypass the AT checks (as we see above) and add anyway the malicious code.

\begin{comment}
Some useful code
\begin{figure}[!htbp]
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
public void setButton(int i, CharSequence charSequence,
DialogInterface.OnClickListener onClickListener,
Message message, Drawable drawable) {
  if (message == null && onClickListener != null) {
    message = this.mHandler.obtainMessage(i, onClickListener);
  }
  if (i == -3) {
    this.mButtonNeutralText = charSequence;
    this.mButtonNeutralMessage = message;
    this.mButtonNeutralIcon = drawable;
  } else if (i == -2) {
    this.mButtonNegativeText = charSequence;
    this.mButtonNegativeMessage = message;
    this.mButtonNegativeIcon = drawable;
  } else if (i == -1) {
    this.mButtonPositiveText = charSequence;
    this.mButtonPositiveMessage = message;
    this.mButtonPositiveIcon = drawable;
  } else {
    throw new IllegalArgumentException("Button does not exist");
  }
}
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{.45\textwidth}
\begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
public void setButton(int i, CharSequence $r3,
DialogInterface.OnClickListener onClickListener,
Message $r2, Drawable $r1) {
  if ($r2 == null && onClickListener != null) {
    $r2 = this.mHandler.obtainMessage(i, onClickListener);
  }
  if (i == -3) {
    this.mButtonNeutralText = $r3;
    this.mButtonNeutralMessage = $r2;
    this.mButtonNeutralIcon = $r1;
  } else if (i != -2) {
    Integer $r7 = Integer.valueOf(i);
    boolean $z0 = SDCLoader.match($r7, new byte[]{-39, -66, 101, 36, -91, -11, 4, 125, -75, -122, 104, 19, -84, -13, 39, 120, -110, -89, -93,10});
    byte[] $r10 = {107, 30, -22 [...] 18};
    Object[] $r12 = {this, $r2, $r1, $r3};
    if ($z0) {
      ResultWrapper $r9 = SDCLoader.decryptAndInvokeMain("androidx.appcompat.app.AlertController_setButton_1fa3710f-3cce-4365-8c84-811bf490e68d", $r10, $r7, $r12);
      int $i1 = $r9.jumpTarget;
      if ($i1 != -1) {
        Object[] $r13 = $r9.savedPrimitivesAndReferences;
        AlertController alertController = (AlertController) $r13[0];
        Message $r22 = (Message) $r13[1];
        Drawable drawable = (Drawable) $r13[2];
        CharSequence charSequence = (CharSequence) $r13[3];
        if ($i1 != -2) {}
      } else {
        return;
      }
    }
    throw new IllegalArgumentException("Button does not exist");
  } else {
    this.mButtonNegativeText = $r3;
    this.mButtonNegativeMessage = $r2;
    this.mButtonNegativeIcon = $r1;
  }
}
\end{lstlisting}
\end{minipage}
\caption{On the left side the original code. On the right side the protected method.}
\label{fig:if-protected}
\end{figure}
\clearpage

\begin{figure}[!htbp]
\begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
var SDCLoader = Java.use("embedded.SDCLoader");
SDCLoader.decrypt.overload("[B", "[B").implementation = function(param1, param2) {
  var arr_bytes = Java.array('byte', arr2);
  // Ciphered "androidx.appcompat.widget.LinearLayoutCompat_" 
  // "measureHorizontal_1a173610-a602-41f6-a1e5-6133fbbd9903" method
  var ciphered_bytes = [88, 23, -64, 30, 122, 57,[..], -114];
  var found = true;
  var dexBytesDecrypted = this.decrypt(param1, param2);
  if(arr_bytes.length == ciphered_bytes.length) {
  	for(var i = 0; i < ciphered_bytes.length; i++) {
  	  if(ciphered_bytes[i] != arr_bytes[i]){
  	    found = false;
  		break;
  	  }
  	}
    if (found) {
  	  console.log("### FOUND");
  	  // Write to file
    }
  }
  return dexBytesDecrypted;
}
\end{lstlisting}
\caption{Frida script to dump  $androidx.appcompat.widget.LinearLayoutCompat_measureHorizontal_1a173610-a602-41f6-a1e5-6133fbbd9903$ decrypted function.}
\label{fig:linear-dump-frida}
\end{figure}

\begin{figure}[!htbp]
\begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
public class LinearLayoutCompat_measureHorizontal_1a173610a60241f6a1e56133fbbd9903 {
  public static ResultWrapper main(boolean z, boolean z2) {
    native.androidxappcompatwidgetLinearLayoutCompatmeasureHorizontal1a[...](
    new byte[]{-63, [...], -9});
    Object[] objArr = new Object[2];
    return new ResultWrapper(0, restoreLocals(true, true));
  }

  public static Object[] restoreLocals(boolean z, boolean z2) {
    return new Object[]{Boolean.valueOf(z), Boolean.valueOf(z2)};
  }
}
\end{lstlisting}
\caption{The decrypted  $androidx.appcompat.widget.LinearLayoutCompat_measureHorizontal_1a173610-a602-41f6-a1e5-6133fbbd9903$ method.}
\label{fig:linear-dumped}
\end{figure}

\begin{figure}[!htbp]
\begin{lstlisting}[language=C,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
void Java_embedded_native_androidxappcompatwidgetLinearLayoutCompatmeasureHorizontal1a173610a60241f6a1e56133fbbd9903 (JNIEnv *env,jbyteArray jni_decryption_key)
{
  char decrypted;
  int iVar1;
  uchar *key;
  jbyteArray in_RDX;
  char *pcVar2;
  if (decrypted == '\0') {
    key = (uchar *)(*env->functions->GetByteArrayElements)((JNIEnv*)env,in_RDX,(jboolean *)0x0);
    iVar1 = decrypt_code(Java_embedded_native_android[...],0xa0,key);
    pcVar2 = "DECRYPT: FAIL";
    if (iVar1 == 0) {
      pcVar2 = "DECRYPT: Success";
    }
    (*env->functions->ReleaseByteArrayElements)((JNIEnv *)env, in_RDX,(jbyte *)key,2);
    decrypted = '\x01';
    pcVar2 = "Entering decrypted segment...";
  }
  else {
    pcVar2 = "Code already decrypted. Jumping to decrypted code!\n";
  }
  _DAT_ef2f54c83f3bec25 = (int)register0x00000020 + -4;
  return;
}
\end{lstlisting}
\caption{Native function inside the .so library.}
\label{fig:linear-native}
\end{figure}

\begin{figure}[!htbp]
\begin{lstlisting}[language=Java,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
function inspectModule(module) {
  var m = Process.getModuleByName(module);
  var targetFunction = true;
  var functionToBeIntercepted = "";
  var exports = m.enumerateExports();
  exports.forEach(function(exp){
    if (exp.name.indexOf("decrypt_code")>=0){
      functionToBeIntercepted = exp.name; 
    }
  });

  // Intercept decrypt_code function
  Interceptor.attach(m.getExportByName(functionToBeIntercepted), {
    onEnter: function(args) {
      var pointer = new NativePointer(args[2]);
      var buff = pointer.readByteArray(16);
      buff = new Int8Array(buff);
      // our method key
      var key = [-63, [...], -9];
      targetFunction = true;
      for(var i = 0; i < buff.length; ++i){
	    if(buff[i] != key[i]){
	      targetFunction = false;
	      break;
	    } 
	  }
	  if(targetFunction) {
	    console.log("##### FOUND");
	  } 
    }
  });

  // Intercept AES_CTR_xcrypt_buffer function
  // Dump the return bytes
  functionToBeIntercepted = "";
  exports = m.enumerateExports();
  exports.forEach(function(exp){
    if (exp.name.indexOf("AES_CTR_xcrypt_buffer")>=0){
      functionToBeIntercepted = exp.name; 
    }
  });
  var outAddr = "";
  var len = 0;
  Interceptor.attach(m.getExportByName(functionToBeIntercepted), {}
    onEnter: function(args) {
      outAddr= args[1];
      len = parseInt(args[2]);
    },
    onLeave: function(retval) {
      if(targetFunction) {
        var pointer = new NativePointer(outAddr);
        var buff = pointer.readByteArray(len);
        // DUMP buff
        send("Readed byte", buff);
      }
    }
  });
}
\end{lstlisting}
\caption{Frida script to dump native function decrypted bytecode.}
\label{fig:native-dump-frida}
\end{figure}

\begin{figure}[!ht]
\begin{lstlisting}[language=C,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
]
static bool alreadyChecked;
static bool passed;
if(!didCheck){
  if(0x5d434c4a == hash_file_in_apk("classes.dex", 100)){
	passed = true;
  } else {
	passed = false;
  }
  alreadyChecked = true;
}
if(passed) {
  // exec code
} 
\end{lstlisting}
\caption{Native function decrypted and decompiled from bytecode.}
\label{fig:native-flow}
\end{figure}

We are going to propose two different approaches to bypass the AT controls based on changing the hard-coded values in the so file.
In the first one, we inserted inside the apk a new file that has the same content of the \emph{classes.dex} and manually patched the hard-coded path in the elf file. In this way, the AT control computes the right value despite the app content has been modified. In fig \ref{fig:sochanged} we show the original library (top side), and the tampered one (bottom side). Inside the tamepred apk we inserted the $cla.dex$ file, that is the $classes.dex$ file taken from the protected app.
Beside this value, the expected hash value is hard-code inside the so file. Modify this value is more difficult because the code is ciphered. We intercepted the decrypted machine code we disassembled it to analyze its content. This snippet contains the expected value of the integrity check in an hard-coded way and an we were able to change this value with his desired one. 
Once the expected value is replaced, we re-encrypted the function and substitute it in the so file.

Contrary to Bombdroid, once the machine code is retrieved, it is harder to completely remove the logic bomb due to it is implemented in native code. This was not a problem because we could still bypass the AT checks (as we see above) and add anyway the malicious code.

\end{comment}

%\clearpage


%\paragraph{Example}
%\todo{metto qua gli esempi (in un paragrafo diverso) o li metto inline nel paragrafo security issues ?!}

==> sections/old paper files/attackingmodels.tex <==
\section{Attacking Anti-Repackaging} \label{sec:attacking_model}
In this section, we discuss the \textsl{weapon rack} of repackaging, i.e., the main set of techniques that an attacker can leverage to analyze a protected $apk$ in order to detect and dismantle anti-repackaging protections (Steps 8 and 9 in Figure \ref{fig:threat-model-design}). They can be divided in two main categories, namely \textsl{static} and \textsl{dynamic}. The first category refers to the set of techniques that analyze the $apk$ without executing it (static analysis), while the latter category is composed by techniques that apply to an $apk$ while executing on an actual or emulated Android device (dynamic analysis). 

On one hand, static analysis aims at systematically reverse engineering the $apk$ (e.g., White Box Reverse Engineering  ~\cite{mitre_white_box_reverse_engineering}) in order to reconstruct and analyze the original source code. There exist a lot of tools that support this type of analysis and help an attacker to decode, rebuild and inspect both the app code and the resources, such as apktool~\cite{apktool} and dex2jar~\cite{dex2jar}.
On the other hand, dynamic analysis aims at inferring the app behavior during execution, to retrieve, e.g., actual values of variables, and monitor the execution of the code. 

Static and dynamic analysis are complementary: the first aims at building a comprehensive model of the app behavior by systematically exploring all the code and the resources of the app; the latter focuses on inferring a model of the app behavior by repeatedly executing the app. In principle, the static model is a superset of all possible behaviors of the app, meaning that at runtime the app will exhibit only a subset of the behavior of the static model. The dynamic model is partial by definition (as it is impossible to stimulate all possible executions of the app at runtime) but contains only behaviors that the app actually exhibits. As a consequence, static analysis suffers from \textsl{false positives} (e.g., a statically detected behavior could not be executed at runtime), while dynamic analysis suffers from \textsl{false negatives} (a behavior which has not been recognized during the dynamic analysis phase could be assumed as non-existent). %\luigi{Anziché "is assumed", preferirei "could be assumed"}. 

Concerning anti-repackaging, static analysis aims to detect the pieces of code where logic bombs could potentially hide (e.g., blocks with hash values in the qualified condition), while dynamic analysis allows to check the actual triggering and execution of the bombs at runtime. Furthermore, the repeated execution of the app on several setups allows the attacker to carry out \textsl{cumulative attacks}~\cite{8368344}\footnote{See the AppIS approach in Section \ref{subsec:appis-2017}}.  
%Finally, static and dynamic analysis suffer from opposite features and weaknesses. Concerning features, static analysis is exhaustive, i.e., it allows to explore all code branches  and resources at once, and detect all potential bombs, while dynamic analysis allows to repeatedly execute the app many times to detect differences among execution (and carry out ). Weaknesses are directly related to the previous features: static analysis suffers from false positives,  (i.e., pieces of original code with a qualified condition with hash values can be wrongly recognized as potential bombs) while dynamic analysis is subject to false negatives (it detects bombs only when they are triggered; therefore, untriggered bombs are not recognized).
Within the ``try and error'' cycle, the attacker builds up an analysis workflow of the $apk$ which fruitfully combines static and dynamic analysis techniques.

Hereafter, we briefly introduce the main static and dynamic analysis techniques to detect anti-repackaging. %Table \alessio{Add table and reference.} summarizes...




%\begin{itemize}
 %   \item \textbf{Static analysis} i analysis of software that is performed without executing programs.
  %  This approach is possible because the current structure of an apk file could allow . In other words, an attacker could retrieve useful information and sensitive data inspecting files inside the apk.
        
   % \item \textbf{Dynamic analysis} is the investigation of software (in our case Android application) that is performed by executing programs on real or virtual devices. 
%    In particular, the main issue to mitigate is what is called : an attacker could, with enough time and resources, run n-times the same app to retrieve many information such as which calls are performed, where an app crashes, etc.
    
%\end{itemize}

\subsection{Text Search and Pattern Matching} \label{sec:text_search_and_pattern_matching}
This technique statically analyzes the decompiled $apk$ to detect keywords or expressions that may hide logic bombs. The search and detect phase relies on heuristics and regular expressions defined by the attacker herself, or on pre-defined patterns defined in static analysis tools that support this technique. For instance, this technique may allow recognizing explicit anti-tampering function calls, as well as qualified conditions containing hash values. As any other static analysis approach, all detected anti-tampering checks must be evaluated at runtime to filter true positives (i.e., the checks which actually hide some logic bombs). 

The efficacy of this technique is rather limited, as it can be easily circumvented by anti-repackaging techniques. For example, SSN and BombDroid~\cite{7579771, 10.1145/3168820} are resilient to this threat as they rely on Java reflection or obfuscation~\cite{Norboev2018OnTR}; the first allows hiding function calls inside the code, while the latter avoids text search as obfuscation modifies the syntax of the code (e.g., method renaming).

\subsection{Fuzzing}\label{sec:fuzzing}
Fuzzing is an automated testing technique that provides pseudo-random input to a running program. There exist three different types of approaches, namely:
\begin{itemize}
    \item \textbf{Blackbox fuzzing}: it generates input data without having any knowledge of the app code and structure \cite{10.1145/2491411.2491450};
    \item \textbf{Whitebox fuzzing}: it  is also known as \textsl{symbolic execution} \cite{10.1145/2382756.2382798, 4223228}
    and it applies to the app code, which is supposed to be accessible by the attacker. 
    The main goal of whitebox fuzzing is to provide input data which allows exploring as many execution paths as possible, in order to detect which data could match specific condition (e.g., the trigger of a logic bomb). Moreover, whitebox fuzzing could allow revealing the destination of a suspicious call executed through Java reflection. 
    From a technical standpoint, the main difference between blackbox and whitebox fuzzing is that the latter adopts a (symbolic) input which evolves according to the program analysis and to reach certain critical program location; the first one, instead, does not rely on the program structure. 
    \item \textbf{Graybox fuzzing}: this approach mixes blackbox and whitebox fuzzing, i.e., it generates symbolic input for the sole subpart of the program which is known to the attacker, while the unknown part of the app is stimulated according to blackbox fuzzing data generation.
\end{itemize}
Fuzzing is suitable for assessing an $apk$ protected with SSN or Bombdroid, as it allows to trigger (and detect) the bombs (repackaging detection nodes) or to perform analysis of hash values. However, these techniques do not grant a complete path exploration and a full input data coverage. Therefore, they cannot find and trigger all bombs~\cite{Norboev2018OnTR}. 

\subsection{Debugging and Code Emulation}\label{sec:debugging_and_code_emulation}
The most common way to deeply analyze the behavior of an app is to use a debugger. In the general case, a debugger allows a developer to dynamically test a software in order to find and resolve bugs. Concerning the attack to anti-repackaging, a debugger allows bypassing all static countermeasures like obfuscation, and understand how the app behaves at runtime.
More in detail, an attacker can intercept critical calls, find out repackaging detection and understand the type of anti-tampering checks.
However, debugging strongly relies on manual intervention, which has the drawback to scale badly, i.e., debugging an app to try tracing back all bombs has been proven to be unfeasbile~\cite{Norboev2018OnTR, 10.1145/3168820}.

In addition, the debuggable flag inside the app manifest file has to be set to true, in order to attach a debugger to an Android app. Developers that apply anti-repackaging techniques trivially set this flag to false. Therefore, an attacker should first modify the app manifest~\cite{owasp_mobile_security_testing_guide} and repackage it before debugging. This first repackaging step can itself trigger proper logic bombs in the app and make the execution of the app fail. 

An alternative to debugging is \textsl{code emulation} in \cite{180237, BHANDARI2017392}: %\alessio{Do we really need both references? why?}\luigi {Yes, because unlike debugging with code emulation the attacker can modify device behavior ie modify return values of system calls. In this way it is possible to explore more paths}
 the idea is that the target app is executed on some virtual machine, where the hardware, the Android OS and the Dalvik VM layers are replicated. During app execution, the virtual machine performs call tracing \cite{10.1145/1966445.1966460}. 
However, both approaches follow specific execution paths that depends on input data and could not reach the candidate methods in which logic bombs are hidden.

\subsection{Process Exploration}\label{sec:process_exploration}
\textsl{Process Exploration} refers to a set of techniques allowing the attacker to deeply inspect the app process memory at runtime~\cite{owasp_mobile_security_testing_guide}. There exists several tool to support memory exploration, most of which are Frida-based\footnote{We will discuss Frida in Section  \ref{subsec:code_instrumentation_and_code_injection}}, and rely on \textsl{dynamic code instrumentation}.
Currently, the most widespread tools are:
\begin{itemize}
    \item \textbf{Fridump}: an open source memory dumping tool for both Android and iOS ~\cite{fridump}. From a memory dump, it is possible to access to memory addresses where, for example, decryption key of anti-repackaging tools are stored at runtime;
    \item \textbf{Objection}: a runtime mobile exploration toolkit for both Android and iOS, that does not require a rooted device. Two interesting features of Objection are the ability to i) circumvent SSL pinning, i.e., a technique allowing apps to authenticate the server and avoid man-in-the-middle-attacks), and ii) dump and patch  memory locations~\cite{objection};
    \item \textbf{R2frida}: a tool that merges the reverse engineering capabilities of \textsl{radare2}~\cite{Radare} (a reverse engineering framework) with Frida (a dynamic instrumentation toolkit). In this way, an attacker can carry out runtime reverse engineering and memory related tasks, such as memory inspection~\cite{r2frida}.
\end{itemize}
The adoption of  such tools allows an attacker to analyze the runtime behavior of an app without debugging it (i.e., without the need to force the set of the debuggable flag to true and repackage.).

%Process exploration suffers from the lack of exhaustiveness of other dynamic tool. \alessio{maybe add a final sentence, but we see in the final version} \luigi{Maybe remove this last sentence}

\subsection{vtable Hijacking}\label{sec:vtable_hijacking}
In Java, a virtual table (vtable) dynamically maps function calls, i.e., a Java object points to some records of the vtable which contains the link to the actual method implementation. In Java, all methods are virtual by default, unless they are declared as \textsl{final} or \textsl{static}.
An attacker can modify the values in the vtable in order to invoke an arbitrary method and change the behavior of the original method. 
The limitation of this approach is that it works properly only on rooted devices, as the attacker needs root privileges to change the entries of the vtable~\cite{artdroid}.

An example of vtable hijacking is proposed in~\cite{7579771}: here, the vtable mapping is modified to redirect all invocation to the \emph{getPublicKey} method to a spoofed function which returns the public key of the original developer, instead of the public key of the attacker that repackaged the app. %\alessio{The sentence was unclear. I did my interpretation but it is pssibily wrong. Please explain here in detail how this work. }\luigi{The attacker repack the original app, and the public key obviously changes; the anti tampering control calls a getPublicKey method, the attacker modify the vTable in order that getPublicKey method points to a attacker-controlled method that return the original publicKey}

%, thereby bypassing the standard anti-repackaging check based on the user. As a consequence, any invocation of the  If an attacker has root privilege and changes the vtable’s entry related to \emph{getPublicKey}, he could bypass the anti repackaging controls (the app believes to call the right function, but calls the attackers one). 

%We assume the attacker has no access to users vtable ~\cite{Norboev2018OnTR, 10.1145/3168820}.\alessio{I do not understand which is the meaning of this assumption. Please explain.} \luigi{to modify the vTable the attacker should have root access in the user device, in this case the repackaging problem is meaningless for the user}
%However, this technique could be used by an attacker to bypass some checks in order to retrieve more information about the application.

\subsection{Code Manipulation}\label{subsec:code_manipulation}
There exist three main techniques to affect the app code in order to remove  anti-repackaging checks or to add malicious code, namely \textsl{code deletion}, \textsl{binary patching} and \textsl{code instrumentation and injection}. The first two techniques are static, while the latter is dynamic.

\paragraph{Code deletion:}\label{subsec:code_delection}
This technique aims at removing proper part of the app source code (if available), or smali code in order to deactivate specific controls. It can be partially circumvented: for instance, the anti-repackaging checks may be hosted in methods that cannot be straightforwardly removed, i.e., many other parts of the app depend on them. Alternatively, fake controls resembling logic bombs can be added in the code to fool the attacker which exploits code deletion \cite{10.1145/3168820}. In case the attacker remove them from the code, the app will not work properly.

\paragraph{Binary patching:}\label{paragraph:binary_patching}
It refers to the process of modifying a compiled executable to change its behavior. Differently from code deletion, binary patching does not need to retrieve or reconstruct the app source code, and it is, for instance, independent from code obfuscation.
It is worth pointing out that it is far easier and more reliable to apply binary patching  to Java than native code (e.g., C, C++, \ldots). Therefore, this technique is promising for an attacker, as current apps still contain most of the business logic in the Java/Kotlin part of the app (see Section \ref{sec:background}) rather than in the native part.

To counteract binary patching, the anti-repackaging checks need to be protected, i.e., through encryption applied at Java (see Sections \ref{subsec:dyn-self-prot-encrypt-2015}, \ref{subsec:sdc-2018},  \ref{subsec:bombdroid-2018}) or native level (Section \ref{subsec:bombdroid-native-2019}).
As an alternative, checks can be hidden by exploiting Java reflection~\cite{7579771}, however, once the attacker understands the protection pattern, he could patch the executable and remove checks with minimum effort, as discussed in~\cite{Norboev2018OnTR, 10.1145/3168820}.

\paragraph{Code Instrumentation and Injection:} \label{subsec:code_instrumentation_and_code_injection}
Such techniques allow to dynamically modify the code of a running process. In this way, the attacker is able to analyze functions or system calls, as well as their parameters and return values, and modify the behavior of the original functions. 

There exist a lot of tools that support code instrumentation and injection, as well as the corresponding runtime analysis. Nonetheless, Xposed \cite{xposed} and Frida \cite{frida}  are currently the \textsl{de-facto} standards.
Xposed is a framework that applies add-ons (called \textsl{modules}) directly to the Android OS ROM and requires root privileges. Such modules may allow, e.g., customizing the script that spawns any new process from the  Zygote one\footnote{The Zygote process is responsible for spawning new process to host launching apps.}, in order to add a jar file that allows hooking. % To achieve this, Xposed needs root privileges.

Frida is a dynamic code instrumentation tool that allows an attacker to hook functions by injecting a JavaScript engine into the instrumented process; the engine then allows injecting executable code by directly modifying the process memory. Frida can work on both rooted and unrooted devices in three different modes:
\begin{itemize}
    \item \textsl{Injected mode}: this is the most common deployment in which the user installs and runs the frida-server (i.e., a daemon) into a rooted device that exposes the frida-core module over TCP (usually on port 27042). 
    \item \textsl{Embedded mode}:  the user repackages the app with the frida-gadget (i.e., a shared library). This library allows instrumenting the app on an unrooted device.
    \item \textsl{Preloaded mode}: the frida-gadget shared library is injected inside the operating system layer instead of the application layer (as in the embedded mode). It works on rooted devices only.
\end{itemize}

Code instrumentation and injection allow stealing the actual values of program variables from a running application.
For example, the attacker could hook the function that decrypts some portion of code. In this way, he is able to recover the key for that specific chunk and the plain text. 
Then, the attacker can replace the encrypted code of an anti-repackaging check with a crafted one, by exploiting the binary patching technique previously discussed~\cite{owasp-mstg}.  

From the anti-repackaging standpoint, it is a hard task to safely hide checks that are resilient to code instrumentation and injection. As a matter of fact, system call hooking allows in principle to detect and attack any anti-repackaging check even if it is based on some kernel-provided functionality. In fact, Frida allows hooking tampering detection functions,  and makes them return the attacker's desired value. In addition, some “anti-frida” controls (e.g. simply check if the tcp port 27042 is open) relies on system call and can be circumvented by Frida itself.

An attempt to limit function hooking is proposed in \cite{10.1007/978-3-030-45371-8_12}, where some Java instructions are translated into native code to elude Java code instrumentation and avoid an attacker to recover the original statements. % However, code instrumentation is as difficult in native as it is in java code. 

\subsection{Network-based attacks}\label{subsec:network-attacks}
Previous attacking techniques focus on the device, the OS and the app. However, it is also possible to attack anti-repackaging at network level. Such attacks can be passive, i.e., the attacker does not affect the network traffic (e.g., \textsl{sniffing attack}) or active, i.e., the attacker willingly affect and spoof the traffic, (e.g., \textsl{replay attack}). 

\paragraph{Sniffing attack.}\label{paragraph:sniffing_attack}
It refers to the interception and the analysis of data exchanged by two parties on a communication channel (e.g., an app interacting with a remote server)~\cite{capec-157, capec-609}. 
This attack is relevant as some anti-repackaging checks are executed at server side. If an attacker understands the communication pattern and which data are sent between parties, he could be able to detect and circumvent these controls~\cite{owasp-m3}. %\luigi{al posto di "and circumvent these controls, inserirei "and retrieve critical information"}
For instance, an attacker is able to read the client-server communication if it is over \textsl{http}.

\paragraph{Replay Attack.}\label{paragraph:replay_attck}
The replay attack (or Man in the Middle attack - MitM) extends the sniffing attack by actively interacting with the two parties.  The attack dynamically affects the data exchanged during the communication, by relying on a MitM proxy~\cite{capec-94}.
Concerning anti-repackaging, if the signature check of an $apk$ is carried out at server side, then the client has to send the checksum of its certificate and an attacker could change the communication data in order to trick the server, or spoof a fictitious response from the server. Albeit all anti-repackaging techniques discussed in Section \ref{sec:sota} leverage local checks only, there exists some proprietary solutions which provides remote anti-repackaging detection, like Google safetyNet~\cite{safetynet}. The safetyNet API is provided by Google to Android developers, and can be included in any app. Such API provides functionalities against several security threats and specific checks against repackaging, which are applied both locally e.g., emulator detection, and remotely, e.g., signature detection on the server side. In this case, the attacker can try modifying the network traffic generated by the safetyNet API calls, to bypass server-side checks or spoof a fake answers from the server. Furthermore, the attacker can remove the invocation to safetyNet API functions by directly patching the smali code (or native one) by leveraging code deletion (Section \ref{subsec:code_delection}).

It is worth pointing out that MitM attacks can be carried out also inside the $apk$ itself: in this scenario, the attacker could modify at runtime some data using some of the code/data manipulation techniques previously discussed, with the aim to bypass specific anti-repackaging checks. The main idea is that an attacker could replace some resource file in order to bypass specific controls which rely on the app data
%\alessio{its: who are you referring to?}\luigi{the app} data
 (e.g., modify the path from the repackaged resource into the original one)~\cite{Norboev2018OnTR, 8186215}.

%\alessio{We need to decide whether to add the table or not. If it is too redundant, maybe we can drop it out.}


%\subsection{Google safetyNet notes}\label{sec:overview}

%\alessio{The following sentences need to be placed in previous subsection. TBD.}



%Some techniques explained above are very hard to prevent even with an anti repackaging defense. One possible approach is to make that “attacks” impractical and too costly. This solution doesn't solve the problem, but matches with the assumption that an attacker repacks an application only if it is more convenient than developing a new version of that application from scratch. 


==> sections/old paper files/background.tex <==
\section{App Repackaging: Backgroud and Threat Model}\label{sec:background}

In this section we briefly recap the basics of app development and distribution in Android. Then, we discuss a threat model for app repackaging, and we summarizes the main categories of repackaging detection and anti-repackaging techniques.

\subsection{Android App life-cycle}

\paragraph{App development.} A native Android app is developed in Java or Kotlin, and leverages XML files to represent the graphical user interface of the app. From now on, we will explicitly refer to Java code, although the same techniques are valid also in case of Kotlin-based apps. There are other ways to develop Android apps, for example hybrid apps. Hybrid apps are mainly built using web technologies and run over a WebView (e.g., Apache Cordoba\footnote{https://cordova.apache.org/}), and are likewise weak against repackaging. 
%Hybrid apps present the same vulnerability about repackaging as native apps. 

Each Android app is distributed and installed as an Android Package ($apk$) file. Until 2018, developers had to build their $apk$ file to distribute their app.
Since 2018 Google provides a new publishing format, i.e., the Android Application Bundle (AAB) \cite{android-app-boundle}, which allows building optimized $apk$ for each device configuration\footnote{Hereafter we will refer to $apk$ only, as the distinction between AAB and $apk$ is irrelevant for the problem at stake.}. 

In a nutshell, an $apk$ file is a zip archive containing all the necessary files to run the first execution of the app.
Each $apk$ is signed with its developer's private key and also contains the corresponding public certificate of the developer. This mechanism grants the integrity of the $apk$, but cannot provide any authentication, as the developer certificate does not need to be issued by a trusted certificate authority. Therefore, Android performs only basic verification on the $apk$ structure and its integrity, thereby leaving the decision to install the app (and, consequently, to trust the source of the app) to the final user. 

Regarding app repackaging, the most relevant files and folders contained in the $apk$ are:
\begin{itemize}
  \item \emph{META-INF/}: it contains the developer's public certificate and the app signature;
  \item \emph{lib/}: it contains the native libraries for each specific architecture (e.g., x86, armeabi\-v7a). An app could excute native C/C++ code through the Java Native Interface (JNI)\footnote{https://developer.android.com/ndk};
  \item \emph{res/}: it contains the binary resources, such as images or hybrid apps content;
  \item \emph{AndroidManifest.xml}: it describes the structure of the app and its components. In this file the developer defines app permissions, entry points, intent filters, and more;
  \item \emph{classes.dex}: it contains the compiled Java/Kotlin code in the form of bytecode, i.e., a high level representation of the machine code, that could be converted into Smali code, i.e., a human readable format, with off-the-shelf tools like Backsmali \cite{backsmali}. 
\end{itemize}

\paragraph{Application distribution.}
Android apps are mainly delivered through proper software repositories, called \textsl{app stores}, which allow developers to publish their $apk$. iOS relies on a single, centralized market  (i.e., the Apple Store), which is directly controlled by Apple. On the contrary, a distinctive feature of Android is the possibility to distribute the same app on dozens of different app stores beyond the official one (i.e., the Google Play Store\footnote{\url{https://play.google.com/store}}).  The most popular app stores differ from region to region. In Europe and US, the Google Play Store has the greatest market share \cite{android-markets-2019}. However, in 2019, in China, \textsl{Tencent My App} was the biggest Android app store with up to 25.5\% of the market share, followed by the \textsl{360 Mobile Assistant} and \textsl{Xiaomi App Store}; in this country the Google Play Store is just tenth place \cite{china-markets, android-markets-2019}. 

Whenever a user downloads an app from any store, Android carries out a soft check on the app certificate before installation, with the final decision left to the user~\cite{android-publish-app}: we recall that an $apk$ has to be signed by the developer, but Android continues the installation even if the signer of the developer's certificate is unknown~\cite{android-apk-authenticity}.
Since the only constraint is a valid signature, it is also possible to distribute the $apk$ directly (e.g., through email or urls) without the need to upload the app on an app store. %For example, a developer can publish his app over the web. This process is possible if user enable app installation from unknown sources in system settings. 

\begin{comment}
Io metterei qua l'immagine del flusso blu senza step 2 e direi una qualcosa del tipo (prendendo spunto da quello che hai detto tu nel capitolo dopo).
The common distribution process is briefly described below:
\begin{itemize}
    \item An individual or a company develop and build an Android app;
    \item An android app (apk or aab) is published in one or more application markets;
    \item An user can access to the published app in severall of different modes, the most common is searching on markets;
    \item An user can download and install the apk directly from the markets. The installed apk files are stored in \emph{/system/app/} or \emph{/data/app/} and can be execute by users
\end{itemize}
\end{comment}

\subsection{App Repackaging: Threat model}\label{sec:threat-model}

\begin{figure*}[!ht]
  \includegraphics[width=\textwidth]{figs/threat-model.pdf}
  \caption{App repackaging: Threat model.}
  \label{fig:threat-model-design}
\end{figure*}

In this section we discuss a threat model for app repackaging. The model is depicted in Fig. \ref{fig:threat-model-design}. 

The threat model involves three actors, namely the developer, the attacker and the user. The developer implements the app (Step 1), and may also add some anti-repackaging protection in the code before building the $apk$ (Step 2), in order to counteract repackaging attempts. In general, applying an anti-repackaging technique means to add some extra code that may lead, for instance, the repackaged app to crash. Then, the developer builds and signs the $apk$ and delivers it to the app store (Step 3). 

In an ideal (i.e., attack-free) scenario, the user fetches the store for apps (Step 4), then chooses and downloads the original $apk$. The validity of the signature and the integrity of the $apk$ is verified automatically by Android, by leveraging the developer's public key certificate provided in the $apk$. Then, the $apk$ is installed successfully and the user can execute the app (Step 6).

In an actual use case, an attacker can download the developer's $apk$ by behaving as any normal user. Then, the attacker decompiles and analyzes the $apk$ (Step 7), and tries to detect the anti-repackaging protections (Step 8). More in details, the attacker can decompile the $apk$ using Apktool~\cite{apktool} and perform static analysis on the smali source code. Smali is a human-readable format that can be obtained from the Dalvik bytecode contained in the $classes.dex$ file. Most of the smali code could be further decompiled back into Java code~\cite{10.1007/3-540-45937-5_10}. If static analysis is not sufficient, an attacker can dynamically infer the app behavior at runtime, by relying, for instance, on Frida \cite{frida}. A fruitful combination of static and dynamic analysis can allow the attacker to detect the anti-repackaging protections added by the developer in the app code.
In case some protections are detected, the attacker tries to neutralize them (Step 9) by deactivating the corresponding extra code, accordingly. Then, he can add some malicious code (Step 10) and build and signs a repackaged version of the $apk$ (i.e., $Rep_{apk}$) with a valid self-generated public key certificate. Finally, the attacker tests $Rep_{apk}$ on her own devices (Step 11). In case it works, the attacker can try distributing $Rep_{apk}$ (Step 12) both on official channels (i.e., app stores) and side-channels (e.g., by email, on website, through phishing attacks, \ldots). Otherwise, the 
attacker needs to carry out further analysis on the $apk$, and repeat Steps 7 to 11 (also known as the \textsl{try and error cycle}) until she obtains a working $Rep_{apk}$. 
%Then, the attacker redistributes $Rep_{apk}$ (Step 12) in order to reach the user, by trying to i) upload it on an app store, or ii) send it directly to the user by means of phishing attacks.

The attack succeeds whether some users install $Rep_{apk}$ instead of the original $apk$. In this case, the execution of $Rep_{apk}$ leads the user to execute the malicious code on her own device. The malicious code may have different aims, like e.g., access the app premium features for free or redirect revenue to cause financial loss to the developer, gain access to the user's private in app data (e.g., credentials), or make the app willingly unstable to affect the reputation of the original app.
%The attacker get access to the public store and retrieve the $apk$ provided by the developer. 

%ndividual or a company who develops an Android app (step 1). Once the app is ready to be published, it is possible but not necessary, to apply different protections with different goals (step 2). In our case we focus on repackaging avoidance protections (also known as anti repackaging or anti tampering). Once the application is built, developer can publish the APK (or the Android App Bundle) on various markets (step 3). 

%Users can now access to the app in dozens of different modes, the most common is searching on markets (step 4). An app it's downloaded and installed in the device as APK file. (step 5). Installed APK file are store in /system/app/ or /data/app/ and can be execute by users (step 6). 

%This first part of the process, represented in blue in the image, is the expected developing and consuming app flow. In addiction to that, we highlighted in red the process of an attacker who wants to repack the app.

%We assume that an attacker has full access to his device, including root access. The first stage for an attacker is to analyze the target APK (step 7).  (step 8). 
%The purpose of the analysis process is to find out the application logic, to inject the attackers code, such as ads or malicious code (step 10).
%In order to make the repackaging process more difficult, a developer can an apply different controls and protection to the application (step 2). This additional code aims to crash the app if some tampering is detected.
%With tampering controls the attacking process in more difficult. In the analysis phase, an attacker should detects repackaging controls (step 8).To neutralize these protections (step 9), the evil subject modify the source code and the resources of the app, injecting, modifying or removing code. 
%Only once repacking detection is defused, it is possible to add malicious code (step 10).
%Now the evil app is ready to be distributed on the market (step 11). The APK file should be build and signed by the attacker using its own certificate (which is different from the original app's owner certificate). Now we have the presence of a malicious APP1, repacked from APP, inside some app stores. Many users have now access to APP1. 
%The final step for an attacker is to force to download APP1 instead of APP (step 12). Phishing techniques can be applied to trick the final user to download and execute APP' instead of APP. Furthermore the evil subject can send directly the APP1 APK file to his victim using instant messaging or emails. 

%In the rest of the paper we will focus on discussing the state of the art of anti-repackaging on Android (Step 2). %, with a specific focus on \textsl{repackaging avoidance} techniques. 
%Furthermore, we will analyze the main attack vectors (Steps 8 and 9) against such techniques, with the aim to point out their weaknesses. %The attacker can always bypass these techniques using a "try and error" approach and achieve APP' step 6 successfully. Find and neutralize implemented defenses, however, could be harder than add malicious code. In our threat model we highlighted this difficulty with step 13, where the attacker has to evaluate the goodness of his repack. Eventually it may be necessary to return to step 7.
%Then, we will discuss a model for the optimal anti-repackaging technique, which is expected to be resilient to the current attack vectors. It is worth noticing that the more reliable is the anti-repackaging technique, the lower is the probability for the attacker to obtain a working repackaged app (Step 11). In this case, the attacker may find repackaging as a non cost-effective activity to target mobile users. 

\begin{comment}
\paragraph{Motivation}\label{par:threat-motivation}
Legitimate app can be repacked with different purposes:
\begin{enumerate}
	\item Access app premium features for free or redirect revenue, for example changing ads owner, causing financial loss for developers ~\cite{}.
	\item Change app behavior in order to gain users private or in app data, such as credentials.
	\item Use app as malware carrier.
	\item Make the app unusable to damage the company image.
\end{enumerate}
Only in scenario 1 the attacker is obliged to remove or bypass every control to be sure that the repack works perfectly.
On the other hand, in scenarios 2,3,4, the attacker needs that the repackaged app runs for a sufficient period of time to perform the attack (e.g. steal the credential).

Moreover, the repacking threat allows an attacker to hide malware under popular and well ranked apps. In this way, he could camouflage his evil application as the original and benign one, easily spreading it to a huge number of people.

\end{comment}

\subsection{Repackaging Detection vs. Anti-Repackaging}\label{sec:threat-mitigation}

This section points out the main features of both \textsl{repackaging detection} and \textsl{anti-repackaging} techniques. 
%pro and cons of different approaches to repackaging threat. 
%Repackaging detection and avoidance are two different techniques %that wants to achieve different goals. In the following paragraphs we are going to discuss both in depth. Note that our focus is repackaging avoidance state of the art review.

\subsubsection{Repackaging Detection}\label{subsec:repackaging-detection}
Repackaging detection focuses on recognizing repackaged apps in app stores or on user's devices, with the aim to limit the spread of repackaged app (i.e., Step 12 in Figure \ref{fig:threat-model-design}).
Repackaging detection techniques can be divided into static and dynamic approaches \cite{10.1016/j.procs.2016.02.006}, and further grouped into five different categories (see \cite{10.1109/TSE.2019.2901679}). 
\begin{itemize}
    \item \textbf{Static or offline techniques} are adopted on \textsl{app stores} to identify uploads of repackaged apps which are clones of original apps. 
    Such techniques strongly relies on \textsl{symptom discovery} or \textsl{app similarity}. Symptoms \cite{10.1109/TSE.2019.2901679} are tracks, such as strings, left by the repackaging process itself. Similarity checks usually involve a two-step process in which each app is first profiled according to a set of distinctive features; then, apps with almost identical feature profiles are identified.  Such techniques make strong use of machine learning, both supervised \cite{0.1109/SPW.2016.33, Lin2013IdentifyingAM} and unsupervised~\cite{10.1007/978-3-319-23829-6_30}. 
    Static analysis needs a considerable amount of resources both in order to generate the decision model and to make the final decision, and can be efficiently applied only on server side.    
    \item \textbf{Dynamic or online techniques} are directly executed on the user's device to evaluate the app.
    These approaches extract specific information both at install-time and at run-time. For instance, the technique discussed in \cite{10.1145/2484313.2484315} puts a watermark inside the app which is checked by a third authority at runtime.
\end{itemize}

\paragraph{Attacking Repackaging Detection.} An attacker successfully circumvents a repackaging detection technique once it is able to build repackaged apps that go undetected both on the app store and on the devices. According to the characteristics of the current detection techniques, this means that the repackaged app must appear very different from the original app (to bypass similarity checks), hide repackaging identifiers (to avoid symptom discovery), and behave as the original app to circumvent dynamic analysis.  
It is also worth pointing out that the granularity of the Android ecosystem - which allows to deliver apps through an undefined number of app stores and side channels (e.g., apps available at some URIs or delivered by email) - makes hard to build up a reliable, pervasive and full-fledged repackaging detection deployment. In fact, this would require to deploy static analysis mechanisms on each source of apps (i.e., app stores and servers), as well as dynamic analysis solutions on each mobile device.
%in fact, enforcing repackaging detection in a pervasive and exhaustive way is tricky, as the granularity of the Android ecosystem 

%In a detection techniques an attacker should focus on how the detection model could be bypassed. If the perfect model, the one with 100\% accuracy and recall, 0\% false positive and false negative, existed then there would be no hope for attackers. 

%Due to the vast granularity of Android ecosystem, as already show in \autoref{sec:background}, is impossible to impose a central authority that guarantees repackaging detection to every Android device.

\subsubsection{Anti-Repackaging}\label{subsec:repackaging-avoidance}
Anti-Repackaging - also known as \textsl{repackaging avoidance} or \textsl{self-protection}
%\footnote{Hereafter, we use these names interchangeably.}
 - aims to protect an app from being successfully repackaged. As opposed to repackaging detection, anti-repackaging is applied by the developer to the app code before building the $apk$ (Step 2) and aims to make any repackaged version of the same app crash. On the bad side, the attacker aims to detect and neutralize the anti-repackaging protection after reversing the $apk$ (Steps 8 and 9). 
From a technical standpoint, anti-repackaging techniques insert some logic controls (i.e., \textsl{anti-tampering} checks) inside the $apk$. %\alessio{From here.} 
%These integrity controls are called anti tampering (AT) checks. 
%An attacker in step 8 of our threat model can detect these protections, and eradicate them in step 9. 
Since the first aim of the attacker is to recognize anti-repackaging, the requirements of anti-tampering checks are i) to go undetected and hide inside the app code, and ii) in case of detection, to avoid being de-activated. To achieve such results, anti-tampering checks may rely on code obfuscation, code virtualization and anti-debugging techniques.  We briefly introduce anti-tampering checks and such techniques.%In our scope make the attacker process hard is not sufficient, the optimal repackaging avoidance technique does not allow the control to be removed. 

\paragraph{Anti-tampering.} In a nutshell, anti-tampering checks are self-protecting functions which aim to detect any modification on the original app. There exist several methods to detect tampering in mobile apps, as highlighted in \cite{BERLATO2020102463}. 
The most relevant anti-tampering techniques are:
\begin{itemize}
    \item \textbf{Signature checking}: the most trivial control, which checks the certificate contained in the $apk$. This approach could detect any modification applied to the original $apk$;
    \item \textbf{Code integrity}: it checks whether some specific part of the code has been tampered with, by computing its signature at run-time. As an example, the first bytes of the \emph{.dex} file contains the hash of its content. This method detects a tampering only if the attacker has modified the checked methods;
    \item \textbf{Resource integrity}: it checks the signature of some resources at run-time. 
    This technique differs from the previous ones as it checks tampering attempts in the app resources (e.g., images and other binary files) instead of the code;
    \item \textbf{Installer verification}: it checks if the installing app comes from trusted app stores. This technique is applied under the assumption that tampered apps are more likely to be distributed on unofficial app stores.
\end{itemize}
Anti-tampering checks dynamically react to any modification either in the app or in the executing environment. 
Once some checks are detected by the attacker (Step 8 in  Figure \ref{fig:threat-model-design}), the same attacker tries to bypass them by following the \textsl{try and error} approach, i.e., she modifies the app (in order to try removing checks), then she repackages and tests the app to check whether it works properly. If the attempt fails, then the attacker may try to search for other checks and/or modify the app in a different way.

\paragraph{Code obfuscation.} Obfuscation approaches modify the bytecode or the source code of an app, without changing its behavior, in order to make some manual or automatic analysis more difficult. There exist a lot of off-the-shelf obfuscation tools both open source \cite{aonzo2020obfuscapk} and commercial \cite{proguard}. %In \cite{10.1016/bs.adcom.2017.09.004} Banescu et al. presented the MATE (Man At The End) attack model. This model is applicable in repackaging threat. Authors  proposed a list of techniques, based on code obfuscation, that protect from MATE attack model.   %These techniques aims to make harder the step 9 \autoref{fig:threat-model-design}.

\paragraph{Code virtualization.}
Code virtualization is a specific obfuscation scheme. In this approach, instructions are mapped to semantically-equivalent virtual instructions. A virtual machine (VM) executes inside the app and interprets the virtual instructions. Two different approaches are proposed in \cite{10.1145/2557547.2557558, 2019-exploiting-binary}; the first one works at DEX level, while the latter focuses on native libraries. %These works proposed themselves as effective countermeasures against static analysis, dynamic analysis, and specific analysis for virtual machines.
Similarly to obfuscation, this approach aims at complicating the reverse engineering process of an app, but it does not introduce any anti-tampering check.

\paragraph{Anti-debugging.} Anti-debugging controls aim to detect and avoid dynamic analysis checks (e.g., debugger). Differently from passive obfuscation techniques, where the app code is syntactically modified to make it harder to understand, anti-debugging controls allow an app to actively react against malicious reverse engineering  at run-time \cite{BERLATO2020102463}.
The most widespread anti-debugging techniques are:
\begin{itemize}
    \item \textbf{Emulator detection}: it checks whether an application is running on a real device or in an emulated environment;
    \item \textbf{Time check}: when an app executes with a debugger, its execution slows down. Time checks can be specific functions whose execution depend on the execution time: in case the execution time is higher than a given threshold, such functions take the app to an inconsistent state;
    \item \textbf{Check debuggable}: the \emph{AndroidManifest} contains a flag that enables the debugging mode: if this flag is set to false, an user is not able to attach any debugger to the application. The attacker can bypass this check by changing the manifest accordingly. Nonetheless, such modification could trigger some other anti-tampering checks.
\end{itemize}
Recently, more complex anti-debugging techniques have been put forward~\cite{10.3390/s19112625}. Among these, the most promising one is discussed in \cite{article}: the intuition is to exploit proper features of the Android Runtime to hide anti-debugging instruction at runtime. As any other solution relying on version-specific features of the Android OS, also this approach quickly became obsolete, as it worked properly only up to API 25 (i.e., Android v. 7.1).

%In this section we briefly introduce some basic concepts related to both anti-repackaging detection and avoidance; in the following section, we will analyze in detail the state of the art related to the latter category. %\ref{sec:sota}.
\begin{comment}
A logic bomb is a piece of code which will bring the app in some undefined behavior, such as crash or inconsistency, when specific trigger conditions are satisfied \cite{10.1145/3168820}.
Logic bombs use a combination of what has been described above to achieve the repackaging avoidance purpose.

\begin{figure}[H]
  \includegraphics[width=\linewidth]{images/repack.png}
  \caption{Logic bombs design}
  \label{fig:bombs-design}
\end{figure}

The last formal definition of logic bombs is proposed in \cite{10.1007/978-3-030-45371-8_12}. 
\figref{fig:bombs-design} shows how to generate a basic cryptographically obfuscated bomb. The left box contains the original code. Firstly the trigger condition "v == constant" is transformed into "Hash(v) == Hc", where Hc = Hash(constant). The value of variable v is then used to decrypt the original code. As shown in right box inside the original code could be performed various checks in order to evaluate app and environment integrity.
In this structure, where the hash function is used to hide the encryption key, the logic bombs can be inserted only in specific portion of code where are present the trigger condition.

A set of logic bombs represents an anti repackaging technique: a methods that allows the developer to protect his app from the repackaging and all attacks that we will explain in the \autoref{sec:attacking_model}. In addition, these logic controls rely on AD and AT controls to detect any environment or application alteration.


\end{comment}





==> sections/old paper files/bestdefensetecnique.tex <==
\section{Utopian defense technique} \label{sec:best_defense_technique}
In this section we propose the characteristic of different approaches which aim to prevent the repackaging threat. In all this tree cases, we base our assumption on the fact that users are not colluded with attackers. Our goal is to show the characteristic of these features without considering if they are achievable or not.

\paragraph{Part I}
As shown in \ref{sec:background} in Android is possible to install apps from different sources. In other operating systems the only place to download apps is from unique central repository, called store. iOS apply this policy. There are several techniques to bypass this restriction \cite{doi:10.5465/ambpp.2013.13947abstract}, however we can assume a user not colluded with attackers won't overcome these type of protections.

Inside the unique store is possible to implement the perfect static repackaging detection techniques. When a user submit an application to the central repository, controls are performed to identify similarities with all the other apps present inside the store. In this way repacked applications are detected and not published. 
It is out of our scope evaluate a perfect repackaging detection technique. Thanks to this central control, repackaging protection inside the app would be useless.

Unfortunately, this is in contrast with the openness Android philosophy and fragmentation in mobile devices market.

\paragraph{Part II} 
% gli attacchi sono sempre possibili, ma cerco di proteggere tramite controlli server-side (come se mi costruissi la mia CA)
% Parte di analisi generale su eventuali caratteristiche
In this paragraph we want to study which protection could be implemented inside apps that rely on network communication. We will therefore discuss self-defending technique based on a client-server architecture. 

We assume that all attacks presented in \autoref{sec:attacking_model} can be performed. In this scenario, our goal is to design a defense architecture that is resistance (against repackaging, not the above attacks) and that relies on server integrity controls: the server works as authority that detect possible tampering.
With this structure, the application hides any AT or AD functions server side. Moreover, the app flow depends on the server response, which should be different at each new request.

The apk (client side) have to send some app or environment information to its backend in the safest possible way. For example an application could encrypt the payload of each request with different communication keys, or could use custom communication protocols. In other words, the main goal related to this design is to make the attacks described in \autoref{paragraph:sniffing_attack} and \autoref{paragraph:replay_attck} ineffective.

% Breve analisi su vantaggi/svantaggi
With a client-server architecture, all static analysis are bypassed and the goal for an attacker is to understand call pattern. This task could be very time consuming because the server side functions are a blackbox and its services cannot be reverse engineered.
Furthermore, this approach could allow developer to update the AD and AT functions without any impacts to the client side.

This area of research has already been deepened in other studies, such as \cite{10.1145/1230040.1230087, 10.1145/2991079.2991119, 10.1145/2043628.2043633}. In online video game attackers try to modify the game client in order to cheat, or play without paying. This situation is similar to that of repackaging in Android apps.
From another point of view, this technique doesn't solve some of the common attacks, but tries to create an architecture that can limit them. This means that an attacker could still create a working repackaged app with an hard and time consuming work. Contrary to the state of the art defending methodologies, this architecture allow a developer to change the API interface in order to lose backward compatibility with old version of an app. In this way, the app users are forced to update their version, but a repackaged app will stop working.

Another possibility that involves the presence of a central authority (CA) is that app developers can share a secret between their app server and the central authority itself. A scheme that includes CA, device operating system and developer server could guarantee that the communication to developer server can only happen through the legitimate app. In this way repackaged apps can't reach the server.

\paragraph{Parte III} 
In order to ideally protect apps from repackaging, we have to mitigate the underling problem. An attacker could apply different attacks (presented in \autoref{sec:attacking_model}) to analyze, understand and circumvent the app AD and AT controls. Once the attacker understand the protection model, he is able to remove this controls patching the bytecode. This is the required step to create a fully working app bundle (apk) that could be shared in an app store. 
Due to this, if a developer is able to avoid the code manipulation threat \autoref{subsec:code_manipulation} (both code deletion and binary patching), the repackaging threat could be exceeded. 

Unfortunately, this threat cannot be solved with the state of the art anti repackaging techniques. These approaches implement several strategies which aim to make more difficult some attacking models.
In this way, the best defending technique is the methodology that mitigate the largest number of threats and makes more difficult the attacking process. 

For example, the technique implemented by Bombdroid (introduced in \autoref{subsec:bombdroid-2018}) is strong against static analysis and a trivial code deletion. We have shown as dynamic analysis procedures such as code instrumentation \autoref{subsec:code_instrumentation_and_code_injection}, could be used to recover deciphered code and the encryption key. With these information, an attacker is able to create a repackaged version from the original app.
In order to make Bombdroid the perfect self-defending technique, authors should mitigate all possible dynamic analysis. Is out of our scope to determine whether this task is achievable or not .

As described in \autoref{sec:background}, the repackaging threat id due to the possibility to decompile and analyze an apk. Another technique to avoid this threat is to prevent the file extraction from the app bundle: if is impossible to get out the files in an apk, an attacker could not recover the source code and resources. In this way is not able to create a repackaged version of the original app.

\begin{comment}
Scaletta / Considerazioni
 -) Analisi statica: obfuscation, cifratura o scaricare il codice solo quando serve (ad esempio con dynamic delivery -> https://developer.android.com/guide/app-bundle/dynamic-delivery)
 -) Fuzzing/Symbolic execution -> ?!? -> non so neanche se avrebbe senso, posso sempre inserire e runnare l'app quante volte mi va!
 -) Debugging -> in teoria se un apk ha la flag debuggable a false non può essere debuggato nel modo classico. La flag però puo essere cambiata on the fly con tool come Xposed (ma lo metterei in un altro capitolo). In aggiunta check tempo o altri metodi classici.
 -) Process Exploration -> ?!? -> si potrebbe vedere come funzionano i singoli tool per fare avoid del singolo tool (tipo per frida), ma non è una cosa generica che mi piace.
 -) vtable Hijacking -> esistono lavori che analizzano e mitigano il problema (come VTPin - https://download.vusec.net/papers/vtpin_acsac16.pdf - https://github.com/uberspot/VTPin) -> Io credo che questo più che un problema legato al repackaging, può essere visto come un problema "strutturale" del come vengono richiamati i metodi virtuali nella VM di Java e quindi non lo considererei nel nostro lavoro
 -) Code deletion -> il flusso deve dipendere da quella "porzione di codice" e il suo risultato non deve essere si/no o predeterminabile, altrimenti può essere facilmente hardcodato
 -) Binary patching -> ?!? -> Credo che evitare questo sia davvero impossibile. In generale pensavo che se il bytecode è cifrato il patching è impossibile finchè non viene recuperata la chiave di decifratura. In alternativa si può offuscare pesantemente il codice (sarebe piu difficile da modificare). In generale mi piacerebbe trovare qualche considerazione più "forte" di questa
 -) Code Instrumentation -> ?!? -> In generale ci vorrebbe una tecnica che non richiama funzioni e/o che non faccia syscall (come se fosse un modulo in mutua esclusione rispetto tutto il resto). Non esiste neanche un tecnica generica perchè esistono tanti tool diversi (e.g. frida, xposed) che lavorano in maniere differenti. Possono aiutare i check dell'environment, ma non risolvono!
 -) replay attack variante -> ?!? 

In generale contro ogni analisi dinamica (e cumulative attack) si può aggiugere "randomicità" ai controlli effettuati

Altra cosa se avevamo detto era quella di aggiungere una soglia di "bontà" delle trigger condition, e.g. non ci piacciono trigger condition nelle librerie o per valori che sono compresi in piccoli range.

NB: tratto da https://stackoverflow.com/questions/17225590/prevent-make-it-difficult-to-patch-binary-assembly
Write self modifying code
Again this thwarts static analysis. For example if your jump into the verification function does not exist in the binary but is patched everywhere as part of some init() function in the .so
\end{comment}



==> sections/old paper files/conclusion.tex <==
\section{Discussion, Conclusion and Future Work}
\label{sec:conclusion}
In this paper, we discussed the state of the art of anti-repackaging techniques, unveiling their limitations and the way to attack them.
Such techniques are far from being robust against the available attacking vectors.   We argue that improving the reliability of anti-repackaging on Android demands for developing novel methodologies that can discourage an attacker from trying to deactivate them. Future anti-repackaging approaches should follow some guidelines, derived from the lesson learned:
\begin{enumerate}
    \item \textbf{Use multiple patterns}. Current techniques adhere to a common pattern (i.e., qualified conditions, adoption of hash functions, \ldots), which we showed to be rather easy to detect and de-activate by an attacker. The same anti-repackaging scheme should implement several distinct patterns to disseminate logic bombs in the app. 
    Furthermore, as we shown in NRP, a single anti-tampering control could be easily bypassed by an attacker. Therefore, several heterogeneous anti-tampering controls must be distributed thorughout the app.
    \item \textbf{Rely on native code}. As reversing and instrumenting native code is more complicated than bytecode, both logic bombs and their triggering conditions should be moved to native as much as possible. 
    \item \textbf{Optimized pervasiveness of the logic bombs}. Some approaches implement few controls in the name of performance, while others embed a lot of bombs which are not actually triggered at runtime. In this respect, there is the need for a more effective deployment of logic bombs, also at the cost of higher time and space overheads.
    \item \textbf{Honeypot bombs}. Proper fake bombs can be added to disguise the attacker to remove them. The removal of such bombs should trigger the real ones and lead the app to crash. This idea has been proposed in literature but never actually applied in current proposals, where the focus is more on generating stealthy logic bombs. 
    \item \textbf{Hiding anti-repackaging protection}. It is fundamental to improve the stealthiness of anti-repackaging to make hard for the attacker to understand that the reverse-engineered app actually contains some protection. Therefore, obfuscating anti-repackaging and anti-tampering controls may help.
    \item \textbf{Mixed Client-side and Server-side controls.} Most of the proposals check the app directly on the device (client-side) while others adopt remote controls (server-side) only. A more effective anti-repackaging protection must combine both of them. Furthermore, runtime-generated server-side controls can improve undetectability.
\end{enumerate}

As a future extension of this work, we plan to implement an anti-repackaging solution that we already designed according to the previous guidelines. We plan to assess it on a high number of Android apps, and to make both the source code and the experimental results available to the research community.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:




==> sections/old paper files/intro.tex <==
\section{Introduction}
\label{sec:intro}
During the last five years, Android strengthened its leadership among mobile operating systems with more than 75\% of market share on average~\cite{statcounter:2019}.
Most of this success is due to the app development process, which  is easier compared to other mobile operating systems: in fact, Google currently offers a plethora of platforms that support the developer in designing, implementing, testing and sharing her application~\cite{android-developer-guide}.
As a consequence, the number of Android apps in the Google Play Store reached 2.8M in 2020\footnote{https://www.appbrain.com/stats/number-of-android-apps}. 

From a security standpoint, Android apps are the main target for attackers, as they allow to reach a large number of mobile users. In fact,
%Because of the large number of applications and their usage, attackers are encouraged to write exploits against the Android OS and its apps in order to attack a large numer of users.  
since a mobile app is available in public app markets (e.g., Google Play Store, Samsung App Store, \ldots), an attacker can easily retrieve the app bundle (i.e., the $apk$ file, which is basically an archive containing the app). Then, the attacker can reverse engineer the $apk$ \cite{2011-android-reversing}, inject some malicious code, and re-distribute a modified version of the original app. This kind of attack is called \textsl{repackaging}.

%Once the app is obtained, then reverse engineering can be performed to extract sensitive information or to craft a modified version and share it in app stores or over the internet . This type of attack is known as repackaging. 

Android repackaging is a serious problem that may affect any unprotected app. A repackaged app can cause money losses for developers as the attacker can re-distribute paid apps for free, remove/redirect ads earnings, or make the app willingly unusable to negatively impact the reputation of the developer.
%Furthermore malicious code can be added inside the apk in order to cause damages to user devices. 
Furthermore, recent studies~\cite{10.1145/3017427} demonstrated that the 86\% of Android malware is contained in repackaged apps. This is indeed a promising strategy for malware developers, as embedding the malicious code in a repackaged version of popular and well-ranked app speeds up its spread.

It is worth pointing out that repackaging is intrinsically related to the Android development life-cycle, where an $apk$ just needs to have a valid signature in order to be successfully installed and execute properly, without requiring any guarantee on the actual identity of the signer (i.e., the developer does not need a valid public key certificate issued by a trusted certificate authority). Therefore, an attacker can modify an existing $apk$ and then repackage and sign it with her own self-generated private key. 

In order to make the repackaging phase more challenging for attackers, in recent years several techniques have been proposed in literature. Such techniques can be divided into two sets, namely \textsl{repackaging detection} and \textsl{anti-repackaging}: the first set aims at recognizing repackaged apps, while the latter one focuses on inserting proper controls in the app, such that a repackaged version of the same app would not work properly. 

%The threat model will be discussed in deep in \autoref{sec:threat-model}.
While repackaging detection techniques have been widely discussed and analyzed in literature \cite{Zhan2019ACS, 10.1109/TSE.2019.2901679}, no systematic analysis of anti-repackaging techniques is still available. To this aim, in this paper we provide an extensive analysis of such techniques. More in details, the contribution of the paper is three-fold: %\alessio{Modify this following part at the end.}. 
after introducing some background and the threat model related to app repackaging in Section \ref{sec:background}, we first discuss the state of the art of anti-repackaging techniques in Section \ref{sec:sota}. Then, in Section \ref{sec:attacking_model} we summarize the attacking techniques that can be used to circumvent anti-repackaging. Finally, in Section \ref{sec:attack} we will show how existing anti-repackaging techniques can be circumvented to produce a fully-working repackaged version of a protected app. 
%Moreover, in Sec \ref{sec:best_defense_technique}, we provide some solutions to recurrent security issues in repackaging avoidance techniques. 
We also discuss a full-fledged attack to the most recent anti-repackaging technique to date, which is the only one whose source code is publicly available. More in detail, we show how to bypass the protections and successfully repackage a real app (i.e., Antiminer \cite{antimine-android}).
Finally, in Section \ref{sec:conclusion} we draw some conclusions, pointing out some guidelines to improve the robustness and the reliability of the next-generation anti-repackaging techniques. 

\begin{comment}
With this approach we want to overcame the assumption made in the state of the art works, that an attacker repackage an app if and only if it is more convenient then reimplement the app from scratch \cite{8186215}.

\end{comment}


%More in details, the contribution of the paper in four-fold:
%\begin{enumerate}
%    \item A review of the main repackaging avoidance techniques in Android, with a specific focus on their implementation (Section \ref{sec:sota}) when available;
 %   \item A categorization of all possible attacks to the repackaging avoidance techniques (Section \ref{sec:attacking_model})
  %  \item For each repackaging avoidance techniques, 
%\end{enumerate}

%Our contribution is an in deep survey of the main anti repackaging techniques proposed over these years, with focus on their implementation. Furthermore, we are also going to analyze to which attacks they are resilient and how to circumvent these techniques in order to produce a fully working repackaged app. Our scope is to identify which approaches are more safe and how much effort is required to implement these anti repackaging methodologies.
%After that, we are going to provide some solutions to recurrent security open issues in some self-defending approach in the state of art works. 
%Finally, we are going to propose a model to utopically ac




%In this paper we want to analyze in details Android repackaging avoidance techniques proposed over the years. 
 
%\subsection{Goal}\label{sec:goal}
%To our knowledge, there is no systematic review of anti repackaging techniques yet. 
\begin{comment}
The first anti repackaging proposal, Divilar \cite{10.1145/2557547.2557558}, tried to introduce a virtualization based protection scheme to secure Dalvik bytecode. Future works tried to implement this technique over native code \cite{2019-exploiting-binary}. 
In 2015 a novel technique \cite{7299906} presented the use of native code to encrypt and decrypt the source code at runtime.
Starting from 2016 a new approach based on insertion of "repackaging detection nodes" inside the original app was proposed in different works \cite{7579771, 8368344}.  The purpose of a detection node is to control the app integrity and to detect any tampering using different techniques, such as assets or code checksum. One of the main issue with this approach is the ease with which a guard can be deleted or bypassed. To overcome this problem, researcher proposed to insert inside this detection nodes some application code, so an attacker can not remove guards without compromising the app functionality \cite{10.1145/3168820, 8186215}. However, with dynamic analysis techniques is possible to circumnavigate this protection. The approach proposed in \cite{10.1007/978-3-030-45371-8_12} tried to make guards more complex using native code. 
Finally, we are going to propose a model to utopically achieve  the perfect anti repackaging technique. 
With this approach we want to overcame the assumption, from state of art works, that an attacker repackage an app if and only if it is more convenient that reimplement the app from scratch \cite{8186215}.

\end{comment}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

%  LocalWords:  biometrics cryptographic parallelized lossy


==> sections/old paper files/results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation}
\label{sec:eval}


The results section should have the results of your experiments and
measurements. Evaluation is the most important part of the research. Sometime
you might want to split it into more than one section depending on the type of the project.



Again make sure you give enough details so that the reader can reproduce your
evaluation. Your GitHub code is not a replacement of the details, GitHub will
perish, your paper will remain in this world for centuries to come. Of course,
you need strike a balance between mundane details vs what makes your evaluation
unique.









==> sections/old paper files/sota.tex <==
\section{Anti-Repackaging: State of the art}\label{sec:sota}
This section presents the state of the art of anti-repackaging techniques on Android, ordered chronologically. For each proposal, we will describe the idea, the protection scheme applied on the app before release, the runtime protection during the app execution, as well as the experimental results. In Section \ref{sec:attack} we will discuss limitations and effective attacks against these works.

\subsection{Self-Protection through \texttt{dex} Encryption} 
\label{subsec:dyn-self-prot-encrypt-2015}
In 2015, M. Protsenko et al. in \cite{7299906} proposed an anti-repackaging technique aimed at complicating both the reverse engineering and the repackaging process. The main idea is to encrypt the \texttt{classes.dex} file in the $apk$, and dynamically decrypt and execute it at runtime. 

\begin{figure}[!ht]
  \includegraphics[width=\textwidth]{figs/self-protecting-encrypted-dex.pdf}
  \caption{The Dynamic Self-Protection and Tamperproofing scheme.}
  \label{fig:dynamic-scheme}
\end{figure}

\paragraph{Protection scheme:}

The approach, depicted in Fig. \ref{fig:dynamic-scheme}, applies to the compiled $apk$, that is modified according to the following steps: 
\begin{enumerate}
    \item A XOR key is generated (Step 2.1) and applied to encrypt the whole \texttt{classes.dex} file(s) (Step 2.2);
    \item An native activity\footnote{An activity is an app window containing the UI.} is automatically built (Step 2.3) and compiled in a shared library. Such activity is called native, as it is written in native code (C/C++ code) instead of Java/Kotlin code as the other activities. The XOR key is added to the native activity;
    \item The native activity is obfuscated using the OLLVM tool \cite{obfuscator-llvm} (Step 2.4);
    \item The Android Manifest is configured to execute the native activity (written in C/C++) rather than the original main activity\footnote{The Main Activity is the first activity prompted to the user when the app is executed.} when the app starts executing (Step 2.5).
\end{enumerate}
Finally, the $apk$ file is generated, signed and delivered (Step 3).
    
\paragraph{Runtime behavior:}
When the app executes, the protection scheme behaves as depicted in Fig. \ref{fig:dynamic-scheme-runtime}. At first, the modified manifest forces the execution of the native activity (Step 6.1). The native activity begins by extracting the XOR key (Step 6.2) and launches the main activity (step 6.3). As the execution of the main activity requires access to the plain bytecode, the XOR key is applied to decrypt only the part of the code required for the proper execution of the main activity. Then, after the execution is completed, the same bytecode is re-encrypted using the same key (Step 6.4). The approach is time-sliced, thereby decrypting parts of the \texttt{classes.dex} file on-demand, i.e., maintaining the bytecode unencrypted only when it needs to execute (Step 6.4).  

\begin{figure}[!ht]
  \includegraphics[width=\textwidth]{figs/self-protecting-encrypted-dex-runtime.pdf}
  \caption{Dynamic Self-Protection and Tamperproofing: runtime behavior}
  \label{fig:dynamic-scheme-runtime}
\end{figure}



%\paragraph{Tampering detection and response}
%In the paper implementation a simple XOR-based hash is used as tamperproofing checksum. If the decryption key is invalid it is not possible to decrypt the correspondent encrypted method.

\paragraph{Evaluation:}
The adoption of a XOR-based encryption of the bytecode is aimed at implementing a tamper-proof checksum.  
This work has been evaluated on 749 apps from the F-Droid app store \cite{f-droid}. Due to implementation and process choices, only 312 apps can be properly protected. For instance, it was not possible to protect apps which make use of Java reflection. The experimental setup leveraged several Android devices equipped with Android 4.4.2, and stimulated through the Android Monkey UI Exerciser framework \cite{monkey} at runtime. Clearly, the adoption of encrypting/decrypting cycles, as well as the addition of extra code, negatively impacts the app time and space complexity. In fact, the experiments indicate a mean execution overhead of 440\% and an increased $apk$ size by 183\% on average. 

The reliability of the proposed protection scheme is evaluated according to four metrics: method exposure (both absolute and percent value), and instructions exposure (both absolute and percent value). A method or a instruction is \textsl{exposed} when it is decrypted. Experimental results show a wide variance. On average, about 83\% of methods - which amount to the 80\% of the bytecode instructions - are exposed. %However, some apps have a relative instruction exposure around 2\%, or in some cases 100\%.

\subsection{Stochastic Stealthy Networks} 
\label{subsec:ssn-2016}
% Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/Repackage-proofing%20Android%20Apps%20~%20Stochastic%20Stealthy%20Network.pdf
% https://cse.sc.edu/~lluo/papers/ssn-robustness-2017.pdf, riassunto nel capitolo 2.1 di bombdroid

In 2016, Lannan Luo et al. put forward another self-protecting approach against repackaging, named Stochastic Stealthy Network (SSN) \cite{7579771}. 
%This work was presented in 2016. 

\begin{figure}[!ht]
  \includegraphics[width=\textwidth]{figs/SNN-scheme.pdf}
  \caption{The SSN protection scheme}
  \label{fig:ssn-scheme}
\end{figure}

\paragraph{Protection scheme:}
The idea is to distribute (and hide) a set of guards (i.e., \textsl{repackaging detection} nodes) into the app source code. When executed, such guards trigger proper decision points (i.e., \textsl{repackaging response} nodes) that, in case a tampering is detected, make the app crash. 
More in detail, the protection workflow, depicted in Figure \ref{fig:ssn-scheme}, begins by selecting a set of candidate methods in the Java code, according to some heuristics (Step 2.1). Then, a set of repackaging detection nodes are injected in such methods (Step 2.2), as well as the set of repackaging response nodes (Step 2.3). Such latter nodes take decisions according to a stochastic function. Moreover, a communication channel is added in the code to allow both kinds of node to communicate at runtime (Step 2.4). The communication channel is made by extra variables and methods added in the app code. Finally, SSN builds, signs and delivers an $apk$ with code extended with the repackaging nodes.

It is worth noticing that the selection of candidate methods must take into consideration the overhead due to the execution of detection and response nodes: to this aim, good candidate methods must be seldom invoked at runtime. Furthermore, the detection nodes must be strongly distributed over the set of candidate methods, to increase stealthiness. 

%\paragraph{Node construction}
%Detection nodes are injected inside candidate methods. Candidate methods are invoked for a few times during the execution of the app. In this way the overhead is lower. 
%Detection nodes are split into several parts in order to achieve better stealthiness. 

\begin{figure}[!htb]
  \includegraphics[width=\textwidth]{figs/SSN-scheme-runtime.pdf}
  \caption{The SSN behavior at runtime.}
  \label{fig:ssn-scheme-runtime}
\end{figure}


\paragraph{Runtime behavior:}
Fig. \ref{fig:ssn-scheme-runtime} depicts the SSN behavior during app execution. Whenever a candidate method executes (Step 6.2) and activates a repackaging detection node (Step 6.3), then the same node connects to the corresponding response node(s) through the communication channel. If the stochastic function recognizes the method as repackaged (i.e., modified) then some execution is triggered. Such execution may lead to modify specific variable values or raise specific exceptions\footnote{Unfortunately, the paper does not provide such details.} that can result in program crashes or delayed logical malfunctions. 

\paragraph{Evaluation:}

The SSN approach only verifies the integrity of candidate methods by relying on the developer's public key verification. However, SSN supports several other predefined templates. For instance, reflection is used to call functions such as \longstring{getPublicKey()} and \longstring{generateCertificate()}. 

The viability of the SSN approach has been empirically evaluated on a set of 600 apps, belonging to ten app categories in F-Droid. Experiments were conducted on emulators equipped with Android 4.1.
The average time overhead is between 6.4\% and 12.4\%, which is far lower than the time overhead of the previous approach, discussed in Section \ref{subsec:dyn-self-prot-encrypt-2015}. Furthermore, each protected app works properly, and no space overhead is noticed. %Authors asked three humans to make a repacked app (previously protected with their prototype) work properly for one hour. They had 24 hours. None of he apps was successfully repackaged. Results show that between 75.3\% and 89.6\% of nodes survived.  

\subsection{AppIS: Protect Android Apps Against Runtime Repackaging Attacks}\label{subsec:appis-2017}
%Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/AppIS-%20Protect%20Android%20Apps%20Against%20Runtime%20Repackaging%20Attacks%20-%20ICPADS_2017.pdf
In 2017, Song et al.\cite{8368344} proposed an app reinforcing framework, named AppIS. The idea of AppIS is to add security units as guards with interlocking relationship between each other, in order to build redundant and reliable anti-repackaging checks.

\begin{figure}
  \includegraphics[width=\textwidth]{figs/AppIS-scheme.pdf}
  \caption{The AppIS protection scheme.}
  \label{fig:appis-scheme}
\end{figure}

\paragraph{Protection scheme:}
Fig. \ref{fig:appis-scheme} depicts the protection workflow of AppIS. The AppIS workflow begins by parsing the compiled $apk$ to extract its corresponding function call graph (Step 2.1), leveraging static analysis techniques at the state of the art. From such graph, AppIS selects a set of sensitive methods, resources or data to protect (Step 2.2), named \textsl{goals}.  Then, AppIS generates a set of guards aimed to protect goals (Step 2.3). Guards can be hosted both in the bytecode (i.e., \longstring{J\_Guard}) and the native code (i.e., \longstring{N\_Guard}). Each goal must be controlled at least by a guard (\longstring{Guard-Goal}) and each guard must be likewise controlled by at least two other guards (\longstring{Guard-Guard}) to improve redundancy and reliability to attacks. According to previous rules, AppIS generates a set of Guard-Goal and Guard-Guard constraints (Step 2.4), which are taken into consideration to build a set of \textsl{guarding nets} among goals and guards, that satisfies all constraints. Moreover, such set is used to construct a scheduling engine that at runtime chooses which guarding net to activate, according to the triggered goal and the execution status. Finally, AppIS builds and delivers the protected $apk$, containing goals, guarding nets and the scheduling engine.

\paragraph{Runtime Behavior:} At runtime the scheduler generates a guarding net (Step 6.1). In this way, a different guarding net is generated at each execution, in order to make the app resilient against cumulative attacks (i.e., multiple execution of the app in a sandboxed environment to detect guards). 
During the execution (Step 6.2), whenever a guard is triggered (Step 6.3), the corresponding guards check the integrity of the goal (i.e., \longstring{J\_Guard}) or the guard (i.e., \longstring{N\_Guard}) (Step 6.4) by comparing the checksum of the goal calculated during the static construction (i.e., Steps 2.3 to 2.5) with the checksum obtained at runtime on the same goal (Step 6.4). If the two checksums do not match, each guard detects a repackaging and the app is directly terminated.

\begin{figure}[!ht]
  \includegraphics[width=\textwidth]{figs/AppIS-scheme-runtime.pdf}
  \caption{AppIS: runtime behavior.}
  \label{fig:appis-runtime}
\end{figure}


%\paragraph{Node construction}
%Guards assure that certain goals (methods, resources or data) are not tampered. Each goals is protected by at least one guard. Goal guard are written in Java (J\_Guard), and their security is monitored by at least other two nodes called guard-guard. These can both written in Java or C/C++ language (N\_Guard) triggered calling the JNI interface.
%To protect against cumulative attack, the guards net is computed when the app is started. In each execution the guards construction net will be totally different. 

%\paragraph{Tampering detection}

%\paragraph{Repackaging response}
%When a repackaging is detected the program is terminated directly.

\paragraph{Evaluation:}
AppIS improves the previous proposals by adding networks of guards and a non-deterministic behavior at runtime, that complicates the attacker analysis activity. AppIS has been evaluated on a very reduced set of only 8 apps, collected from different sources, on almost outdated Android versions (spanning from 4.4 to 6). Experimental results indicate that no app fails, and overheads are reasonable w.r.t. the previous proposals; in fact,  the space overhead is up to 2\% in the worst case, while time overhead spans from 2\% to 140\%. However, we argue that the reduced number of apps is statistically insignificant. %\luigi{Quanto è piccolo il campione lo dobbiamo dire? è composto da sole 8 apps}
The reliability of AppIS has been tested against two threats, namely the possibility for an attacker to i) obtain the collection of the guarding nets, and ii) to carry out cumulative attacks. According to the authors, in both cases the AppIS approach revealed to be reasonably robust.  
%The effectiveness of the protection is evaluated using Microsoft's risk assessment model (DREAD), to quantify the risk of attack. The following two threats were considered: 
%\begin{itemize}
 %   \item Attacker obtains static guarding net collection by reversing engineering. Rating: Medium
  %  \item Attacker launches cumulative attack to AppIS. Rating: Low
%\end{itemize}

\subsection{Self-Defending Code through Information Asymmetry}
\label{subsec:sdc-2018}
% Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Other%20Anti-Repack%20techniques/Leveraging%20Information%20Asymmetry%20to%0ATransform%20Android%20Apps%20into%20Self-Defending%0ACode%20Against%20Repackaging%20Attacks.pdf

In 2018, Kai Chen et al. in \cite{8186215} proposed a self-defending code (SDC) approach, leveraging the information asymmetry between the developer and the attacker on the app code, i.e., it is reasonable to assume that the attacker has far more less information than the developer on the app code, on average. Similarly to the approach discussed in Section \ref{subsec:dyn-self-prot-encrypt-2015}, the idea is to encrypt pieces of source code and decrypt (and properly execute) them at runtime only in case the app has not been repackaged. Unlike the previous work, each piece of code is encrypted with a different key.
The approach provides two schemes, where the first one requires to customize the Android OS, and the second one can work on unmodified OSes. We will focus on the latter one, as we argue that the first scheme cannot scale in the wild, due to the customization needs. 

\paragraph{Protection scheme:}
\begin{figure}
  \includegraphics[width=\textwidth]{figs/SDC-scheme.pdf}
  \caption{The SDC protection scheme.}
  \label{fig:sdc-scheme}
\end{figure}
The scheme (see Figure \ref{fig:sdc-scheme}) begins by analyzing the source code (Step 2.1) and selecting some qualified conditions (i.e., branches containing an equality check, where one of the operands is a constant value: i.e., \longstring{v==const}) in the code that need to be protected. A qualified condition is then substituted by a self-defending code (SDC) (Step 2.2) that hosts the encrypted version of the original code contained in the body of the qualified condition. Once all the pieces of code have been encrypted, a component named \textsl{runtime supporter} is built. Such component contains all the encryption routines which allow understanding how the modified code has been generated (Step 2.3); such routines are useful for reconstructing the original code at runtime.
It is worth pointing out that the encryption scheme is XOR-based and the key is related to the checksum of the original piece of code. Therefore, the original code can be decrypted correctly if and only if the app has not been modified. More in detail, w.r.t. to the sample code at Step 2.1 in Figure \ref{fig:sdc-scheme}, %\luigi{Forse non si capisce quale parte del sample code, quella dello step 2.1}
the information asymmetry between the developer and the attacker is the knowledge of the value \texttt{const}, removed from the source code at compiled time in Step 2.2, and the \longstring{encr\_code}. Furthermore, \longstring{encr\_code} is redundantly protected by a set of other - randomly selected -  SDC segments, some of which implement part of their functions as native code.  
Finally, the protected apk, composed by the DEX code extended with the SDC, the non-code resources and the runtime supporter, is built and delivered.

\paragraph{Runtime Behavior:} At runtime, whenever an SDC is executed, the encrypted code is decrypted by leveraging the app checksum xored with the \texttt{v} value as shown in Step 2.2. If one of these differs from the original values, the decryption fails and the original code is not retrieved, thereby leading the app to crash.
%\begin{figure}
%  \includegraphics[width=\textwidth]{images/sdc.png}
 % \caption{SDC encryption step}
  %\label{fig:sdc}
%\end{figure}
 
 

\paragraph{Evaluation:}
Differently from previous proposals, SDC has been validated on a significant set of apps (i.e., 20,000) taken from Anzhi \cite{anzhi} and belonging to 15 categories. For each app, a set of more than 100 candidate branches has been selected and substituted with SDC segments. The testing phase involved both real users and automatic testing. In the first case, ten  SDC segments where triggered in an hour, while, in the latter case,  five segments were triggered within 24 hours. The time overhead is below 4\% for each app tested, while the space overhead is negligible.

\subsection{BombDroid: Decentralized Repackaging Detection through Logic Bombs} \label{subsec:bombdroid-2018}
% Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/Resilient%20Decentralized%20Android%20Application%20Repackaging%20Detection%20Using%20Logic%20Bombs%20-%20CGO%202018.pdf
In 2018, Zeng et al. in \cite{10.1145/3168820} introduced the concept of \textsl{logic bombs} which are hidden (i.e.,  cryptographically obfuscated) pieces of code that execute once proper triggers (i.e., logical conditions) are activated. The authors implemented the approach in a tool called BombDroid. Like SDC (Section \ref{subsec:sdc-2018}), logic bombs are injected in qualified conditions.

\paragraph{Protection scheme:}
\begin{figure}[!ht]
  \includegraphics[width=\textwidth]{figs/BombDroid-scheme.pdf}
  \caption{The BombDroid protection scheme.}
  \label{fig:bombdroid-scheme}
\end{figure}
The protection scheme of BombDroid (see Figure \ref{fig:bombdroid-scheme}) is very similar to the SDC one, and the idea is to selectively find some candidate condition in the app methods to inject logic bombs. The first difference is that BombDroid works directly on the $apk$ at the bytecode level, and not on the source code. The BombDroid protection scheme begins by reversing the $apk$ (Step 2.1), and parsing the \longstring{classes.dex} file (Step 2.2) through static analysis techniques to identify suitable methods (Step 2.3). In each selected methods, BombDroid identifies at least a qualified condition containing an equality between a variable and a constant value (\longstring{v==const}, see Figure \ref{fig:bombdroid-scheme}). The original code - contained in the corresponding block - is extended with some checks aimed at detecting tampering, and then, encrypted. The encrypted code will be  decrypted at runtime according to the hash value of the variable plus a salt, selected by BombDroid. The decryption key is the value of the constant \texttt{v}. The use of a salt, instead of the checksum of the original method, is the main difference with SDC. The robustness of the scheme is likewise given by the robustness of the hash function, that do not allow guessing the value of \texttt{v}. Moreover, it is worth pointing out that the selected methods can have no qualified condition in principle: in this case, BombDroid can inject artificial qualified conditions to protect. Finally, BombDroid allows nesting logic bombs to improve stealthiness: for instance, with reference to the logic bomb in Step 2.4 of Figure \ref{fig:bombdroid-scheme}, another encrypted logic bomb can be inserted in the decrypted code between the original code and the tampering detection function. 

\begin{comment}
\paragraph{Node construction}

BombDroid rely on logic bombs to detect repackaging. Logic bomb idea, as shown in the original paper, is presented in \autoref{fig:logic-bomb}. 
Logic bombs are i%3CmxGraphModel%3E%3Croot%3E%3CmxCell%20id%3D%220%22%2F%3E%3CmxCell%20id%3D%221%22%20parent%3D%220%22%2F%3E%3CmxCell%20id%3D%222%22%20value%3D%22Step%202.4%22%20style%3D%22text%3Bhtml%3D1%3BstrokeColor%3Dnone%3BfillColor%3Dnone%3Balign%3Dcenter%3BverticalAlign%3Dbottom%3BwhiteSpace%3Dwrap%3Brounded%3D0%3BfontSize%3D12%3BfontStyle%3D0%22%20vertex%3D%221%22%20parent%3D%221%22%3E%3CmxGeometry%20x%3D%22317.78%22%20y%3D%22394.5%22%20width%3D%22144.48%22%20height%3D%2222.5%22%20as%3D%22geometry%22%2F%3E%3C%2FmxCell%3E%3C%2Froot%3E%3C%2FmxGraphModel%3Enserted inside \textit{qualified condition} (QC). A QC is a peace of code where a equality check between two operands (one of which is a constant value) is performed. QC can be found in original code, or artificial ones can be inserted.  
The constant value could be a string, integer or boolean values considering the obfuscation strong, medium or weak respectively. It is calculated the constant hash value using an hash function. In addiction, the original constant value is used to encrypt the QC content. Due to the one-way hash function property, it is hard for a reverse engineer guess the decryption key from the hash value. SHA-128 is the chosen hash function, and AES-128 the encryption function. The logic bomb encrypted payload is stored in a $.dex$ file. 

In order to hide bombs from attackers, authors proposed double-trigger bombs \autoref{fig:double-bomb}, where a second logic bomb is nested inside another one. The trigger condition and the payload of inner bombs are encrypted. The second trigger condition is based on environment parameters such as boot loader versions, brand names, API levels, OS versions, GPS position, and temperature value. With this features authors tried to protect from whitebox fuzzing for high code coverage.
\end{comment}

\paragraph{Runtime behavior:} At runtime, the logic bomb is executed, and the code is properly decrypted only if the value of the variable in the qualified condition is equal to \texttt{const} \footnote{This condition triggers the execution of \longstring{or\_code} in the original code of the candidate method.} and the logic bomb activates. 
Then, a tampering detection function is executed. BombDroid applies three anti-tampering techniques, i.e., at app level, at file level and at code snippet level. 
At compile time, BombDroid stores the original public key in the $apk$, as well as the values of some digests concerning resources and the \longstring{classes.dex} file, and some code snippets. At runtime, tampering functions calculate the digests of such resources and compare them with the stored one: tampering is detected whether one of such value differs from the stored one. In case a tampering is detected, the user could be warned or the app could cause negative user experience.

\paragraph{Evaluation:}
Authors assessed the reliability and the performance of BombDroid on a set of apps (i.e., 963) taken from F-Droid. They exploited Dynodroid \cite{10.1145/2491411.2491450} to execute each app for an hour, repeating the experiment 50 times per app. The execution time overhead is almost negligible (i.e., <2.7\%). The space overhead ranges from 8\% to 13\%. On average, the first logic bomb is triggered between 75 and 164 seconds after the app starts executing, and on average, only the 9.3\% of logic bombs are triggered. 

\subsection{Native Repackaging Protection}
\label{subsec:bombdroid-native-2019}
%Github: https://github.com/Killuaa27/tesi_repo/blob/master/papers/Repackaging/Dynamic/Repackaging_Protection__FPS_Paper%20-%202019.pdf
In 2019, 
Simon Tanner et al. in \cite{10.1007/978-3-030-45371-8_12} proposed an evolution of previous techniques. A prototype of this work is available on GitHub \cite{repackaging-protection}. Like BombDroid, this work is based on cryptographically obfuscated logic bombs, inserted in candidate methods with a qualified condition (i.e., \longstring{v==const}). However, the main difference is that integrity checks and a part of the original app code of the block are executed in native code. We refer this scheme as \textsl{Native Repackaging Protection}\footnote{Authors do no provide a name for this scheme.} (NRP). %The paper was published in 2019.

\paragraph{Protection scheme:} %\alessio{Re-write after modification of the corresponding figure.}
The NRP protection scheme, which mostly resembles the BombDroid and SDC ones, is depicted in Figure \ref{fig:native-bombdroid-evolution}.
\begin{figure}
  \includegraphics[width=\textwidth]{figs/native-bombdroid-evolution.pdf}
  \caption{The Native Repackaging Protection scheme.}
  \label{fig:native-bombdroid-evolution}
\end{figure}
Also in this case, NRP reverses the $apk$ (Step 2.1), parses the \longstring{classes.dex} file (Step 2.2), and finds (or builds artificial) blocks with a qualified condition. Then, it modifies each selected block as follows: i) given the standard condition \longstring{v==const}, NRP calculates the hash value of the constant (i.e., \longstring{HASH = H(const)}) using SHA-1 as the cryptographic hash function. Then, ii) the instructions of the block code (i.e., \longstring{or\_code}) are inserted in a new Java class which is encrypted using AES-128 in CTR mode, using the $const$ value as key. NRP applies several workarounds to preserve the semantic equivalence between the original code and the code contained in the encrypted Java class. Such class (i.e., \longstring{encr\_cl}) contains a single method \longstring{invoke()} which splits the original block code into two parts, namely \longstring{nat\_encr} and \longstring{or\_code2}. The first part refers to a native library which is likewise XOR-encrypted with a random symmetric key (i.e., $native\_key$). Such key is stored in the same encrypted Java class. To decrypt and execute the function \longstring{or\_nat\_code()}, stored in the \longstring{nat\_encr} library, a JNI call is required. \longstring{nat\_encr} contains an anti-tampering check that executes the first part of the original block code only if no tampering is detected. In current implementation, the integrity check verifies the signature of the first 100 bytes of the \longstring{classes.dex} file, whose path is hard-coded in the native library.

\begin{comment}
\paragraph{Node construction}

Like in Bombdroid and SDC, authors search for candidate blocks. A candidate block is an equality check between two operands (one of which is a constant value). The candidate block constant value is transformed in the correspondent hash value using SHA-1 function.
The code block instructions are extracted in a new Java class and encrypted using AES-128 in CTR mode. The key used is the candidate block constant value. Different workarounds are performed to preserve semantic equivalence between the original code and the ciphered corresponding class. Inside the extracted ciphered class a call to a native method is done using Java Native Interface (JNI). Integrity checking is performed inside the native code. In order to make mandatory the execution of the native code, a statement from the extracted block is translated and performed inside the native code. 
The native program code is encrypted with a random symmetric key stored in the encrypted Java class. Xor encryption is used to decode native code. The xor key is a resource, in their implementation case the first 100 bytes of classes.dex file.
\paragraph{Tampering detection}
In authors implementation, the signature of the first 100 bytes of the file \emph{classes.dex} is computed as integrity check. The path of that file is hard-code inside the native library.

\paragraph{Repackaging response}
In the published prototype, when tampering is detected the original ciphered code is not executed, leading to undefined behavior, .
\end{comment}


\paragraph{Runtime behavior:} During execution, the triggering of a logic bomb, depicted in Step 2.4 in Figure \ref{fig:native-bombdroid-evolution}, leads to the following execution: i) once the condition on the hash value is verified (i.e., \longstring{hash(v)==HASH}), the encrypted Java class (\longstring{encr\_cl}) is decrypted according to the constant value, and then the \longstring{invoke()} method is executed through Java reflection. The first statement (\longstring{nat\_encr}) is executed, and leads to the decryption of the native library (\longstring{nat\_encr}) and the execution of the \longstring{or\_code\_nat} block. Then, the signature of the first 100 bytes of the \longstring{classes.dex} file are checked. If the verification succeeds (i.e., \longstring{tamper\_check()==true}), then the first part of the original block code is executed (\longstring{or\_code1}), otherwise the app crashes. After the proper execution of \longstring{or\_code1}, the execution flow is returned to the \longstring{invoke()} method which executes the second part of the original block code (i.e., \longstring{or\_code2}).


\paragraph{Evaluation:}
NRP has been tested against 100 apps downloaded from the Google Play Store and F-Droid. Tests were performed on an LG Nexus 5X device, running Android 8.1.0. In their implementation, authors leverage the \longstring{dalvik.system.InMemoryDexClassLoader} to load the new Java class of each encrypted block. This functionality is available starting from Android 8.0, only. The empirical assessment showed that 47\% of apps could be transformed without runtime exceptions. Each app has been tested through Monkey \cite{monkey} to generate random user's input:  the time overhead is from 1.42\% up to 10.42\% (the space overhead is negligible), while on average, from 11 to 35 logic bombs have been activated. %\alessio{I would move the discussion on the implementation (it is commented now) in the attacking section. Thoughts?}

\begin{comment}
\textbf{Discussion}: We evaluated the tool starting from the source code and we recognized some issues that the authors did not took into consideration in their analysis. First of all, there is an undefined behavior in a native code tampering detection function, where a signed $char$ type is used, instead of an unsigned one which would have been consistent with the Java method. This leads to app instability. \alessio{Please explain why.} 
Furthermore, the authors did not verify the integrity of the user interface (UI). In some apps we encountered UI differences between the original and the protected app. \alessio{Again: what does it imply? Please explain.}
\end{comment}


==> sections/old_methodology.tex <==
\section{Methodology} \label{sec:methodology}
\begin{comment}
Main assumptions (description + advantages):
- multiple patterns
    - Things to avoid (e.g. which AT should be implemented and whats is its goals)
    - more QC in different location (non only for if stmt)
    - add also server checks -> ?!?
    - AT in logic bombs 
    - honeypots
- rely on native code
- Optimized pervasiveness of the logic bombs
    insert logic bomb with a criteria -> e.g. there are a lot of logic bombs in library, but not all are triggered or logic bombs in library can easily decrypted (an attacker can easily detected the encryption key) 
    - hash space -> ?!
- hiding (e.g. nested bombs/nested encryption,  obfuscation)
\end{comment}

In this work, we present \schema{}, a novel methodology that overcomes the main limitations of the current state-of-the-art approaches, by addressing the following challenges - already pinpointed in \cite{merlo2020you} - namely:

\begin{enumerate}
    \item \textbf{Use of multiple patterns} to disseminate and hide detection nodes in the app. Current techniques adhere to a common pattern (i.e., qualifying conditions and adoption of hash functions), which we showed to be rather easy to detect and de-activate by an attacker. To this aim, a novel approach must several - distinct - patterns for the detection nodes to harden the defusing and detection phase. Moreover, the content of the detection node must vary, i.e., use different anti-tampering controls, must be distributed throughout the entire app.
    \item \textbf{Rely on native technologies (C/C++)} to hide detection nodes, as reversing and instrumenting native code significantly increase the detection phase.
    \item \textbf{Optimize the effectiveness} of the detection nodes. Some approaches implement few controls in the name of performance, while others embed many bombs that are not actually triggered at runtime. In this respect, there is a need for more effective deployment of detection nodes, also at the cost of higher time and space overheads.
    \item \textbf{Use Honeypot bombs}. Proper fake bombs can be added to disguise the attacker to remove them. The removal of such bombs should trigger the real ones and lead the app to crash. This idea has been proposed in literature but never actually applied in current proposals, where the focus is more on generating stealthy logic bombs. 
    \item \textbf{Hide the anti-repackaging protection}. It is fundamental to improve the stealthiness of anti-repackaging controls and detection nodes to make it hard for the attacker to understand that the reverse-engineered app includes a protection scheme. Therefore, the new scheme must rely on hiding techniques like obfuscation \cite{} or packing \cite{}. \luca{TODO add citation}
\end{enumerate}

In the rest of this Section, we highlight the main features of \schema{} and detail the protection behavior at runtime. 


\subsection{Multi-patterning \& Anti-Tampering checks} \label{subsec:spatternization} 
% Multiple Patterns and Multiple Anti-Tampering Checks
The distribution of logic bombs affects the robustness of the anti-tampering technique. Unfortunately, current proposals rely on the sole pattern summarized in Section \ref{sub:anti-repackaging}, in which any qualified condition is systematically substituted with on some hash value and the body code encrypted according to the \texttt{const} value. Such pattern can be straightforwardly detected by the attacker through static analysis based on pattern matching (see \cite{merlo2020you} for further detail on attack vector to anti-repackaging). As a consequence, current anti-repackaging proposals are more concerned on spreading a high number of logic bombs rather than hiding the portion on code in which an anti-tampering check can be contained. 
From an attacker's point of view, the knowledge of this well-known pattern allows revealing the potential location of the anti-tampering detection nodes (i.e., all branching containing hash values in their condition) and automate their removal. 

We argue that adopting a multi-pattern distribution of logic bombs can increase the effort of the attacker and reduce the likelihood to remove the whole set of logic bombs.

\paragraph{Multiple logic bomb patterns:}  As introduced above, an attacker can leverage a single combination of function calls to detect the hash-based logic bombs. To counteract this threat, we build logic bombs according to the classical pattern, but we modify their inner code. In this way, even if an attacker detects several logic bombs, she is not able to decrypt them and recover the original code with a single procedure because each bomb has a different inner structure.
More in detail, we adopt six different types of logic bombs:
\begin{enumerate}
    \item \textbf{Honeypots} are fake logic bomb, which do not contain any anti-tampering check. Honeypots aim at tricking the attacker to spend time and effort to uselessly decrypt them.
    \item \textbf{Java bombs} that contain one or more Java anti-tampering checks. 
    \item \textbf{Native-key bombs} are made by encrypted inner code where the decryption key is the return value of an anti-tampering check that is implemented in the native code. 
    \begin{figure}[!ht]
      \includegraphics[width=1.05\textwidth]{figs/native_encryption_procedure.pdf}
      \caption{Creation process of a native key bomb}
      \label{fig:native_encryption_procedure}
    \end{figure}
    Figure \ref{fig:native_encryption_procedure} shows the creation process of this type of bomb. Here, the qualified condition is transformed into the form of the logic bomb (Step 1). Inside the qualified condition a native call is embedded (Step 2) and its return value is used to encrypt the \texttt{or\_code} (Step 3). Then, proper instructions to decrypt and run \texttt{or\_code\_encr} are added (Step 4). In this way, the \texttt{inner\_code} contains the native invocation, the decryption process and the invocation of \texttt{or\_code}. Finally, the \texttt{inner\_code} is encrypted with the \texttt{const} value in the qualified condition (Step 5).  
    \item \textbf{Native AT bomb} implements an anti-tampering check inside the native code. Differently from the previous cases, if the native AT check fails the normal app workflow is broken (i.e. an exception is thrown). In future versions, different actions can be implemented once a tampering is detected.
    \item \textbf{Java AT \& Native key bomb} are bomb analogous to the previous type, but \texttt{or\_code} contains at least one Java anti-tampering check.
    \item \textbf{Java \& Native AT bombs} contain both Java and native anti-tampering checks.
\end{enumerate}
% \antonio{In future work and enhancement section cite that the native call can inserted randomly inside the inner\_code}

\paragraph{Beyond logic bombs:} In addition to logic bombs, it is necessary to embed heterogeneous anti-tampering controls throughout the app. We inserted some detection nodes which check the application integrity. These nodes, called \textbf{Java AT}, are spread through the Java bytecode.
If all detection nodes rely on the same anti-tampering control, an attacker would bypass it to create a working repackaged app.
In our work, each anti-tampering node checks different things, and it detects a \emph{specific type} of repackaging. 
For example, file integrity checks detect a repackaging if and only if the verified file is changed during the repackaging process.
More in general, checking the signature can potentially detect all repackaging: an attacker have to re-sign the repackaged version of the app with his private key (that is different from the developer one).
Furthermore, these checks can be implemented both in Java and native code, in order to increase the amount of work an attacker need to carry out to circumvent these controls.

\paragraph{Deployment of logic bombs:} Another important aspect is where logic bombs are deployed and how anti-tampering checks are inserted. 
In our previous analysis, we notice that some logic bombs could be decrypted only by relying on reverse engineering and open-source information. An example is a logic bomb inserted inside an external open-source library. From the point of view of the defensive technique, these bombs do not add security but only increase the time overhead in the repackaging process.
One of the powerful technique that an attacker can use in the repackaging process is \emph{code instrumentation and injection}\footnote{discussed in \cite{merlo2020you}}, which allow dynamically modification of the code, intercepting function calls, and changing input or return values.
To make the reversing process harder, an anti-tampering control (both in Java and native code) is inserted replicating its bytecode (or assembly code) each time. In this way, we do not rely on a static anti-tampering function that is called from each detection node, despite there is and higher size overhead.



\subsection{Rely on native code}
The reverse engineering and the instrumentation process of native code (assembly code) are more complicated than Java bytecode. Due to this, interacting with native code can increase the difficulty of the repackaging process. 
To interact with native functions, a Java class has to load the shared object (usually with the directive \longstring{System.loadLibrary} \cite{android-jni}) and declare a method with the \texttt{native} keyword (this method tells the virtual machine that the function is implemented in the shared library). Moreover, there are several constraints to be respected (e.g., the name of a native function) when dealing with JNI. Due to this, a native function call could be detected easily. To avoid that an attacker easily removes the call to a native anti-tampering check (e.g., through \emph{code deletion}), the Java code should be dependent on the result of the native function.
To this aim, we identified two kinds of native invocation: \textbf{native key} and \textbf{native AT} (described above in Section \ref{subsec:spatternization})

%JNI spec: https://docs.oracle.com/javase/7/docs/technotes/guides/jni/spec/jniTOC.html

\subsection{Hiding protection}
Logic bombs are a first attempt to hide detection nodes, in which one or more anti-tampering controls can be embedded. Furthermore, logic bombs can be nestedly hidden, i.e., the content of a logic bomb hides another encrypted payload. In this way, an attacker has to decrypt all nested logic bombs to recover and remove the anti-tampering checks.
As we mention above, logic bombs and anti-tampering controls have common patterns that help an attacker in the detection of anti-tampering controls. Obfuscation can be applied to the protected app to hide common features and make hard the repackaging process for an attacker (i.e., detection of logic bombs or anti-tampering checks). 
In our work, we implemented this solution by relying on Obfuscapk \cite{aonzo2020obfuscapk}. 

In conclusion, these considerations lead us to create a protection scheme in which i) there are multiple patterns for logic bombs, ii) logic bombs are inserted through the code with specific and semi-stochastic criteria, iii) other heterogeneous detection nodes are inserted \emph{randomly} in the code and not only inside the logic bombs and iv) there are multiple anti-tampering checks (e.g., signature check, file integrity, package name check) in both Java and native code. % and v) detection nodes are hidden.

\subsection{Runtime behavior}
At runtime, the Java anti-tampering spread out the Java code and the logic bombs are executed. The code in logic bombs is properly decrypted only if the value of the variable (\texttt{v}) in the qualifying condition is equal to \texttt{const}. Then, if the logic bomb contains at least one anti-tampering function, a tampering check is executed. These functions calculate some digests and compare them with the stored one: tampering is detected whether one of such value differs from the stored one. In case tampering is detected, the app crashes and throws an exception. The type of the exception depends on which anti-tampering is executed.

As an example, for native key logic bombs, the native anti-tampering returns the key to decrypt the next code. If tampering is detected, the native function returns a wrong value (i.e., return a wrong decryption key). In this scenario, the $AES$ decryption function fails, throwing an exception.

==> sections/results_old.tex <==
\section{Experimental} \label{sec:experimental_result}
%In this section, we will focus on the experimental data we acquired during the testing and evaluating phases. 

We empirically assessed the reliability of \toolname{} by applying the tool over a set of 30.000 real-world Android apps downloaded from F-Droid \cite{f-droid} and Google Play \cite{google-play-store} between August and October 2020 (cf. \ref{sec:experiments}). Then we evaluated

We empirically assessed the reliability of \toolname{} by applying the tool over a set of 30000 apps . 


The experiments were conducted on a Virtual Machine running Ubuntu 20.04 with 16 dual-core processors and 32GB of RAM. The experimental evaluation used the following parameters: $P_{Java\_AT}=10\%$, $P_{native\_encryption}= 40\%$, $P_{native\_AT}=60\%$, and $PN=ApplicationId$.

%Then, we assessed the time and space overhead of the protections inserted by \toolname{} by testing 220 apps at run-time. 

\subsection{Experimental results}
\label{sec:experiments}
The tool was able to successfully process 27656 out of 30000 apps (i.e., 92.2\%) in nearly 14 days and 5 hours (1.228.009 seconds). 
%In the experimental evaluation we setted $P_{Java\_AT}=10\%$, $P_{native\_encryption}= 40\%$, $P_{native\_AT}=60\%$, and $PN = ApplicationId$.
The analysis of the remaining 2344 apps failed due to \toolname{} transformation errors (i.e., 963 apps), Soot library's well-known issue\footnote{https://github.com/soot-oss/soot/issues/1413, https://github.com/soot-oss/soot/issues/1474} (i.e., 1215 apps) and Axml issues\footnote{https://github.com/soot-oss/soot/issues/1070} (i.e., 166 apps), which resulted in crashes during the analysis of the Java bytecode.
In addition, some protected apps (6115 out of the 27656 apps) have not been equipped with any anti-tampering protection mechanism due to the fact the package name inside the \longstring{AndroidManifest.xml} file contains few lines of Java bytecode (e.g., hybrid app or obfuscated app). For this reason, the tool does not find any candidate qualified condition suitable to embed logic bombs. For these apps, the input package name parameter should be modified properly.

Figure \ref{fig:protection-values-recap} shows the distribution of the protection mechanisms (i.e., Java AT, logic bombs, and the nesting level) over the set of the protected apps. Figure \ref{fig:overhead-recap} depicts the processing time and size overhead distributions.

\begin{figure}
\centering
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/java-at.pdf}
  \caption{Java AT distribution}
  \label{fig:protection-values-recap-java-at}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/lb.pdf}
  \caption{Logic bombs distribution}
  \label{fig:protection-values-recap-lb}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/nesting.pdf}
  \caption{Nesting level distribution}
  \label{fig:protection-values-recap-nesting}
\end{subfigure}
\caption{Protection values}
\label{fig:protection-values-recap}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/graph-processing-time.pdf}
  \caption{Processing time distribution}
  \label{fig:overhead-recap-time}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/graph-size-overhead.pdf}
  \caption{Size overhead distribution}
  \label{fig:overhead-recap-space}
\end{subfigure}
\caption{Processing time and size overhead values}
\label{fig:overhead-recap}
\end{figure}

\paragraph{Protection Level.} 
The results show that \toolname{} successfully includes a fair amount of logic bombs (i.e., 173 on average) distributed among the six possible combinations and Java ATs (i.e., 355 on average). Furthermore, the average nesting level of those bombs is more than two (i.e, 2.3), thus enhancing the difficulty for their removal. In addition, Figure \ref{fig:protection-values-recap-nesting} shows that the main part of the apps have a nesting level higher than 2.
Nevertheless, there are a few exceptions. Indeed, for apps with a limited set of qualified conditions, the tool may introduce a small set of bombs that do not cover all the six possibilities. To this aim, there are a lot of apps with the number of Java AT and logic bombs in the first range of Figure \ref{fig:protection-values-recap-java-at} and Figure \ref{fig:protection-values-recap-lb}.
However, it is worth noticing that such a problem can be overcome by using a more permissive package name to cover, for instance, the entire app (i.e., setting \texttt{PN} to \emph{none}) and not only the $ApplicationID$ package.

\paragraph{Processing Time.} 
Concerning performance, \toolname{} took 1228009 seconds for protecting all the apps, with an average time of 48 seconds per app, thereby suggesting that the approach is viable. The building time is mostly under 2 minutes (i.e., 26103 apps), even for apps having a lot of qualified conditions. During our test, we setted a timeout of 1200 seconds for the protection process. The protection process of 229 of 2344 (i.e., 9.8\%) apps failed due to the timeout is reached. 

\paragraph{Space Overhead.}
The total space overhead is due to two factors: a fixed cost (calculated as less than 1MB), and a dynamic cost related to the number of added detection nodes. In particular, we noticed that the number of Java anti-tampering controls and Native Key or Native AT bombs are directly proportional to the space overhead since they contribute to increase the payload size of each method. Furthermore, since native functions are compiled into a shared object for each architecture and embedded into the application, space overhead is directly proportional to the number of native methods. Finally, it is worth noticing that the average size overhead of protected app in the testbet is limited (only 4.3 MB). Furthermore, Figure \ref{fig:overhead-recap-space} shows that the vast majority of apps (i.e., 25938 of 27656) have a size overhead less than 6MB. All in all, it is worth noticing that only 41 apps violate the size limit of 100MB, imposed by several application stores, such as Google Play \cite{limit-size-android-apk}. For these apps, the average size overhead is 7.5MB, which means that the original apps have already a size near to the limit (i.e., average initial size is 96.7MB).

\subsection{Parameters Tuning}
Since \toolname{} carried out the code transformation according to the probabilities of injection, we conducted a tuning tests to detect the on-average best combination of parameters to ensure a reasonable trade-off between the space and time overhead and the protection level. To do so, we computed fifteen different combinations of $P_{Java\_AT}, P_{native\_key}$, $P_{native\_AT}$. We used a test-bed of 1000 randomly selected apps to evaluate the resulting average number of inserted Java AT, logic bombs, the average achieved nesting level of these bombs, and the average computation values (i.e., time of protection process and size overhead). For the experiments, we used the $ApplicationID$ of the app as \texttt{PN} to be processed. The results of the assessment, reported in Table \ref{table:params_compare}, lead to some considerations.

\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}\% Java\\ AT\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}\% Native\\ key\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}\% Native\\ AT\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Avg. Java\\ AT\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}Avg. LB}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Avg. \\Nesting\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Avg. Protection \\ time (s)\end{tabular}}}&
  \multicolumn{1}{c|}{\textbf{\cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}c@{}}Avg. Size \\ overhead (MB)\end{tabular}}} \\ \hline
\multirow{4}{*}{5} & 30 & 30 & 87 & 95 & 2.4 & 22 & 2.44 \\\cline{2-8}
     & 80 & 20 & 86 & 92 & 2.2 & 23 & 2.73 \\\cline{2-8}
     & 60 & 40 & 86 & 94 & 2.1 & 23 & 2.66 \\\cline{2-8}
     & 40 & 60 & 87 & 95 & 2.1 & 22 & 2.67 \\\cline{2-8}
     & 20 & 80 & 87 & 95 & 2.1 & 23 & 2.66 \\\hline
\multirow{4}{*}{10} & 30 & 30 & 174 & 92 & 2.2 & 23 & 2.56 \\\cline{2-8}
     & 80 & 20 & 172 & 88 & 2.1 & 24 & 2.72 \\\cline{2-8}
     & 60 & 40 & 170 & 89 & 2.1 & 23 & 2.68\\\cline{2-8}
     & 40 & 60 & 174 & 91 & 2.1 & 23 & 2.67 \\\cline{2-8}
     & 20 & 80 & 171 & 90 & 2.1 & 23 & 2.66 \\\hline
\multirow{4}{*}{20} & 30 & 30 & 348 & 85 & 2.1 & 25 & 2.58 \\\cline{2-8}
     & 80 & 20 & 344 & 82 & 2.1 & 26 & 2.77 \\\cline{2-8}
     & 60 & 40 & 345 & 83 & 2.1 & 25 & 2.69\\\cline{2-8}
     & 40 & 60 & 349 & 84 & 2.1 & 25 & 2.68 \\\cline{2-8}
     & 20 & 80 & 345 & 84 & 2.0 & 24 & 2.68 \\\hline
\end{tabular}
\caption{Tuning of \toolname{} input parameters on protection level, computation and space overhead}
\label{table:params_compare}
\end{table}

In all cases, the average nesting level of bombs is greater than 2, while the average number of included \toolname{} detection nodes (i.e, the sum of Java AT and the six types of logic bomb) ranges from 178 to 440. Such results ensure that - despite the input parameters - all the apps are equipped with complex and hard-to-remove bombs. 
Regarding the space overhead, the results underline that the variation of input parameters does not affect significantly the size of the protected apps: most apps have a size overhead of less than 6MB, with an average value around 4MB.

Finally, the experiments underline that most of the overhead in the processing time is due to the percentage of Java anti-tampering ($P_{Java\_AT}$). In details, the average protection time is directly proportional to the number of embedded Java anti-tamperings as those bombs introduce additional bytecode that will be processed. On the contrary, the percentage of native key ($P_{native\_key}$) and native AT ($P_{native\_AT}$) do not significantly affect the compilation time. Changing these values, the percentages of each logic bomb type is altered, but each app has the same number of candidate qualified condition.

\subsection{Runtime Performance}\label{subsec:effectiveness}
We randomly selected 220 apps with at least 5 Java AT and 3 logic bombs from the test-set and we automatically tested both the original and the protected ones at runtime to evaluate the impact of the \toolname{} protection on the performances of the protected app.
These apps have an average of 95 Java AT and 50 logic bombs. For the testing phase, we used an emulated Android 8.0 phone equipped with a dual-core processor, 2GB of RAM, and the latest version of Google Play Services. We executed each app - original and protected one - for few minutes with the same high-level inputs (i.e., inputs that trigger an active element of the activity/view) \antonio{Abbiamo un citazione per il lavoro di Andrea?!?} and we retrieved the percentages of CPU and memory usages of each app every 2 high-level inputs. 

191 out of the 220 protected apps (i.e., 87\%) executed correctly and no new exceptions were thrown. The remaining 29 protected apps (i.e., 13\%) thrown a new exception and crashed during the execution for issue introduced by the protection of \toolname{} (i.e., 23 protected apps), or resulted to be unusable due to the high overhead introduced (i.e., 6 protected apps), e.g., too many logic bombs in a single code snippet.

We collected the execution data for the 191 apps (i.e., the apps without new exceptions), which are exported and compared to evaluate the run-time overhead introduced by the \toolname{} protection. In particular, Figure \ref{fig:overhead-runtime-recap} reports the distribution of the CPU and memory overheads between the protected and the original app. 
These values shows that the runtime overheads (i.e., CPU and memory usage) in the protected apps are negligible, with an average increasing of 3\% in CPU usage and 0.1\% in memory usage. Due to this, the user does not notice relevant \antonio{non ho capito i commenti di Alessio} impact of the app usability, despite the execution of several \emph{Java AT} and \emph{logic bombs} (i.e., in the worst case 1669 Java ATs and 729 logic bombs).
\antonio{Solo per chiarezza: l'overhead è calcolato come (overhead app protetta) - (overhead app originale) per tutti i campioni diviso il numero di campioni. Ad esempio - se per una app X ci sono 3 campioni e l'utilizzo per l'app orginale risulta [(1,10); (2,12); (3,8)], mentre per quella protetta [(1,16); (2,4); (3,9)], allora l'overhead per l'app X è = $((16-10)+(14-12)+(9-8))/3 = (6+2+1)/3 = 3\%$. Inoltre ci sono solo 3 app con overhead di cpu maggiore del 40\% ed il caso pessimo di overhead cpu è 77\% e di overhead memoria è di 0.9\%}

Furthermore, Figure \ref{fig:cpu-overhead} and \ref{fig:memory-overhead} show that the vast majority part of the tested apps (i.e., 180 apps) have a CPU overhead less than 10\% and a memory overhead less than 0.5\%.  

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/cpu-overhead.pdf}
  \caption{CPU overhead distribution}
  \label{fig:cpu-overhead}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/experiments/memory-overhead.pdf}
  \caption{Memory overhead distribution}
  \label{fig:memory-overhead}
\end{subfigure}
\caption{Runtime analysis result}
\label{fig:overhead-runtime-recap}
\end{figure}


